Signal-to-noise ratio aware minimax analysis of sparse linear regression

We consider parameter estimation under sparse linear regression -- an extensively studied problem in high-dimensional statistics and compressed sensing. While the minimax framework has been one of the most fundamental approaches for studying statistical optimality in this problem, we identify two important issues that the existing minimax analyses face: (i) The signal-to-noise ratio appears to have no effect on the minimax optimality, while it shows a major impact in numerical simulations. (ii) Estimators such as best subset selection and Lasso are shown to be minimax optimal, yet they exhibit significantly different performances in simulations. In this paper, we tackle the two issues by employing a minimax framework that accounts for variations in the signal-to-noise ratio (SNR), termed the SNR-aware minimax framework. We adopt a delicate higher-order asymptotic analysis technique to obtain the SNR-aware minimax risk. Our theoretical findings determine three distinct SNR regimes: low-SNR, medium-SNR, and high-SNR, wherein minimax optimal estimators exhibit markedly different behaviors. The new theory not only offers much better elaborations for empirical results, but also brings new insights to the estimation of sparse signals in noisy data.

==> draft.tex <==
First, it's easy to show that $\mathcal{B}_{n,p} \overset{p}{\rightarrow} +\infty$ since
\begin{equation*}
    \frac{\mu^{2}}{2} \|x_{1}\|^{2} + \mu x_{1}^{T} z = \frac{\mu^{2}}{2} \Big( 1+O_{p}(\frac{1}{\sqrt{n}}) \Big) + \mu \cdot O_{p} (1) \overset{p}{\rightarrow} 0 
\end{equation*}
as $p-1 \rightarrow +\infty$ and $\mu\rightarrow 0$.

Next, we show that as $\mu\rightarrow 0$, $\mathcal{A}_{n,p} \overset{p}{\rightarrow} 1$. We utilize the weak law of triangular arrays in Lemma \ref{lem::WLLN-triangular}. Let 
\begin{equation*}
    Y_{p,i} := \exp\Big[ \|\mu x_{1} + z\|\mu x_{i,1} - \frac{\mu^{2}}{2}x_{i,1}^{2} - \frac{\mu^{2}}{2}\|x_{i,-1}\|^{2} \Big].
\end{equation*}
Then
\begin{equation*}
    \mathcal{A}_{n,p} = \frac{1}{p-1}\sum_{i=2}^{p} Y_{p,i}.
\end{equation*}
For certain $b$ to be determined, we need to prove
\begin{enumerate}[label=(\roman*)]
    \item $\sum_{i=2}^{p}P\Big(Y_{p,i}>b ~\Big|\|\mu x_{1}+z\| \Big) \rightarrow 0 $ a.s..
    \item $b^{-2} \sum_{i=2}^{p} \E \Big [ Y_{p,i}^{2} \mathbbm{1}_{(Y_{p,i}\leq b)} ~\Big| \|\mu x_{1} + z\| \Big] \rightarrow 0$ a.s..
\end{enumerate}

For condition (i), following the calculations in \eqref{eq::simplified-cond-i-WLLNtriangular} and adopting the non-central $\chi^{2}$ inequality in Lemma \ref{lem::concentration-non-central-chisquare}, we have
\begin{eqnarray*}
    && \sum_{i=2}^{p} P\Big(Y_{p,i}>b ~\Big|\|\mu x_{1}+z\| \Big) \\
    &=& (p-1) P \bigg[ \Big( \sqrt{n}x_{i,1} - \frac{\sqrt{n}}{\mu} \|\mu x_{1}+ z\| \Big)^{2} + \Big(\sqrt{n} \|x_{i,-1}\|\Big)^{2} < \frac{n}{\mu^{2}} \Big( \|\mu x_{1}+z\|^{2} -2\log b \Big) ~\Big | \|\mu x_{1}+z\| \bigg] \\
    &=& (p-1) P \bigg( \chi_{n}^{2}(\lambda_{1}) < \frac{n}{\mu^{2}} \big( \|\mu x_{1} + z\|^{2} -2\log b \big) ~\Big| \|\mu x_{1}+z\| \bigg) \\
    & \leq & (p-1) \exp \bigg[ - \frac{n c_{1}^{2}}{4(n+2\lambda_{1})^{2}} \bigg] \\
    &=& \exp \bigg[ - \frac{n}{4(n+2\lambda_{1})^{2}}\Big( c_{1} - \frac{2(n+2\lambda_{1})}{\sqrt{n}}\sqrt{\log(p-1)} \Big)\Big( c_{1} + \frac{2(n+2\lambda_{1})}{\sqrt{n}}\sqrt{\log(p-1)} \Big) \bigg].
\end{eqnarray*}
where $c_{1}= n+ n/\mu^{2} \cdot 2\log b$ and $\lambda_{1} = n/\mu^{2} \cdot \|\mu x_{1} + z\|^{2}$. Select $b$ such that
\begin{align}
    & 2\log b = 4 \sqrt{n\cdot\log (p-1)} \cdot (1+o(1)), \text{ and} \label{eq::b-selection-i}\\
    & 2\log b - 4 \sqrt{n \cdot \log (p-1)} = \omega \Big( \sqrt{\frac{n}{\log(p-1)}} \Big). \label{eq::b-selection-ii}
\end{align}
There exists such choice of $b$ since $\log p \rightarrow \infty$. As $\|\mu x_{1} + z\|^{2}/n \rightarrow 1$ a.s. and $\mu\rightarrow0$, we have $c_{1} = n/\mu^{2}\cdot 2\log b \cdot (1+o(1))$ and $\lambda_{1} = n^{2}/\mu^{2} \cdot (1+o_p(1))$. By continuous mapping theorem, the above choice of $b$ gives
\begin{align*}
    & c_{1} = \frac{2(n+\lambda_{1})}{\sqrt{n}} \sqrt{\log (p-1)} \cdot (1+o_{p}(1)), \text{ and} \\
    & \bigg[\frac{n}{4(n+2\lambda_{1})^{2}}\Big( c_{1} + \frac{2(n+2\lambda_{1})}{\sqrt{n}}\sqrt{\log(p-1)} \Big)\bigg]^{-1} = o_{p} \Big( c_{1} - \frac{2(n+2\lambda_{1})}{\sqrt{n}}\sqrt{\log(p-1)} \Big).
\end{align*}
Thus,
\begin{equation*}
    \sum_{i=2}^{p} P\Big(Y_{p,i}>b ~\Big|\|\mu x_{1}+z\| \Big) \rightarrow 0 \text{ a.s..}
\end{equation*}

For condition (ii), following the calculation in \eqref{eq::simplified-cond-ii-WLLNtriangular} and applying Lemma \ref{lem::concentration-non-central-chisquare}, we have
\begin{eqnarray*}
    && \sum_{i=2}^{p} \E \Big[ Y_{p,i}^{2} \mathbbm{1}_{(Y_{p,i}\leq b)} ~ \Big | \|\mu x_{1} + z\| \Big] \\
    &=& (p-1) \Big(1+\frac{2\mu^{2}}{n}\Big)^{-n/2} \exp \bigg( \frac{2\|\mu x_{1}+ z\|^{2}}{2+n/\mu^{2}} \bigg) \\
    && \cdot P\bigg[ \Big(Z - \frac{n/\mu^{2}}{\sqrt{2+n/\mu^{2}}} \|z+\mu x_{1}\| \Big)^{2} + \chi_{n-1}^{2} \geq \Big(2 +n/\mu^{2}\Big)\Big(\|\mu x_{1} + z\|^{2} - 2\log b \Big) ~\Big | \|\mu x_{1}+z\| \bigg] \\
    &\leq& (p-1)  \Big(1+\frac{2\mu^{2}}{n}\Big)^{-n/2} \exp \bigg( \frac{2\|\mu x_{1}+ z\|^{2}}{2+n/\mu^{2}} \bigg).
\end{eqnarray*}
Since $n/\log (p-1) \rightarrow \infty$, the selection of $b$ in \eqref{eq::b-selection-i} satisfies
\begin{equation*}
    2\log b = 4 \sqrt{n\log(p-1)} = \omega \big( \log(p-1) \big).
\end{equation*}
Thus,
\begin{equation*}
    (p-1)  \Big(1+\frac{2\mu^{2}}{n}\Big)^{-n/2} \exp \bigg( \frac{2\|\mu x_{1}+ z\|^{2}}{2+n/\mu^{2}} \bigg) = (p-1) \cdot \exp\Big(\mu^{2}\cdot (1+o_{p}(1))\Big) = o_{p} (b^{2}).
\end{equation*}
Therefore,
\begin{equation*}
    b^{-2} \sum_{i=2}^{p} \E \Big[ Y_{p,i}^{2} \mathbbm{1}_{(Y_{p,i}\leq b)} ~ \Big | \|\mu x_{1} + z\| \Big] \rightarrow 0 \text{ a.s..}
\end{equation*}

It remains to check 
\begin{equation*}
    a_{n,p}:= \sum_{i=2}^{p} \E \Big[ Y_{p,i} \mathbbm{1}_{(Y_{p,i}\leq b)} ~\Big| \|\mu x_{1}+z\|\Big] = (p-1) \cdot (1+o_{p}(1)).
\end{equation*}
From the calculation in \eqref{eq::a_n_p-calculation}, we have
\begin{eqnarray*}
    a_{n,p} &=& \sum_{i=2}^{p} \E \Big[ Y_{p,i} \mathbbm{1}_{(Y_{p,i}\leq b)} ~\Big| \|\mu x_{1}+z\|\Big] \\
    &=& (p-1) \Big(1 +\mu^{2}/n \Big)^{-n/2} \exp\bigg( \frac{\|\mu x_{1} + z\|^{2}}{2(1+n/\mu^{2})} \bigg) \bigg( 1- P\Big[ \chi_{n}^{2} (\lambda_{3}) \leq n+\lambda_{3}-c_{3} ~\Big | \|\mu x_{1} + z \| \Big] \bigg),
\end{eqnarray*}
where $c_{3}= (1+n/\mu^{2})\cdot2\log b + n - \frac{1+2n/\mu^{2}}{1+n/\mu^{2}} \|\mu x_{1} + z\|^{2}$ and $\lambda_{3} = \frac{(n/\mu^{2})^{2}}{1+n/\mu^{2}}\|\mu x_{1} + z\|^{2}$.
We will show that
\begin{equation*}
    P\Big[ \chi_{n}^{2} (\lambda_{3}) \leq n+\lambda_{3}-c_{3} ~\Big | \|\mu x_{1} + z \| \Big] \rightarrow 0 \text{ a.s..}
\end{equation*}
Applying the concentration inequality in Lemma \ref{lem::concentration-non-central-chisquare}, we have
\begin{equation*}
    P\Big[ \chi_{n}^{2} (\lambda_{3}) \leq n+\lambda_{3}-c_{3} ~\Big | \|\mu x_{1} + z \| \Big] \leq \exp \bigg[ - \bigg( \frac{\sqrt{n}c_{3}}{2(n+\lambda_{3})} \bigg)^{2} \bigg].
\end{equation*}
Adopting the selection of $b$ in \eqref{eq::b-selection-i} and using $\mu \rightarrow 0$ and $\|\mu x_{1} + z\|^{2}/ n \rightarrow 1$ a.s., we have
\begin{align*}
    c_{3} = n/\mu^{2} \cdot 4 \sqrt{n \log (p-1)} \cdot (1+o(1)) + n - 2 n \cdot (1+o_{p}(1)) = 4 n/\mu^{2} \sqrt{n \log (p-1)} (1+o_{p}(1)),
\end{align*}
and $\lambda_{3} = n^{2}/\mu^{2} \cdot (1+o_{p}(1))$. Thus,
\begin{equation*}
    \frac{\sqrt{n}c_{3}}{2(n+2\lambda_{3})} = \sqrt{\log (p-1)} \cdot (1+o_{p}(1)) \rightarrow + \infty \text{ a.s..}
\end{equation*}
Therefore,
\begin{equation*}
    P\Big[ \chi_{n}^{2} (\lambda_{3}) \leq n+\lambda_{3}-c_{3} ~\Big | \|\mu x_{1} + z \| \Big] \rightarrow 0 \text{ a.s..}
\end{equation*}
As $\mu \rightarrow 0$ and $\|\mu x_{1} + z\|^{2} / n \rightarrow 1$ a.s., we obtain 
\begin{equation*}
    a_{n,p} = (p-1) \cdot (1+o_{p}(1)).
\end{equation*}
Thus, from Lemma \ref{lem::WLLN-triangular} and using the bounded convergence theorem, we have for $\forall \epsilon > 0$,
\begin{equation*}
    P\bigg( \bigg| \frac{S_{n,p}-a_{n,p}}{b_{n,p}}\bigg| > \epsilon \bigg) = \E P\bigg( \bigg| \frac{S_{n,p}-a_{n,p}}{b_{n,p}}\bigg| > \epsilon \bigg | \|\mu x_{1} + z\| \bigg) \rightarrow 0.
\end{equation*}
Combining this with $a_{n,p}/(p-1) \overset{p}{\rightarrow} 1$, we conclude
\begin{equation*}
    \mathcal{A}_{n,p} \overset{p}{\rightarrow} 1.
\end{equation*}

%%%%%%%%%%%%%%%%%%%%%%% original proof of first order lowr bound of sparse minimax problem
Let $a_{n,p} := \sum_{i=2}^{p} \E \left[ Y_{p,i}\mathbbm
    {1}_{(Y_{p,i}\leq b)} | \|z+\tau x_{1}\| \right]$ and $S_{n,p} := \sum_{i=2}^{p} Y_{p,i}$, then using Lemma \ref{lem::WLLN-triangular} we will have
    \begin{equation*}
        P\left( \left. \left|\frac{S_{n,p} - a_{n,p}}{b_{n,p}}\right| > \epsilon \right\vert \|z+\tau x_{1}\| \right) \rightarrow 0 \text{ a.s. } \forall \epsilon >0.
    \end{equation*}
    $Y_{p,i} \leq b$ is equivalent to 
    \begin{eqnarray*}
        && \exp\left[ -\frac{1}{2} (\tau x_{i,1} - \|\tau x_{1} + z\|)^{2} - \frac{1}{2} \tau^{2} \|x_{i,-1}\|^{2} + \frac{1}{2}\|\tau x_{1} + z\|^{2} \right] \leq b \\
        &\Leftrightarrow& (\tau x_{i,1} - \|\tau x_{1} + z\|)^{2} + (\tau \|x_{i,-1}\|)^{2} \geq \|\tau x_{1} + z\|^{2} - 2\log b.
    \end{eqnarray*}
    We claim that: in condition (i),
    \begin{eqnarray}
        && \sum_{i=2}^{p} P(Y_{p,i}> b |\|\tau x_{1} + z\|) \label{eq::simplified-cond-i-WLLNtriangular}\\
        &=& (p-1) P\left( \left. \left(\sqrt{n} x_{i,1} - \frac{\sqrt{n}}{\tau}\|\tau x_{1} + z\|\right)^{2} + (\sqrt{n}\|x_{i,-1}\|)^{2} < \frac{n}{\tau^{2}} (\|\tau x_{1} + z\|^{2} - 2\log b) \right\vert \|\tau x_{1} + z\| \right). \nonumber
    \end{eqnarray}
    In condition (ii), 
    \begin{eqnarray}
        && \sum_{i=2}^{p} \E\left[Y_{p,i}^{2}\mathbbm{1}_{(Y_{p,i}\leq b)}|\|\tau x_{1} + z\|\right] \label{eq::simplified-cond-ii-WLLNtriangular}\\
        &=& (p-1) \left(1+\frac{2\tau^{2}}{n}\right)^{-\frac{n}{2}} \exp \left( \frac{2\| \tau x_{1} + z\|^{2}}{2+n/\tau^{2}} \right) \cdot \nonumber\\
        && P\left[\left. \left(Z - \frac{n/\tau^{2}}{\sqrt{2+n/\tau^{2}}} \|z+\tau x_{1}\| \right)^{2} + \chi_{n-1}^{2} \geq (2+\frac{n}{\tau^{2}})(\|\tau x_{1} + z\|^{2} - 2\log b)  \right\vert \|\tau x_{1} + z\|\right], \nonumber
    \end{eqnarray}
    where $Z\sim \mathcal{N}(0,1)$, $\chi_{n-1}^{2}$ is chi-squared variable with degrees of freedom $n-1$. $(Z, \chi_{n-1}^{2}, x_{1}, z)$ are mutually independent. 

    We only need to show the calculation for condition (ii).
    \begin{eqnarray*}
        && \E \left[\E\left( \left.Y_{p,i}^{2} \mathbbm{1}_{(Y_{p,i}\leq b)} \right\vert x_{i,-1}, \|z+\tau x_{1}\|\right)\right] \\ 
        &=& \E\left[ \E \left(\exp\left( 2\tau \|\tau x_{1} + z\| x_{i,1} - \tau^{2} x_{i,1}^{2} - \tau^{2} \|x_{i,-1}\|^{2} \right) \cdot\right.\right.\\
        &&\left.\left.\left. \mathbbm{1}_{((\tau x_{i,1} - \|\tau x_{1} + z\|)^{2} + (\tau \|x_{i,-1}\|)^{2} \geq \|\tau x_{1} + z\|^{2} - 2\log b)} \right\vert x_{i,-1}, \|z+\tau x_{1}\|\right)\right] \\
        &=& \E \left[ \frac{1}{\sqrt{1+2\tau^{2}/n}} \exp\left( \frac{2\|z+\tau x_{1}\|^{2}}{2+n/\tau^{2}}\right) \cdot \exp\left(-\tau^{2}\|x_{i,-1}\|^{2}\right) \cdot \right. \\
        && \left. \left. \mathbbm{1}_{\left[\left(Z-\frac{n/\tau^{2}}{\sqrt{2+n/\tau^{2}}}\|z+\tau x_{1}\|\right)^{2} \geq \left(2+\frac{n}{\tau^{2}}\right)\left(\|\tau x_{1}+z\|^{2} - 2\log b - \tau^{2} \|x_{i,-1}\|^{2}\right)\right]} \right\vert \|z+\tau x_{1}\|\right], \\
        &=& \left(1+\frac{2\tau^{2}}{n}\right)^{-\frac{1}{2}} \exp\left( \frac{2\|z+\tau x_{1}\|^{2}}{2+n/\tau^{2}}\right)  \E\left[ \exp\left(-\frac{\tau^{2}}{n} \cdot n \|x_{i,-1}\|^{2}\right) \cdot \right.\\
        && \left. \left. \mathbbm{1}_{\left[ n\|x_{i,-1}\|^{2} \geq \frac{n}{\tau^{2}} \left( \|\tau x_{1} + z\|^{2} - 2\log b \right) - \frac{n/\tau^{2}}{2+n/\tau^{2}} \left( Z - \frac{n/\tau^{2}}{\sqrt{2+n/\tau^{2}}} \|\tau x_{1} + z\| \right)^{2}  \right]} \right\vert \|\tau x_{1} + z\| \right] \\
        &=& \left(1+\frac{2\tau^{2}}{n}\right)^{-\frac{n}{2}} \exp\left( \frac{2\|z+\tau x_{1}\|^{2}}{2+n/\tau^{2}}\right) \cdot \\
        && P\left( \left. \chi_{n-1}^{2} \geq \left(1+\frac{2\tau^{2}}{n}\right) \left[ \frac{n}{\tau^{2}} \left( \|\tau x_{1} + z\|^{2} - 2\log b \right) - \frac{n/\tau^{2}}{2+n/\tau^{2}} \left(Z - \frac{n/\tau^{2}}{\sqrt{2+n/\tau^{2}}}\|z+\tau x_{1}\|\right)^{2} \right] \right\vert \|\tau x_{1} + z\| \right) \\
        &=& \left(1+\frac{2\tau^{2}}{n}\right)^{-\frac{n}{2}} \exp\left( \frac{2\|z+\tau x_{1}\|^{2}}{2+n/\tau^{2}}\right) \cdot \\
        && P\left( \left. \left(Z - \frac{n/\tau^{2}}{\sqrt{2+n/\tau^{2}}}\|z+\tau x_{1}\|\right)^{2} + \chi_{n-1}^{2} \geq \left(2 + \frac{n}{\tau^{2}}\right) \left( \|\tau x_{1} + z\|^{2} - 2\log b \right) \right\vert \|\tau x_{1} + z\| \right),
    \end{eqnarray*}
    where $Z\sim \mathcal{N}(0,1)$ and is independent of $x_{1}, z, x_{i,-1}$, and $\chi_{n-1}^{2}$ is independent of $Z, x_{1}, z$.

    Both condition (i) and (ii) are related to probabilities of non-central chisquare. We apply the results in Lemma \ref{lem::concentration-non-central-chisquare} for estimation. From \eqref{eq::simplified-cond-i-WLLNtriangular}, let $\lambda_{1} = \frac{n}{\tau^{2}} \|\tau x_{1} + z\|^{2}$, we have
    \begin{eqnarray*}
        && \sum_{i=2}^{p} P\left(\left. Y_{p,i}> b \right\vert \|z+\tau x_{1}\|\right) \\
        &=& (p-1)P\left(\left. \chi_{n}^{2}(\lambda_{1}) < \frac{n}{\tau^{2}} \left(\|\tau x_{1} + z\|^{2} - 2\log b \right) \right\vert \|\tau x_{1} + z\| \right) \\
        &\leq& (p-1) \exp\left[ -\frac{nc_{1}^{2}}{4(n+2\lambda_{1})^{2}} \right],
    \end{eqnarray*}
    where $c_{1} = n+\lambda_{1} - \frac{n}{\tau^{2}} (\|\tau x_{1} + z\|^{2} - 2\log b) = n +\frac{n}{\tau^{2}}2\log b$. Select $b$ satisfying the followings and denoted by $b^{*}$:
    \begin{eqnarray}
        && 2\log b - \left[ \left(n+2\frac{n}{\tau^{2}} \|\tau x_{1} + z\|^{2}\right) \sqrt{\frac{2}{n}} \nu_{p} - n \right] \frac{\tau^{2}}{n} \rightarrow +\infty, \label{eq1::truncation-choice-first-order-spike}\\
        &\&& 2\log b = \left[ \left(n+2\frac{n}{\tau^{2}} \|\tau x_{1} + z\|^{2}\right) \sqrt{\frac{2}{n}} \nu_{p} - n \right] \frac{\tau^{2}}{n} (1+o(1)). \label{eq2::truncation-choice-first-order-spike}
    \end{eqnarray}
    We will show that this choice of $b^{*}$ satisfies both condition (i) and (ii). For condition (i), we have
    \begin{eqnarray*}
        && \sum_{i=2}^{p} P\left( \left. Y_{p,i} > b^{*} \right\vert \|\tau x_{1} + z\| \right) \\
        &\leq& \exp\left[ \frac{n}{4(n+2\lambda_{1})^{2}} \left( - \left(n+\frac{n}{\tau^{2}}2\log b^{*} \right)^{2} + \frac{4(n+2\lambda_{1})^{2} \log (p-1)}{n}\right) \right] \\
        &\leq& \exp\left[ \frac{n}{4(n+2n\|\tau x_{1} + z\|^{2}/\tau^{2})^{2}} \left( n + \frac{n}{\tau^{2}} 2\log b^{*} + \frac{\sqrt{2} (n + 2n\|\tau x_{1}+ z\|^{2}/\tau^{2} ) \nu_{p}}{\sqrt{n}} \right) \right.\\
        && \left. \cdot \left( -n-\frac{n}{\tau^{2}} 2\log b^{*} + \frac{\sqrt{2} (n+2n \|\tau x_{1} + z\|^{2} /\tau^{2})\nu_{p}}{\sqrt{n}} \right)\right] \\
        &\overset{(*)}{\rightarrow}& 0 \text{ a.s..}
    \end{eqnarray*}
    The selection of $b^{*}$ makes $\left( -n-\frac{n}{\tau^{2}} 2\log b^{*} + \frac{\sqrt{2} (n+2n \|\tau x_{1} + z\|^{2} /\tau^{2})\nu_{p}}{\sqrt{n}} \right) \rightarrow -\infty$. Using the fact that $n^{-1}\|\tau x_{1}+z\|^{2} \rightarrow 1$ a.s. from strong law of large numbers and $\tau^{2} = o(n)$, we obtain (*).

    For condition (ii), from \eqref{eq::simplified-cond-ii-WLLNtriangular}, let $\delta_{0}$ denote a positive constant, we have
    \begin{eqnarray*}
        && (b^{*})^{-2} \sum_{i=2}^{p} \E \left[ \left. Y_{p,i}^{2} \mathbbm{1}_{(Y_{p,i}\leq b^{*})} \right\vert \|z+\tau x_{1}\|\right] \\
        &\leq& (b^{*})^{-2} (p-1) \left(1+\frac{2\tau^{2}}{n}\right)^{-\frac{n}{2}} \exp\left( \frac{2\|\tau x_{1} + z\|^{2}}{2+n/\tau^{2}} \right) \\
        &\leq& (1+\delta_{0}) e^{-\tau^{2}} (b^{*})^{-2} (p-1) \exp\left( \frac{2\|\tau x_{1} + z\|^{2}}{2+n/\tau^{2}} \right) \\
        &=& (1+\delta_{0}) \exp \left( -2\log b^{*} + \log (p-1) -\tau^{2} + \frac{2\|\tau x_{1} + z\|^{2}}{2+n/\tau^{2}} \right) \\
        &\leq& (1+\delta_{0}) \exp \left( -\left[ \left(n+2n\|\tau x_{1} + z\|^{2}/\tau^{2}\right)\sqrt{\frac{2}{n}}\nu_{p} - n \right] \frac{\tau^{2}}{n} + \frac{1}{2}\nu_{p}^{2} - \tau^{2} + \frac{2\|\tau x_{1} + z\|^{2}}{2+n/\tau^{2}} \right) \\
        &=& (1+\delta_{0}) \exp \left[ \left( -2\sqrt{2} \frac{\nu_{p}}{\sqrt{n}} + \frac{2}{2+n/\tau^{2}} \right) \|\tau x_{1} + z\|^{2} + \frac{1}{2}\nu_{p}^{2} - \sqrt{2} \frac{\tau^{2}}{\sqrt{n}} \nu_{p} \right] \\
        &=& (1+\delta_{0}) \exp \left[ \left( -2\sqrt{2} \frac{\nu_{p}}{\sqrt{n}} + o\left(\frac{\nu_{p}}{\sqrt{n}}\right) \right) \|\tau x_{1} + z\|^{2} + \frac{1}{2}\nu_{p}^{2} + o\left(\nu_{p}^{2}\right) \right] \\
        &\rightarrow& 0 \text{ a.s.,} \quad \text{ since } \|\tau x_{1} + z\|^{2}/n \rightarrow 1 \text{ a.s..}
    \end{eqnarray*}

    Finally, we need to calculate $a_{n,p} := \sum_{i=2}^{p} \E \left[ \left. Y_{p,i} \mathbbm{1}_{(Y_{p,i}\leq b^{*})} \right\vert \|z+\tau x_{1}\| \right]$ and verify $a_{n,p} = \omega(b_{n,p}^{*})$. Similar to the calculation of \eqref{eq::simplified-cond-ii-WLLNtriangular}, we have
    \begin{eqnarray}
        a_{n,p} &=& \sum_{i=2}^{p} \E \left[ \left. Y_{p,i} \mathbbm{1}_{(Y_{p,i}\leq b^{*})} \right\vert \|z+\tau x_{1}\| \right] \nonumber\\
        &=& (p-1) \left(1+\tau^{2}/n\right)^{-\frac{n}{2}} \exp \left( \frac{\|z+\tau x_{1}\|^{2}}{2(1+n/\tau^{2})} \right) \cdot \nonumber\\
        && P\left[  \left(Z-\frac{n/\tau^{2}\|z+\tau x_{1}\|}{\sqrt{1+n/\tau^{2}}}\right)^{2} + \chi_{n-1}^{2} \geq \left(1+\frac{n}{\tau^{2}}\right) \left( \|z+\tau x_{1}\|^{2} - 2\log b^{*} \right) \right] \nonumber\\
        &=& (p-1) \left(1+\tau^{2}/n\right)^{-\frac{n}{2}} \exp \left( \frac{\|z+\tau x_{1}\|^{2}}{2(1+n/\tau^{2})} \right) \left( 1-P\left[ \left.\chi_{n}^{2}(\lambda_{3}) \leq n+\lambda_{3}-c_{3} \right\vert \|z+\tau x_{1}\| \right] \right), \label{eq::a_n_p-calculation}
    \end{eqnarray}
    and using Lemma \ref{lem::concentration-non-central-chisquare}, 
    \begin{equation}
        P\left( \left. \chi_{n}^{2}(\lambda_{3}) \leq n + \lambda_{3} -c_{3} \right\vert \|z+\tau x_{1}\| \right) \leq \exp \left[ -\left(\frac{\sqrt{n}c_{3}}{2(n+2\lambda_{3})}\right)^{2} \right], \label{eq::probability-first-order-spike}
    \end{equation}
    where $\lambda_{3} = \frac{(n/\tau^{2})^{2}}{1+n/\tau^{2}}\|z+\tau x_{1}\|^{2}$ and
    \begin{eqnarray*}
        c_{3} &=& n + \frac{(n/\tau^{2})^{2}}{1+n/\tau^{2}}\|z+\tau x_{1}\|^{2} - (1+n/\tau^{2}) (\|z+\tau x_{1}\|^{2} - 2 \log b^{*}) \\
        &=& (1+n/\tau^{2}) 2\log b^{*} + n - \frac{1+2n/\tau^{2}}{1+n/\tau^{2}} \|z+\tau x_{1}\|^{2} \\
        &\geq& \left(1+\frac{n}{\tau^{2}}\right) \frac{\tau^{2}}{n} \left[ \left( n+2\frac{n}{\tau^{2}} \|z+\tau x_{1}\|^{2} \right) \sqrt{\frac{2}{n}} \nu_{p} - n \right] + n - \frac{1+2n/\tau^{2}}{1+n/\tau^{2}} \|z+\tau x_{1}\|^{2} \\
        &=& \left[ 2 \left(1+\frac{n}{\tau^{2}}\right)\sqrt{\frac{2}{n}} \nu_{p} - \frac{1+2n/\tau^{2}}{1+n/\tau^{2}} \right] \|z+\tau x_{1}\|^{2} - \tau^{2} \\
        &\geq& \left[ 2\sqrt{2} \frac{\sqrt{n}\nu_{p}}{\tau^{2}} + o\left( \frac{\sqrt{n} \nu_{p}}{\tau^{2}} \right) \right] \|z+\tau x_{1}\|^{2} - \tau^{2}.
    \end{eqnarray*}
    This implies
    \begin{eqnarray*}
        \frac{\sqrt{n}c_{3}}{2(n+2\lambda_{3})} &\geq& \frac{\left[ \sqrt{2} n/\tau^{2} \cdot \nu_{p} + o\left( n\nu_{p}/\tau^{2} \right) \right] \| z + \tau x_{1} \|^{2} - \frac{1}{2} \sqrt{n} \tau^{2} }{n + 2(n/\tau^{2})^{2}/(1+n/\tau^{2}) \cdot \|z+\tau x_{1}\|^{2} } \\
        &=& \frac{\sqrt{2}}{2} \nu_{p} - \frac{\frac{\sqrt{2}}{2} n \nu_{p} + \frac{1}{2} \sqrt{n} \tau^{2} - o\left( n\nu_{p}/\tau^{2} \right) \|z+\tau x_{1}\|^{2} }{n + 2 (n/\tau^{2})^{2}/(1+n/\tau^{2}) \cdot \|z+\tau x_{1}\|^{2}} \\
        &\rightarrow& +\infty \text{ a.s.,} \quad \text{ since } \|z+\tau x_{1}\|^{2}/n \rightarrow 1 \text{ a.s..}
    \end{eqnarray*}
    From continuous mapping theorem and \eqref{eq::probability-first-order-spike}, $P\left( \left. \chi_{n}^{2}(\lambda_{3}) \leq n + \lambda_{3} -c_{3} \right\vert \|z+\tau x_{1}\| \right) \rightarrow 0$ a.s.. Therefore,
    \begin{equation*}
        \frac{a_{n,p}}{(p-1) \left(1+\tau^{2}/n\right)^{-\frac{n}{2}} \exp\left[ \frac{1}{2} \frac{1}{1+n/\tau^{2}} \|z+\tau x_{1}\|^{2} \right]} \rightarrow 1 \text{ a.s..}
    \end{equation*}
    Recall that $b^{*}$ satisfies \eqref{eq2::truncation-choice-first-order-spike}, we have
    \begin{align*}
        & \frac{(b^{*}_{n,p})^{-1} a_{n,p}}{\exp\left[ -\log b_{n,p}^{*} + \frac{1}{2} \nu_{p}^{2} + \frac{1}{2} \frac{1}{1+n/\tau^{2}} \|z+\tau x_{1}\|^{2} - \frac{\tau^{2}}{2} \right]} \rightarrow 1 \text{ a.s.,} \\
        & \text{and } \exp \left[ - \log b_{n,p}^{*} + \frac{1}{2} \nu_{p}^{2} + \frac{1}{2}\frac{1}{1 + n/\tau^{2}} \|z+\tau x_{1}\|^{2} - \frac{\tau^{2}}{2} \right] \rightarrow +\infty \text{ a.s.,}
    \end{align*}
    since $(2\sqrt{2} \sqrt{n} \nu_{p})^{-1} b_{n,p}^{*} \rightarrow 1$ a.s. and $n^{-1} \|z+\tau x_{1}\|^{2} \rightarrow 1$ a.s.. 

    In conclusion of the weak law of triangular arrays (Lemma \ref{lem::WLLN-triangular}), for
    \begin{equation*}
        S_{n,p} = \sum_{i=2}^{p} Y_{p,i} = \sum_{i=2}^{p} \exp \left[\tau \|\tau x_{1} + z\| x_{i,1} - \frac{\tau^{2}}{2} x_{i,1}^{2} - \frac{\tau^{2}}{2} \|x_{i,-1}\|^{2} \right],
    \end{equation*}
    we have
    \begin{eqnarray*}
        && P\left(\left. \left|\frac{S_{n,p} - a_{n,p}}{b_{n,p}^{*}}\right|>\epsilon \right\vert \|z+\tau x_{1}\| \right) \\
        &\leq& \sum_{i=2}^{p} P\left( \left. |Y_{p,i}|> b_{n,p}^{*} \right\vert \|z+\tau x_{1}\| \right) + (b_{n,p}^{*}\epsilon)^{-2} \sum_{i=2}^{p} \E \left[\left. Y_{p,i}^{2} \mathbbm{1}_{(Y_{p,i}\leq b_{n,p}^{*})}\right\vert \|z + \tau x_{1}\|\right] \\
        &\rightarrow& 0 \text{ a.s.} \quad \text{ since } n^{-1}\|z+\tau x_{1}\|^{2} \rightarrow 1 \text{ a.s.},
    \end{eqnarray*}
    where 

    \begin{equation*}
        a_{n,p} = (p-1) \left(1+\tau^{2}/n\right)^{-\frac{n}{2}} \exp \left( \frac{\|z+\tau x_{1}\|^{2}}{2(1+n/\tau^{2})} \right) \left( 1-P\left[ \left.\chi_{n}^{2}(\lambda_{3}) \leq n+\lambda_{3}-c_{3} \right\vert \|z+\tau x_{1}\| \right] \right),
    \end{equation*}
    and
    \begin{equation*}
        \frac{a_{n,p}}{(p-1) \left(1+\tau^{2}/n\right)^{-\frac{n}{2}} \exp\left[ \frac{1}{2} \frac{1}{1+n/\tau^{2}} \|z+\tau x_{1}\|^{2} \right]} \rightarrow 1 \text{ a.s..}
    \end{equation*}
    By boundedness of probability function, we conclude
    \begin{equation*}
        P\left( \left| \frac{S_{n,p} - a_{n,p}}{b_{n,p}^{*}} \right| > \epsilon \right) = \E P \left( \left. \left| \frac{S_{n,p} - a_{n,p}}{b_{n,p}^{*}} \right| > \epsilon \right\vert \|z+\tau x_{1}\| \right) \rightarrow 0.
    \end{equation*}
    Therefore,
    \begin{equation*}
        \mathcal{A}_{n,p} = \frac{\sum_{i=2}^{p} \exp\left( \|\tau x_{1} + z\| \tau x_{i,1} - \frac{\tau^{2}}{2} x_{i,1}^{2} - \frac{\tau^{2}}{2} \|x_{i,-1}\|^{2} \right)}{(p-1) (1+\frac{\tau^{2}}{n})^{-\frac{n}{2}} \exp\left( \frac{1}{2} \frac{1}{1+n/\tau^{2}} \|z+\tau x_{1}\|^{2} \right) } \overset{p}{\rightarrow} 1.
    \end{equation*}


%%%%%%%%%%%%%%%% bounding the gaussian complexity

 Using the Cauchy-Scharwtz inequality, we have
    \begin{equation*}
        \E \sup_{u \in T(s) } ~ \langle g, u \rangle = \E \max_{\substack{S\subseteq [p] \\ |S|=s}} \sup_{\|u_{S}\|_{2}=1} g_{S}^{T}u_{S} = \E \max_{\substack{S\subseteq [p] \\ |S|=s}} ~ \|g_{S}\|_{2}. 
    \end{equation*}
    $g \sim \calN(0, I_{p})$ implies
    \begin{equation*}
        P \Big( \|g_{S}\|_{2} \geq \sqrt{|S|} + \delta \Big) \leq e^{-\delta^{2}/2}.
    \end{equation*}
    Thus, $(\|g_{S}\|_{2} - \sqrt{|S|})$ is sub-gaussian with sub-gaussian norm 
    \begin{equation*}
        \inf \{ t>0: \E \exp \frac{(\|g_{S}\|_{2}-\sqrt{|S|})^{2}}{t^{2}} \leq 2 \} \leq 2.
    \end{equation*}
    Then by Lemma \ref{lem::max-sub-gaussian}, the maximum of sub-gaussians has the upper bound
    \begin{equation*}
        \E \max_{\substack{S\subseteq [p] \\ |S|=s}} \Big( \|g_{S}\|_{2} - \sqrt{|S|} \Big) \leq C\sqrt{\log \binom{p}{s}} \leq C\sqrt{s \log (ep/s)}.
    \end{equation*}
        Thus,
    \begin{equation*}
        \E \max_{\substack{S\subseteq [p] \\ |S|=s}} ~\|g_{S}\|_{2} \leq C\sqrt{s\log (p/s)} + \sqrt{s} \leq C\sqrt{s\log(p/s)}.
    \end{equation*}



    %%%%%%%%%%%%%%%%%%%%%%%% first order upper bound for sparse minimax: the proximal oracle estimator is close to LASSO
    The following lemma follows Lemma 4.2 in \cite{su2016slope}. They proved it for SLOPE, but the proof method also works for Lasso.
\begin{lemma}\label{lem::close-to-beta-tilde}
    Let $T\subseteq \{1,\ldots, p\}$ be a subset of columns assumed to contain the supports of $\hat{\beta}, \betaO$ and $\beta$, i.e. $T\supseteq \supp(\hat{\beta})\cup \supp(\betaO) \cup \supp(\beta)$. Suppose all the eigenvalues of $X_{T}^{T}X_{T}$ lie in $[1-\delta, 1+\delta]$ for some $\delta<1/2$. Then
    \begin{equation*}
        \|\betaO-\hat{\beta}\|_{2}^{2} \leq \frac{3\delta}{1-2\delta} \|\betaO-\beta\|_{2}^{2}.
    \end{equation*}
\end{lemma}
\begin{proof}
    We first prove that $\betaO$ and $\hat{\beta}$ are close when $X$ is nearly orthogonal, i.e., in the case where $T=\{1,\ldots, p\}$. By definition $\hat{\beta}$ and $\betaO$ are the minimizer of the following loss functions respectively
    \begin{align*}
        & L_{1}(b) := \frac{1}{2}\|X(\beta - b)\|^{2} + z^{T}X(\beta-b) + \lambda \|b\|_{1}, \\
        & L_{2}(b) := \frac{1}{2} \|\beta - b\|^{2} + z^{T}X(\beta - b) + \lambda \|b\|_{1}.
    \end{align*}
    Then the assumptions about the eigenvalues of $X^{T}X$ implies that these two functions are related
    \begin{align*}
        & L_{2}(\betaO) - \frac{\delta}{2}\|\beta - \betaO\|^{2} \leq L_{1}(\betaO) \leq L_{2}(\betaO) + \frac{\delta}{2}\|\beta - \betaO\|^{2}, \\
        & L_{2}(\hat{\beta}) - \frac{\delta}{2}\|\beta - \hat{\beta}\|^{2} \leq L_{1}(\hat{\beta}) \leq L_{2}(\hat{\beta}) + \frac{\delta}{2}\|\beta - \hat{\beta}\|^{2}.
    \end{align*}
    Chaining these inequalities gives
    \begin{equation}
        L_{2}(\betaO) + \frac{\delta\|\beta-\betaO\|^{2}}{2} \geq L_{1}(\betaO) \geq L_{1}(\hat{\beta}) \geq L_{2}(\hat{\beta}) - \frac{\delta\|\beta - \hat{\beta}\|^{2}}{2}. \label{eq::chain-lasso-prox}
    \end{equation}
    Now the strong convexity of $L_{2}$ also gives
    \begin{equation*}
        L_{2}(\hat{\beta}) \geq L_{2}(\betaO) + \frac{\|\betaO - \hat{\beta}\|^{2}}{2},
    \end{equation*}
    and plugging this in the right-hand side of \eqref{eq::chain-lasso-prox} yields
    \begin{equation*}
        \frac{\|\betaO-\hat{\beta}\|^{2}}{2} - \frac{\delta\|\beta-\hat{\beta}\|^{2}}{2} \leq \frac{\delta\|\beta-\betaO\|^{2}}{2}.
    \end{equation*}
    Since $\delta\|\beta-\hat{\beta}\|^{2}/2\leq\delta \|\betaO - \hat{\beta}\|^{2} + \delta\|\beta-\betaO\|^{2}$ by the basic inequality $(a+b)^{2}\leq 2a^{2}+2b^{2}$, the conclusion follows. 

    We now consider the general case of $T\subseteq \{1,\ldots,p\}$. Let $m$ be the cardinality of $T$ and for $b\in\R^{m}$, and observe that by assumption, $\hat{\beta}_{T}$ and $\betaO_{T}$ are solutions to the reduced problems
    \begin{equation}
        \arg\min_{b\in \R^{|T|}} \frac{1}{2}\|y-X_{T}b\|^{2} +\lambda\|b\|_{1}, \label{eq::lasso-reduced-prob}
    \end{equation}
    and
    \begin{equation*}
        \arg\min_{b\in \R^{|T|}} \frac{1}{2}\|\beta_{T}+X_{T}^{T}z-b\|^{2} +\lambda\|b\|_{1}.
    \end{equation*}
    Using the fact that $X\beta=X_{T}\beta_{T}$, we see that $\hat{\beta}_{T}$ and $\betaO_{T}$ respectively minimize
    \begin{align*}
        & L_{1}(b) := \frac{1}{2}\|X_{T}(\beta_{T} - b)\|^{2} + z^{T}X_{T}(\beta_{T}-b) + \lambda \|b\|_{1}, \\
        & L_{2}(b) := \frac{1}{2} \|\beta_{T} - b\|^{2} + z^{T}X_{T}(\beta_{T} - b) + \lambda \|b\|_{1}.
    \end{align*}
    From now on, the proof is just as before.
\end{proof}

 %%%%%%%%%%%%%%%%%%%%%%%%%%%% first order upper bound for sparse minimax: LASSO achieves the asymptotic first order minimax risk with high probability

 
Throughout this section, we consider the Lasso estimator 
\begin{equation}\label{eq::lasso-estimator}
    \hat{\beta} = \argmin_{b\in\R^{p}}\frac{1}{2}\|y-Xb\|_{2}^{2} + \lambda \|b\|_{1},
\end{equation}
with the choice of 
\begin{equation}
    \lambda = \lambda_{\varepsilon} := (1+\varepsilon)\sqrt{2\log(p/k)}, \label{eq::lambda-epsilon}
\end{equation}
for a given $\varepsilon >0$. Consider the oracle estimator
\begin{equation}\label{eq::oracle-estimator}
    \betaO := \eta_{\lambda}\big(\beta + X^{T}z\big),
\end{equation}
 with the same choice of $\lambda$ as in \eqref{eq::lambda-epsilon}, where 
\begin{equation*}
    \eta_{\lambda}(y):= \argmin_{b\in \R^{p}} \frac{1}{2} \|y-b\|_{2}^{2} + \lambda \|b\|_{1},
\end{equation*}
is the soft thresholding function defined on $y \in \R^{p}$.

\begin{definition}[Resolvent set of Lasso]\label{def::resolvent-set-lasso}
    Fix $S=\supp(\beta)$ of cardinality at most $k$, and an integer $k^{*}$ obeying $k<k^{*}<p$. The set $S_{*}=S_{*}(S,k^{*})$ is said to be a resolvent set if it is the union of $S$ and the $k^{*}-k$ indicies with the largest values of $|X_{i}^{T}z|$ among all $i\in\{1,\ldots, p\}\setminus S$.  
\end{definition}

The following lemma follows Lemma 4.2 in \cite{su2016slope}. They proved it for SLOPE, but the proof method also works for Lasso.
\begin{lemma}\label{lem::close-to-beta-tilde}
    Let $T\subseteq \{1,\ldots, p\}$ be a subset of columns assumed to contain the supports of $\hat{\beta}, \betaO$ and $\beta$, i.e. $T\supseteq \supp(\hat{\beta})\cup \supp(\betaO) \cup \supp(\beta)$. Suppose all the eigenvalues of $X_{T}^{T}X_{T}$ lie in $[1-\delta, 1+\delta]$ for some $\delta<1/2$. Then
    \begin{equation*}
        \|\betaO-\hat{\beta}\|_{2}^{2} \leq \frac{3\delta}{1-2\delta} \|\betaO-\beta\|_{2}^{2}.
    \end{equation*}
\end{lemma}

Let 
\begin{equation}
    S_{\diamond} := \supp(\beta)\cup\supp(\hat{\beta})\cup\supp(\betaO).
\end{equation}


In the following proofs, we introduce an orthogonal matrix $Q\in \R^{n\times n}$ such that
\begin{equation*}
    Qz = \big( \|z\|, 0, \ldots, 0\big).
\end{equation*}
In the proofs, $Q$ can further be set to be measurable with respect to $z$. $Q$ is independent of $X$. Let
\begin{equation*}
    W=\begin{bmatrix}
\tilde{\omega}\\ 
\tilde{W}
\end{bmatrix} := QX,
\end{equation*}
where $\tilde{\omega}\in\R^{1\times p}$ and $\tilde{W}\in\R^{(n-1)\times p}$. $Q$ being independent of $X$ implies that $W$ is still a Gaussian random matrix, with i.i.d. $\calN(0,1/n)$ entries. Note that
\begin{equation}\label{eq::Xz-omega-tilde}
    X_{i}^{T}z = (QX_{i})^{T}(Qz) = \|z\|(QX_{i})_{1} = \|z\|\tilde{\omega}_{i}.
\end{equation}
This implies that $S_{*}$ is constructed as the union of $S$ and $k^{*}-k$ indices in $\{1,\ldots, p\}\setminus S$ with the largest $|\tilde{\omega}_{i}|$. Since $\tilde{\omega}$ and $\Tilde{W}$ are independent, $\Tilde{W}$ and $S_{*}$ are also independent. Thus, $\tilde{W}_{S_{*}^{c}}$ and $\Tilde{W}_{S_{*}}$ are both Gaussian random matrices.

The resolvent set $S_{*}$ was introduced by \cite{su2016slope} to bound the size of the active set of SLOPE. The same choice of $S_{*}$ also works for Lasso here. 

\begin{proof}
        By construction, $\supp(\beta)\subseteq S_{*}$ so we only need to show (\romannum{1}) $\supp(\hat{\beta})\subseteq S_{*}$ and (\romannum{2}) $\supp(\betaO)\subseteq S_{*}$. We begin with (\romannum{1}). By the KKT condition of Lasso, $\supp(\hat{\beta})\subseteq S_{*}$ if 
    \begin{equation*}
        \|X_{S_{*}^{c}}^{T}(y-X_{S_{*}}\hat{\beta}_{S_{*}}) \|_{\infty} \leq \lambda_{\varepsilon},
    \end{equation*}
    which would follow from
    \begin{equation}
        \| X_{S_{*}^{c}}^{T}X_{S_{*}}(\beta_{S_{*}} - \hat{\beta}_{S_{*}}) \|_{\infty} \leq \frac{\varepsilon}{2} \sqrt{2\log(p/k)}, \label{eq::lasso-kkt-1}
    \end{equation}
    and
    \begin{equation}
        \|X_{S_{*}^{c}}^{T}z\|_{\infty} \leq \big(1+\frac{\varepsilon}{2}\big) \sqrt{2\log(p/k)}. \label{eq::lasso-kkt-2}
    \end{equation}

    \textbf{Bound \eqref{eq::lasso-kkt-1}}. In the following proof, let $C$ be a constant that does not dependent on any variable or parameter and whose value may change at each occurrence. Rearrange the objective term as
    \begin{align*}
        &X_{S_{*}^{c}}^{T}X_{S_{*}}(\beta_{S_{*}}-\hat{b}_{S_{*}}) = X_{S_{*}^{c}}^{T}X_{S_{*}}(X_{S_{*}}^{T}X_{S_{*}})^{-1}\big( X_{S_{*}}^{T}(y-X_{S_{*}}\hat{b}_{S_{*}}) - X_{S_{*}}^{T}z\big) \\
        &= X_{S_{*}^{c}}^{T}Q^{T}\underbrace{QX_{S_{*}}(X_{S_{*}}^{T}X_{S_{*}})^{-1} \big (X_{S_{*}}^{T}(y-X_{S_{*}}\hat{b}_{S_{*}}) - X_{S_{*}}^{T}z\big)}_{:=\xi}.
    \end{align*}
    
    We first derive the bound for $\|\xi\|$. Since $\hat{b}_{S_{*}}$ is the solution to the reduced Lasso problem \eqref{eq::lasso-reduced-prob} with $T=S_{*}$, its KKT condition implies that 
    \begin{equation}
        \|X_{S_{*}}(y-X_{S_{*}}\hat{b}_{S_{*}})\|_{\infty} \leq \lambda_{\varepsilon}. \label{eq::S*-KKT}
    \end{equation}
    Lemma \ref{lem::X_S*-singular-values} with $t=1/2$ gives
    \begin{equation*}
        \|X_{S_{*}}(X_{S_{*}}^{T}X_{S_{*}})^{-1}\| \leq \Big( \sqrt{1-1/n} - \sqrt{k^{*}/n} - 1/2 \Big)^{-1} < 2.01 \label{eq::X_S*-operator-norm}
    \end{equation*}
    with probability at least $1-e^{-n/8}$ for sufficiently large $p$, where in the last step we have used $k^{*}/n\rightarrow 0$. 
    
    Hence, from \eqref{eq::S*-KKT} and \eqref{eq::X_S*-operator-norm} we get
    \begin{align}
        \|\xi\| & \leq \|X_{S_{*}}(X_{S_{*}}^{T}X_{S_{*}})^{-1}\| \cdot \|X_{S_{*}}^{T}(y-X_{S_{*}}\hat{b}_{S_{*}}) - X_{S_{*}}^{T}z\| \nonumber\\
        & \leq 2.01 \Big( \sqrt{k^{*}}\lambda_{\varepsilon} + 4\sqrt{2k^{*}\log(p/k^{*})} \Big) \nonumber\\
        & \leq 2.01 \Big((1+\varepsilon)\sqrt{2} + 4\sqrt{2}\Big) \sqrt{k^{*}\log(p/k^{*})} \nonumber\\
        & = C \cdot \sqrt{k^{*}\log(p/k^{*})} \label{eq::xi-2norm-bound}
    \end{align}
    with probability at least 
    \begin{equation*}
        1-e^{-n/2} - (\sqrt{2} ek^{*}/p)^{k^{*}} - e^{-n/8}=: 1- P_{\xi};
    \end{equation*}
    we used Lemma \ref{lem::sup-X^T_S*z} in the second line and $k^{*}\geq k$ in the third.

    Now, write
    \begin{equation}
        X_{S_{*}^{c}}^{T}X_{S_{*}}(\beta_{S_{*}} - \hat{b}_{S_{*}}) = X_{S_{*}^{c}}^{T}Q^{T}\xi = \big(\tilde{\omega}_{S_{*}^{c}}^{T}, 0\big)\xi + \big( 0, \Tilde{W}_{S_{*}^{c}}^{T} \big)\xi. \label{eq::omega-xi-plus-W-xi}
    \end{equation}
    For the first term, we have
    \begin{equation*}
        \|(\tilde{\omega}_{S_{*}^{c}}^{T}, 0)\xi\|_{\infty} = \xi_{1} \cdot \|\tilde{\omega}_{S_{*}^{c}}^{T}\|_{\infty} \leq \|\xi\|_{2} \cdot \|\tilde{\omega}_{S_{*}^{c}}^{T}\|_{\infty}.
    \end{equation*}
    With \eqref{eq::Xz-omega-tilde} and Lemma \ref{lem::Gaussian-order-statistics}, let $|\zeta|_{(i)}$ denote the $i$-th largest among $p-k$ i.i.d. $\calN(0,1)$, we obtain
    \begin{equation}
        \sqrt{n}\|\tilde{\omega}_{S_{*}^{c}}\|_{\infty} = |\zeta|_{(k^{*}-k+1)} \leq (1+\frac{\varepsilon}{4}) \cdot \sqrt{2 \log \frac{2(p-k)}{k^{*}-k+1}} \leq (1+\frac{\varepsilon}{3}) \sqrt{2\log \frac{p}{k}}, \label{eq::omega-tilde-bound}
    \end{equation}
    with probability at least 
    \begin{equation*}
        1- \exp \big[ - c_{1} \varepsilon k \sqrt{2\log(p/k^{*})} \big] =: 1 - P_{1},
    \end{equation*}
    for some constant $c_{1}>0$; we used that $k^{*} \geq 2k$ and $k^{*}-k+1\leq k^{*}$. Thus, from \eqref{eq::xi-2norm-bound} and \eqref{eq::omega-tilde-bound}, we obtain
    \begin{equation*}
        \|(\tilde{\omega}_{S_{*}^{c}}^{T}, 0)\xi\|_{\infty} \leq C \cdot \sqrt{\frac{k^{*}}{n}\log\frac{p}{k^{*}}} \cdot \sqrt{2\log p} \leq C \cdot \sqrt{\frac{k^{*}\log p}{n}} \sqrt{2\log \frac{p}{k}},
    \end{equation*}
    where we have used that $k^{*}\geq k$. For the second term in \eqref{eq::omega-xi-plus-W-xi}, exploiting the independence between $\xi$ and $\Tilde{W}_{S_{*}^{c}}$, we have
    \begin{equation*}
        (0, \Tilde{W}_{S_{*}^{c}}^{T})\xi \overset{d}{=} \sqrt{\frac{\xi_{2}^{2}+\cdots+\xi_{n}^{2}}{n}} (\zeta_{1}, \ldots, \zeta_{p-k^{*}}),
    \end{equation*}
    where $\zeta_{1},\ldots, \zeta_{p-k^{*}}\simiid \calN(0,1)$. By Lemma \ref{lem::Gaussian-maxima}, we have
    \begin{equation}
        |\zeta|_{(1)} \leq C\cdot \sqrt{2\log(p-k^{*})}, \label{eq::tilde-W-gaussian-max-bound}
    \end{equation}
    with probability at least 
    \begin{equation*}
        1- \exp[-c_{2} \log  p] =: 1-P_{2},
    \end{equation*}
    for arbitrary large constant $c_{2}>0$; we used $k^{*}/p \rightarrow 0$. Combing \eqref{eq::xi-2norm-bound} and \eqref{eq::tilde-W-gaussian-max-bound}, we obtain
    \begin{equation*}
        \|(0, \Tilde{W}_{S_{*}^{c}}^{T}) \xi\|_{\infty} \leq \|\xi\|_{2} \frac{1}{\sqrt{n}} |\zeta|_{(1)} \leq C\sqrt{\frac{k^{*}}{n}\log \frac{p}{k^{*}}} \sqrt{2\log (p-k^{*})} \leq C\sqrt{\frac{k^{*}\log p}{n}} \sqrt{2\log \frac{p}{k}}.
    \end{equation*}
    Therefore, 
    \begin{equation}
        \|X_{S_{*}^{c}}^{T}X_{S_{*}}(\beta_{S_{*}} - \hat{\beta}_{S_{*}})\|_{\infty} \leq \|(\Tilde{\omega}_{S_{*}^{c}}^{T}, 0)\xi\|_{\infty} + \|(0, \Tilde{W}_{S_{*}^{c}}^{T})\xi\|_{\infty} \leq C\sqrt{\frac{k^{*}\log p}{n}} \sqrt{2\log (p/k)}, \label{eq::XTX(betahat-beta)-inf-bound}
    \end{equation}
    with probability at least $1-P_{\xi} - P_{1}- P_{2}$ combing event \eqref{eq::xi-2norm-bound}, \eqref{eq::omega-tilde-bound} and \eqref{eq::tilde-W-gaussian-max-bound}.

    \textbf{Bound \eqref{eq::lasso-kkt-2}}. By \eqref{eq::Xz-omega-tilde}, under event \eqref{eq::tilde-W-gaussian-max-bound} and $\|z\|_{2}/\sqrt{n} \leq (1+\varepsilon/3)$, we have that
    \begin{equation}
        \|X_{S_{*}^{c}}^{T}z\|_{\infty} = \frac{\|z\|_{2}}{\sqrt{n}} |\zeta|_{(k^{*}-k+1)} \leq (1+\frac{\varepsilon}{3}) \sqrt{2\log \frac{2(p-k)}{k^{*}-k+1}} \cdot (1+\frac{\varepsilon}{3}) \leq (1+\frac{\varepsilon}{2}) \sqrt{2\log \frac{p}{k}} \label{eq::Xz-inf-bound}
    \end{equation}
    holds with probability at least $1 - P_{z} - P_{\xi}$ where
    \begin{equation*}
        P(\|z\|_{2}/\sqrt{n} \geq 1 + \varepsilon/3) \leq e^{-n\varepsilon^{2}/18} := P_{z}.
    \end{equation*} 

    \textbf{Show (\romannum{2})}. Finally, a sufficient condition that $\supp(\betaO) \subseteq S_{*}$ is 
    \begin{equation}
        \|X_{S_{*}^{c}}^{T}z\|_{\infty} \leq \lambda_{\varepsilon}. \label{eq::supp-beta-tilde}
    \end{equation}
    This holds under event \eqref{eq::Xz-inf-bound}. 

    In combination of \eqref{eq::XTX(betahat-beta)-inf-bound}, \eqref{eq::Xz-inf-bound} and \eqref{eq::supp-beta-tilde}, we have $\supp(\hat{\beta}) \subseteq S_{*}$ holds with probability at least
    \begin{equation*}
        1- P_{\xi} - P_{1} - P_{2} - P_{z} = 1 - \exp\big[ -c_{1}\varepsilon k\sqrt{2\log(p/k^{*})} \big] - \exp \big[-c_{2}\log p\big] - c_{3}e^{-c_{4}n\varepsilon^{2}},
    \end{equation*}
    for some constants $c_{1},c_{2},c_{3},c_{4}>0$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% first order upper bound for sparse minimax: the MSE bound for Lasso

Now, let $X \in \R^{n\times p}$ be the Gaussian random design $X=\frac{1}{n}(x_{1}^{T},\ldots, x_{n}^{T})^{T}$ with $x_{i}\simiid \calN(0,I_{p})$. Fix $\delta_{2},\delta_{3}, \delta_{4}$ satisfying the condition in Lemma \ref{lem::lasso-l2-bound}. Let $c_{0}=c_{0}(\delta_{2},\delta_{3},\delta_{4})$ be defined by \eqref{eq::c_0} and denote
\begin{equation}\label{eq::event-E}
    E := \bigg\{ X\in\R^{n\times p}: ~\max_{j=1,\ldots, p} \|Xe_{j}\|_{2}^{2} \leq 1+\delta_{4}, ~ \inf_{\delta\in\mathcal{C}_{SRE}(k,c_{0}):\delta\neq 0}\frac{\|X\delta\|_{2}}{\|\delta_{2}\|_{2}} \geq \sqrt{1-\delta_{4}} \bigg\}.
\end{equation}

\begin{proposition}\label{prop::lasso-MSE-bound}
    Assume model \eqref{model::gaussian-model} and $\varepsilon>0$. Let $\hat{\beta}$ be the Lasso estimator defined in \eqref{eq::lasso-estimator} with tuning parameter $\lambda_{\varepsilon}$ in \eqref{eq::lambda-epsilon}. Let $E$ be in \eqref{eq::event-E} with $\delta_{2}, \delta_{3}, \delta_{4} >0$ such that $\sqrt{1+\delta_{4}}(1+\delta_{3})(1+\delta_{2}) < 1+\varepsilon$. Then for $q>2$, we have
    \begin{equation*}
        \E \Big[ \|\hat{\beta}-\beta\|_{2}^{q} ~ \mathbbm{1}_{E}\Big] \leq \bigg( \frac{\sqrt{1+\delta_{4}}(1+\delta_{3})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} + 1 \bigg)^{q} \Big(\frac{\lambda_{\varepsilon}\sqrt{k}}{\delta_{3}^{2}}\Big)^{q} \Big[\frac{1}{ (1-\delta_{4})^{q} } + \frac{C_{q}}{(\delta_{3}^{2}k\log(p/k))^{q}}\Big].
    \end{equation*}
\end{proposition}

\begin{proof}
Lemma \ref{lem::lasso-MSE-bound} constructed an uniform upper bound for the conditional expectation $\E \Big(\|\hat{\beta}-\beta\|_{2}^{q} ~|X\Big)$ for all $X\in E$. Using tower property, we obtain
\begin{align*}
    & \E \Big[ \|\hat{\beta}-\beta\|_{2}^{q} ~ \mathbbm{1}_{E}\Big] =   \E \bigg[ \E \Big(\|\hat{\beta}-\beta\|_{2}^{q} ~|X\Big)\mathbbm{1}_{E} \bigg] \\
    & \leq \bigg( \frac{\sqrt{1+\delta_{4}}(1+\delta_{3})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} + 1 \bigg)^{q} \Big(\frac{\lambda_{\varepsilon}\sqrt{k}}{\delta_{3}^{2}}\Big)^{q} \Big[\frac{1}{ (1-\delta_{4})^{q} } + \frac{C_{q}}{(\delta_{3}^{2}k\log(p/k))^{q}}\Big].
\end{align*}
\end{proof}



%%%%%%%%%%%%%%%%%%%% first order upper bound for sparse minimax: MSE bound for lasso
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Prove that max \|Xe_{j}\| \leq 1+\delta, strong restricted eigenvalue \geq \sqrt{1-\delta} with high probability
  In this proof, we denote by $C_{i}$ absolute positive constants. If $v \in \mathcal{C}_{SRE}(k,c_{0})$, i.e. $\|v\|_{1} \leq (1+c_{0})\sqrt{k}\|v\|_{2}$ implies that $\sum_{j=k+1}^{p} |v|_{(j)} \leq (1+c_{0}) \sqrt{k} \|v\|_{2}$, thus
    \begin{align*}
        \sum_{j=k+1}^{p} |v|_{(j)} \sqrt{\log(2p/j)} & \leq \sqrt{\log(2p/k)} \sum_{j=k+1}^{p} |v|_{(j)} \leq (1+c_{0}) \|v\|_{2} \sqrt{k\log(2p/k)} \\
        & \leq (1+c_{0}) \|v\|_{2} \sqrt{\sum_{j=1}^{k} \log(2p/j)},
    \end{align*}
    where the last inequality follows from \eqref{eq::stirling}. For the first $k$ components, the Cauchy-Schwarz inequality yields 
    \begin{equation*}
        \sum_{j=1}^{k} |v|_{(j)} \sqrt{\log(2p/j)} \leq \|v\|_{2} \sqrt{\sum_{j=1}^{k} \log(2p/j)}.
    \end{equation*}
    Using \eqref{eq::stirling} again, we have $\sum_{j=1}^{p}|v|_{(j)} \sqrt{\log(2p/j)} \leq (1+c_{0})\sqrt{k\log(2ep/k)}$. Thus, $\mathcal{C}_{SRE}(k,c_{0})\cap \{v\in\R^{p}: \|v\|_{2}=1\} \subseteq T$ where
    \begin{equation*}
        T := \bigg\{ v\in\R^{p}: \sum_{j=1}^{p} |v|_{(j)} \sqrt{\log(2p/j)} \leq r, \|v\|_{2}=1 \bigg\} \text{ and } r = (1+c_{0}) \sqrt{k\log(2ep/k)}.
    \end{equation*}
    It follows from Theorem 1.12 in \cite{mendelson2016upper} that for all $u>0$, with probability at least $1-2\exp\Big( -C_{2}\min(u^{2}, u\sqrt{n}) \Big)$
    \begin{equation}\label{eq::x-concentration}
        \sup_{v\in T} \bigg| \frac{1}{n}\sum_{i=1}^{n}(v^{T}x_{i})^{2} - \E \Big[ (v^{T}x)^{2} \Big] \bigg| \leq C_{1} \bigg( \frac{\gamma}{\sqrt{n}} + \frac{\gamma^{2}}{n} + \frac{u}{\sqrt{n}} \bigg),
    \end{equation}
    where $\gamma = \E[\sup_{v\in T} G_{v}]$ and $(G_{v})_{v\in T}$ is a centered Gaussian process indexed by $T$ with covariance structure given by $\E[G_{v}G_{u}] = v^{T}u$ for all $u,v\in T$. For instance, one can take $G_{v} = v^{T}\zeta$ for $v\in T$, where $\zeta\sim \calN(0,I_{p})$. Then, $\gamma = \E \sup_{v\in T}v^{T}\zeta$. 

    By \eqref{eq::x-concentration}, if we take $u= \delta_{4}\sqrt{n}/(3C_{1})$ and if the number of observations $n$ satisfies $n\geq \bigg(
    \frac{C_{1}}{3\delta_{4}}\vee \Big(\frac{C_{1}}{3\delta_{4}}\Big)^{2}\bigg)\gamma^{2}$, then with probability at least $1-2\exp\Big( -C_{3}\delta_{4}^{2} n \Big)$,
    \begin{equation*}
        1-\delta_{4} \leq \frac{1}{n}\sum_{i=1}^{n} (v^{T}x_{i})^{2} \leq 1+\delta_{4}, \quad \forall v\in T.
    \end{equation*}
    Following Lemma G.1 and \eqref{eq::x-concentration} that if $n\geq \bigg(
    \frac{C_{4}}{\delta_{4}}\vee \Big(\frac{C_{4}}{\delta_{4}}\Big)^{2}\bigg)r^{2}$ then with probability at least $1-2\exp\Big( -C_{5} \delta_{4}^{2}n\Big)$, we have $1-\delta_{4} \leq \|Xv\|_{2}^{2} \leq 1+\delta_{4}$ for any $v\in T$. By rescaling, for any $v\in C_{SRE}(k,c_{0})$ we obtain $\|Xv\|_{2}^{2} \geq (1-\delta_{4})\|v\|_{2}^{2}$. This proves that the second inequality in \eqref{eq::random-matrix-SRE-condition} is satisfied if $n\geq  \bigg(
    \frac{C_{4}}{\delta_{4}}\vee \Big(\frac{C_{4}}{\delta_{4}}\Big)^{2}\bigg)r^{2}$.


    By Lemma \ref{lem::gaussian-matrix-satisfy-SRE}, Gaussian random matrix satisfies an enlargement of the column constraint, i.e. with high probability,
\begin{equation}\label{eq::gaussian-column-constraint}
    \max_{j=1,\ldots, p}\|Xe_{j}\|_{2} \leq \sqrt{1+\delta_{0}}.
\end{equation}
Assume $X\in\R^{n\times p}$ is fixed satisfying \eqref{eq::gaussian-column-constraint}, rescaling the result in Lemma \ref{lem::bound-on-stochastic-error} leads to
\begin{equation}\label{eq::modified-stochastic-error-event}
    z^{T}Xu \leq \sqrt{1+\delta_{0}} \max \Big(H(u),G(u)\Big), ~ \forall u\in\R^{p}
\end{equation}
with probability at least $1-\deltanum{delta::5}/2$.





\subsection{Proof of Theorem \ref{thm::first-order-upper-bound}}
Let $\betaO$ be the oracle estimator defined in \eqref{eq::oracle-estimator} and $\betaL$ be the Lasso estimator defined in \eqref{eq::lasso-estimator}, with $\lambda$ set by \eqref{eq::lambda-epsilon}. In addition, let $\hat{\beta}^{MLE}$ denote the MLE defined in \eqref{eq::MLE}. Let
\begin{equation}\label{eq::event-A}
    \mathcal{A} := E_{\delta_{0}} = \bigg\{ X\in\R^{n\times p}: ~\max_{j=1,\ldots, p} \|Xe_{j}\|_{2}^{2} \leq 1+\delta_{0}, ~ \inf_{\delta\in\mathcal{C}_{SRE}(k,c_{0}):\delta\neq 0}\frac{\|X\delta\|_{2}}{\|\delta_{2}\|_{2}} \geq \sqrt{1-\delta_{0}} \bigg\},
\end{equation}
where $E_{\delta_{0}} = E$ is the event defined in \eqref{eq::event-E}, with $0<\delta_{0}<\varepsilon$ to be determined. Define the estimator
\begin{equation}\label{eq::beta-double-hat-estimator}
    \hat{\hat{\beta}} := \betaL \mathbbm{1}_{\mathcal{A}} + \hat{\beta}^{MLE}\mathbbm{1}_{\bar{\mathcal{A}}}.
\end{equation}
Let $0 < \delta < 1/2$ be a small number to be set later and
\begin{align}\label{eq::event-B}
    \mathcal{B} = \mathcal{B}_{\delta} := \bigg\{ & \supp(\betaL)\cup\supp(\betaO)\cup\supp(\beta) \subseteq S_{*}, \nonumber \\
    & \text{all eigenvalues of }X_{S_{*}}^{T}X_{S_{*}} \text{ lie in } [1-\delta, 1+\delta] , \nonumber \\
    & \|z\|_{2} \leq (1+\varepsilon)/\sqrt{n} \bigg\},
\end{align}
where $S_{*}$ is the resolvent set of Lasso in Definition \ref{def::resolvent-set-lasso}. 

\begin{theorem}\label{thm::first-order-upper-bound}
Assume model \eqref{model::gaussian-model}. Given $\forall \tilde{\varepsilon}>0$ and $0<\delta_{0}<\varepsilon<\tilde{\varepsilon}$, let $\hat{\hat{\beta}}$ be the estimator in \eqref{eq::beta-double-hat-estimator} with event $\mathcal{A}$ and $\mathcal{B}$ defined in \eqref{eq::event-A} and \eqref{eq::event-B} respectively. The tuning parameter is chosen as in \eqref{eq::lambda-epsilon}. Then 
\begin{equation*}
    \E \|\hat{\hat{\beta}} - \beta\|^{2} \leq (1+\tilde{\varepsilon})^{2} 2 k\log(p/k).
\end{equation*}
\end{theorem}

\begin{proof}
In this proof, we assume that $\varepsilon, \delta, \delta_{1}$ are given arbitrary small positive numbers. Let $q, r > 2$, then
\begin{subequations}\label{eq::beta-double-hat-l2-decomp}
    \begin{align}
    \E \|\hat{\hat{\beta}} - \beta\|^{2} & = \E \|\betaL - \beta\|^{2} \mathbbm{1}_{\mathcal{A}} + \E \|\hat{\beta}^{MLE} - \beta\|^{2} \mathbbm{1}_{\bar{\mathcal{A}}} \nonumber\\
    & = \E \|\betaO - \beta\|^{2}\mathbbm{1}_{\mathcal{A}\cap \mathcal{B}} + 2\E (\betaL - \betaO)^{T}(\betaO - \beta)\mathbbm{1}_{\mathcal{A}\cap \mathcal{B}} + \E \|\betaL - \betaO\|^{2}\mathbbm{1}_{\mathcal{A} \cap \mathcal{B} } \nonumber\\
    & + \E \| \betaL - \beta \|^{2}\mathbbm{1}_{ \mathcal{A} \cap \bar{\mathcal{B}} } + \E \| \hat{\beta}^{MLE} - \beta \|^{2}\mathbbm{1}_{\Bar{\mathcal{A}}} \nonumber\\
    & \leq \E \| \betaO - \beta \|^{2} \mathbbm{1}_{ \mathcal{A}\cap\mathcal{B} } + 2\sqrt{\E\| \betaL - \betaO \|^{2} \mathbbm{1}_{ \mathcal{A} \cap \mathcal{B}}} \cdot \sqrt{ \E \| \betaO - \beta \|^{2} \mathbbm{1}_{ \mathcal{A} \cap \mathcal{B} } } + \E \| \betaL - \betaO \|^{2} \mathbbm{1}_{ \mathcal{A} \cap \mathcal{B}}  \nonumber\\
    & + \Big( \E \| \betaL - \beta \|^{q} \mathbbm{1}_{\mathcal{A}} \Big)^{\frac{2}{q}} P(\Bar{\mathcal{B}}) + \Big( \E \| \hat{\beta}^{MLE} - \beta \|^{r} \Big)^{\frac{2}{r}} P( \bar{\mathcal{A}} ).
\end{align}
\end{subequations}


We will show that only the first term in \eqref{eq::beta-double-hat-l2-decomp} dominates and the remainings are higher order terms. For the first term, under $\mathcal{B}$, $\|z\| \leq (1+\varepsilon)\sqrt{n}$. Conditional on $\|z\| = c\sqrt{n}$ for some $0<c\leq 1+\varepsilon$, $X^{T}z\sim \calN(0, c^{2}I_{p})$ and conditionally
\begin{equation*}
    \| \eta_{\lambda_{\varepsilon}}(\beta+X^{T}z) - \beta \| \overset{d}{=} c\| \eta_{\lambda_{\varepsilon'}}(\beta/c + \calN(0,I_{p})) - \beta/c \|
\end{equation*}
for $\varepsilon' = (1+\varepsilon)/c - 1\geq 0$. Hence, the MSE upper bound of Lasso under orthogonal design (for instance, Theorem 1 in \cite{guo2022signal}) gives, for arbitrarily small $\delta_{1}>0$,
\begin{align*}
    \E\bigg[ \|\betaO - \beta \|^{2} \mathbbm{1}_{\mathcal{B}} \bigg] &  \leq \E \bigg[ \frac{\|z\|^{2}}{n} \E \Big( \| \eta_{\varepsilon'} \big( \beta/c + \calN(0,I_{p}) \big) - \beta/c \|^{2} ~\Big| \|z\|=c\sqrt{n} \Big) \mathbbm{1}_{\{\|z\|\leq(1+\varepsilon)\sqrt{n}\}} \bigg] \nonumber\\
    & \leq \E \bigg[ \frac{\|z\|^{2}}{n} (1+\delta_{1}) 2(1+\varepsilon')^{2}k\log(p/k) \mathbbm{1}_{\{\|z\|\leq(1+\varepsilon)\sqrt{n}\}} \bigg] \nonumber\\
    & \leq 2(1+\delta_{1})(1+\varepsilon)^{2}k\log(p/k), \nonumber
\end{align*}
where the last inequality is due to $(1+\varepsilon)^{2}/c^{2} = (1+\varepsilon')^{2}$.

For the second and the third terms, from Lemma \ref{lem::close-to-beta-tilde},
\begin{equation*}
    \E\|\betaL - \betaO \|^{2} \mathbbm{1}_{ \mathcal{A} \cap \mathcal{B}} \leq \frac{3\delta}{1-2\delta} \E \| \betaO -\beta \|^{2} \mathbbm{1}_{ \mathcal{B} }.
\end{equation*}
For the fourth term, by Proposition \ref{prop::lasso-MSE-bound},
\begin{align*}
    & \Big( \E \| \betaL - \beta \|^{q} \mathbbm{1}_{\mathcal{A}} \Big)^{\frac{2}{q}} P(\Bar{\mathcal{B}}) \\
    \leq  & \bigg( \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} + 1 \bigg)^{2} \Big(\frac{\lambda_{\varepsilon}\sqrt{k}}{\deltanum{delta::4}^{2}}\Big)^{2} \Big[\frac{1}{ (1-\delta_{0})^{2} } + \frac{C_{q}^{2/q}}{(\deltanum{delta::4}^{2}k\log(p/k))^{2}}\Big] \cdot P(\bar{\mathcal{B}}).
\end{align*}
Given $\varepsilon, \delta_{0}, \deltanum{delta::4}$ and note that
\begin{equation*}
    P\Big( \|z\|\leq (1+\varepsilon)\sqrt{n} \Big) \geq 1 - e^{-\varepsilon^{2}n/2}.
\end{equation*}
Combined with Proposition \ref{prop::lasso-conditions-hold}, there exist $k,n,p$ such that $P(\bar{\mathcal{B}})$ is small enough such that
\begin{equation*}
    \Big( \E \| \betaL - \beta \|^{q} \mathbbm{1}_{\mathcal{A}} \Big)^{\frac{2}{q}} P(\Bar{\mathcal{B}}) \leq \delta_{1} (\lambda_{\varepsilon} \sqrt{k})^{2}  = \delta_{1} (1+\varepsilon)^{2} 2k\log(p/k).
\end{equation*}
For the last term, based on Proposition \ref{prop::MLE-bound} and Lemma \ref{lem::gaussian-matrix-satisfy-SRE}, for arbitrary small $\delta_{1},\varepsilon >0$, we have
\begin{equation*}
    \Big( \E \| \hat{\beta}^{MLE} - \beta \|^{r} \Big)^{\frac{2}{r}} P( \bar{\mathcal{A}} ) \leq \delta_{1} (1+\varepsilon)^{2} 2k\log(p/k).
\end{equation*}
\end{proof}





%%%%%%%%%%%%%%%%% reference

% @article{zhang2012minimax,
%   title={Minimax $\ell_q$ risk in $\ell_p$ balls},
%   author={Zhang, Cun-Hui},
%   journal={Contemporary Developments in Bayesian Analysis and Statistical Decision Theory: A Festschrift for William E. Strawderman},
%   pages={78},
%   year={2012}
% }


% @article{collier2017minimax,
%   title={Minimax estimation of linear and quadratic functionals on sparsity classes},
%   author={Collier, Olivier and Comminges, La{\"e}titia and Tsybakov, Alexandre B},
%   journal={The Annals of Statistics},
%   volume={45},
%   number={3},
%   pages={923--958},
%   year={2017},
%   publisher={Institute of Mathematical Statistics}
% }

% @article{butucea2018variable,
%   title={Variable selection with Hamming loss},
%   author={Butucea, Cristina and Ndaoud, Mohamed and Stepanova, Natalia A and Tsybakov, Alexandre B},
%   journal={The Annals of Statistics},
%   volume={46},
%   number={5},
%   pages={1837--1875},
%   year={2018},
%   publisher={Institute of Mathematical Statistics}
% }


% @article{donoho1994minimax,
%   title={Minimax risk over $\ell_p$ balls for $\ell_q$ losses},
%   author={Donoho, DL and Johnstone, IM},
%   journal={Probab. Theory Related Fields},
%   volume={99},
%   pages={277--303},
%   year={1994}
% }

% @book{le1986asymptotic,
%   title={Asymptotic methods in statistical decision theory},
%   author={Le Cam, Lucien},
%   year={1986},
%   publisher={Springer Science \& Business Media}
% }


% @book{lehmann1998theory,
%   title={Theory of point estimation},
%   author={Lehmann, Erich L and Casella, George},
%   year={1998},
%   publisher={Springer Science \& Business Media}
% }


% @article{zhang2016minimax,
%   title={Minimax rates of community detection in stochastic block models},
%   author={Zhang, Anderson Y and Zhou, Harrison H},
%   journal={The Annals of Statistics},
%   volume={44},
%   number={5},
%   pages={2252--2280},
%   year={2016},
%   publisher={Institute of Mathematical Statistics}
% }

% @article{loffler2021optimality,
%   title={Optimality of spectral clustering in the Gaussian mixture model},
%   author={L{\"o}ffler, Matthias and Zhang, Anderson Y and Zhou, Harrison H},
%   journal={The Annals of Statistics},
%   volume={49},
%   number={5},
%   pages={2506--2530},
%   year={2021},
%   publisher={Institute of Mathematical Statistics}
% }

% @article{cai2021transfer,
%   title={Transfer learning for nonparametric classification: Minimax rate and adaptive classifier},
%   author={Cai, T Tony and Wei, Hongji},
%   journal={The Annals of Statistics},
%   volume={49},
%   number={1},
%   pages={100--128},
%   year={2021},
%   publisher={Institute of Mathematical Statistics}
% }


% @book{wainwright2019high,
%   title={High-dimensional statistics: A non-asymptotic viewpoint},
%   author={Wainwright, Martin J},
%   volume={48},
%   year={2019},
%   publisher={Cambridge University Press}
% }

% @book{buhlmann2011statistics,
%   title={Statistics for high-dimensional data: methods, theory and applications},
%   author={B{\"u}hlmann, Peter and Van De Geer, Sara},
%   year={2011},
%   publisher={Springer Science \& Business Media}
% }

% @book{fan2020statistical,
%   title={Statistical foundations of data science},
%   author={Fan, Jianqing and Li, Runze and Zhang, Cun-Hui and Zou, Hui},
%   year={2020},
%   publisher={Chapman and Hall/CRC}
% }
% @book{Tsybakov:2008:INE:1522486,
%  author = {Tsybakov, Alexandre B.},
%  title = {Introduction to Nonparametric Estimation},
%  year = {2008},
%  isbn = {0387790519, 9780387790510},
%  edition = {1st},
%  publisher = {Springer Publishing Company, Incorporated},
% } 

% @book{gine2021mathematical,
%   title={Mathematical foundations of infinite-dimensional statistical models},
%   author={Gin{\'e}, Evarist and Nickl, Richard},
%   year={2021},
%   publisher={Cambridge university press}
% }

% @article{zou2005regularization,
%   title={Regularization and variable selection via the elastic net},
%   author={Zou, Hui and Hastie, Trevor},
%   journal={Journal of the royal statistical society: series B (statistical methodology)},
%   volume={67},
%   number={2},
%   pages={301--320},
%   year={2005},
%   publisher={Wiley Online Library}
% }

% @book{hastie2009elements,
%   title={The elements of statistical learning: data mining, inference, and prediction},
%   author={Hastie, Trevor and Tibshirani, Robert and Friedman, Jerome H and Friedman, Jerome H},
%   volume={2},
%   year={2009},
%   publisher={Springer}
% }


% @article{hazimeh2020fast,
%   title={Fast best subset selection: Coordinate descent and local combinatorial optimization algorithms},
%   author={Hazimeh, Hussein and Mazumder, Rahul},
%   journal={Operations Research},
%   volume={68},
%   number={5},
%   pages={1517--1537},
%   year={2020},
%   publisher={INFORMS}
% }

% @article{mazumder2022subset,
%   title={Subset selection with shrinkage: Sparse linear modeling when the SNR is low},
%   author={Mazumder, Rahul and Radchenko, Peter and Dedieu, Antoine},
%   journal={Operations Research},
%   year={2022},
%   publisher={INFORMS}
% }

% @article{zheng2017does,
%   title={Does $\ell_p$-Minimization Outperform $\ell_1$-Minimization?},
%   author={Zheng, Le and Maleki, Arian and Weng, Haolei and Wang, Xiaodong and Long, Teng},
%   journal={IEEE Transactions on Information Theory},
%   volume={63},
%   number={11},
%   pages={6896--6935},
%   year={2017},
%   publisher={IEEE}
% }

% @article{weng2018overcoming,
%   title={Overcoming the limitations of phase transition by higher order analysis of regularization techniques},
%   author={Weng, Haolei and Maleki, Arian and Zheng, Le},
%   journal={The Annals of Statistics},
%   volume={46},
%   number={6A},
%   pages={3099--3129},
%   year={2018},
%   publisher={Institute of Mathematical Statistics}
% }


% @book{besse1978manifolds,
%   title={Manifolds all of whose geodesics are closed},
%   author={Besse, Arthur L},
%   volume={93},
%   year={1978},
%   publisher={Springer Science \& Business Media}
% }

% @article{bianco2004robust,
%   title={Robust estimators in semiparametric partly linear regression models},
%   author={Bianco, Ana and Boente, Graciela},
%   journal={Journal of Statistical Planning and Inference},
%   volume={122},
%   number={1-2},
%   pages={229--252},
%   year={2004},
%   publisher={Elsevier}
% }


==> proof_thm2_upper_bound.tex <==
\section{Proof of upper bound in Theorem \ref{thm::first-order-sparse-minimax}}


As we discussed in Section \ref{sec::lower_bound}, using the scale invariance property \ref{sec:scaling} of the minimax risk, it's sufficient to prove Theorem \ref{thm::first-order-sparse-minimax} for $\sigma=1$. Throughout the proof, for notational simplicity, everytime we use constant notation $C>0$, we mean it is a constant that does not depend on any variable or parameter, but whose value may change at each occurrence. For $X\in \R^{n\times p}$, let $i\in\{1,\ldots,p\}$ and $X_{i}$ stand for the $i$-th column of $X$; let $T\subseteq[p]$ and $X_{T}$ stand for the submatirx consists of the columns with indices contained in $T$.

\subsection{Proof of upper bound in Theorem \ref{thm::first-order-sparse-minimax}}

\subsubsection{Roadmap of the proof}
Obtaining constant-sharp upper bounds for the minimax risk of the sparse linear regression is quite challenging and for that reason it has remained open, despite the existing extensive literature on the topic. The main idea is to consider a good estimator such as LASSO or subset selection and obtain an upper bound for the risk of that estimate, defined below and obtain an upper bound for the risk of those estimates. 
\begin{itemize}
\item LASSO: 
\begin{equation}\label{eq::lasso-estimator0}
    \betaL(\lambda) := \argmin_{b\in\R^{p}}\frac{1}{2}\|y-Xb\|_{2}^{2} + \lambda \|b\|_{1}.
\end{equation}


\item Maximum likelihood estimator:
\begin{equation}\label{eq::MLE0}
    \betaM := \argmin_{b\in \Theta(k)} \|y-Xb\|_{2}^{2}.
\end{equation}
\end{itemize}
However, the main reason the problem has remained open is the following: when bounding the risk of the LASSO the size of the active set of $\betaL(\lambda)$ can impact the upper bounds of the risk. While we can guarantee that the size is with high probability small, but controlling the risk on the low-probability event that the active set is large compared to $n$, seems to be very challenging. Hence, it is difficult to obtain an upper bound with the sharp constants for the risk of LASSO. 

On the other hand, for the variable selection method we have an accurate bound on the number of nonzeros in $\hat{\beta}^M$. \textcolor{red}{We should provide an explanation why we cannot get a good bound here either. }  

Hence, to obtain an upper bound matching the lower bound  we construct an estimator that combines the maximum likelihood estimator and LASSO. Our estimator is defined as 
\begin{equation}\label{eq::beta-double-hat-estimator}
    \hat{\hat{\beta}} := \betaL \mathbbm{1}_{\mathcal{A}} + \betaM \mathbbm{1}_{\mathcal{A}^{c}}.
\end{equation}
where $\mathcal{A}$ is defined as: \textcolor{red}{A is a function of $c_0 and k$ too and later they will become important. }
\begin{equation}\label{eq::event-A}
    \mathcal{A}:=\mathcal{A}(\delta_{0}) := \bigg\{ X\in\R^{n\times p}: ~\max_{j=1,\ldots, p} \|Xe_{j}\|_{2}^{2} \leq 1+\delta_{0}, ~ \inf_{\Delta\in\mathcal{C}_{SRE}(k,c_{0}):\Delta\neq 0}\frac{\|X\Delta\|_{2}}{\|\Delta\|_{2}} \geq \sqrt{1-\delta_{0}} \bigg\},
\end{equation}
where $0<\delta_{0}$ is a constant that will be determined later, and \begin{equation*}
\mathcal{C}_{SRE}(k,c_{0}):=\{\Delta\in\R^{p}: ~\|\Delta\|_{1}\leq(1+c_{0})\sqrt{k}\|\Delta\|_{2}\},
\end{equation*}
with $c_{0}$ determined later in the proof. \textcolor{red}{We have to describe carefully, why this estimator makes sense so that people can understand our argument. }

We should emphasize that the LASSO estimate depends on the regularization parameter $\lambda>0$. Our choice of $\lambda$ for this proof will be discussed later. For notational simplicity, throughout the proof, we will usually use the notation $\betaL(\lambda)=:\betaL$, but we will carefully discuss the choice of $\lambda$ later in the proof. Our goal is to show that for a good choice of $\lambda$, 
\[
\sup_{\beta \in \Theta(k)} \E \| \hat{\hat{\beta}} - \beta\|_2^2 = 2k \log (p/k)(1+ o(1)).
\]
From the construction of $\betahh$, it is straightforward to show that
\begin{eqnarray} \label{eq::lasso-MLE-decomposition}
    \E \|\hat{\hat{\beta}} - \beta\|^{2} = \E \|\betaL - \beta\|^{2} \mathbbm{1}_{\mathcal{A}} + \E \|\betaM - \beta\|^{2} \mathbbm{1}_{\mathcal{A}^{c}}.
\end{eqnarray}
We will show that
\begin{enumerate}
\item $\E\|\betaM - \beta\|^{2}\mathbbm{1}_{\mathcal{A}^{c}} = o\Big(k\log (p/k)\Big)$;



\item  $\E \|\betaL - \beta\|^{2} \mathbbm{1}_{\mathcal{A}} = 2k\log (p/k) \Big(1+o(1)\Big)$.
\end{enumerate}

\begin{itemize}

\item Proof of $\E\|\betaM - \beta\|^{2}\mathbbm{1}_{\mathcal{A}^{c}} = o\Big(k\log (p/k)\Big)$: First note that from the Cauchy-Schwartz inequality we have:
\begin{eqnarray}\label{eq::cauchy-schwarz-expansion-for-MLE-bound}
\E \| \betaM - \beta\|^2 \leq  \Big( \E \|\betaM - \beta\|_{2}^{r} \Big)^{\frac{2}{r}} P(\mathcal{A}^c). 
\end{eqnarray}
Hence, we will prove that $\Big( \E \|\betaM - \beta\|_{2}^{r} \leq C k \log (\frac{p}{k})$ and that  $P(\mathcal{A}^c)= o(1)$. Let us start with the simpler one, i.e. $P(\mathcal{A}^c)= o(1)$. The following lemma proves this claim. 



The following lemma guarantees that $SRE(s,c_{0})$ holds for Gaussian random matrix with high probability.
\begin{lemma}\label{lem::gaussian-matrix-satisfy-SRE}
    Let $X\in\R^{n\times p}$ have the random Gaussian design with i.i.d. $\calN(0,\frac{1}{n})$ entries. Consider the $SRE(k,c_{0})$ with $c_{0}>0$ and $k\in\{1,\ldots, p\}$. There exist absolute constants $C, C'>0$ such that the following holds. For $\forall \delta_{0}\in(0,1)$, if
    \begin{equation}\label{eq::large-n-SRE-condition}
        n\geq Cc_{0}^{2}\delta_{0}^{-2} k \log(2ep/k)
    \end{equation}
    then with probability at least $1-3\exp\big( -C' n\delta_{0}^{2} \big)$ we have
    \begin{equation}\label{eq::random-matrix-SRE-condition}
        \max_{j=1,\ldots, p} \|Xe_{j}\|^{2} \leq 1+\delta_{0}, \quad \inf_{\Delta\in\mathcal{C}_{SRE}(k,c_{0}): \Delta\neq 0} \frac{\|X\Delta\|_{2}}{\|\Delta\|_{2}} \geq \sqrt{1-\delta_{0}}.
    \end{equation}
\end{lemma}

\begin{proof}
    The statement of the second inequality in \eqref{eq::random-matrix-SRE-condition} follows from the proof of Theorem 8.3 in \cite{bellec2018slope}. Hence, we prove the first inequality of \eqref{eq::random-matrix-SRE-condition} only. Applying a standard concentration result for $\chi^{2}$ RVs (for example, Lemma 1 in \cite{laurent2000adaptive}), we have for some constant $C>0$, with probability at least $1-\exp(-Cn\delta_{0}^{2})$, \textcolor{red}{We are referring to many results from the other papers. This makes the paper unreadable. It is better to copy-paste most of these results and write them in our own notation, so that people do not have to read 10 other papers to understand ours.  }
    \begin{equation*}
        \|Xe_{j}\|_{2}^{2} \leq  1 + \delta_{0}.
    \end{equation*}
    Then using the union bound, we have $\max_{j=1,\ldots, p} \|Xe_{j}\|_{2}^{2} \leq 1+\delta_{0}$ holds with probability at least 
    \begin{equation*}
        1-pe^{-Cn\delta_{0}^{2}}\geq 1 - e^{-Cn\delta_{0}^{2}/2}, 
    \end{equation*}
    if $n\geq C\delta_{0}^{-2}\log p$. Note that $k\log(ep/k)\geq \log p$ for all $ k\in\{ 1,\ldots,p\}$. The conclusion holds for the second inequality in \eqref{eq::random-matrix-SRE-condition}.

    
\end{proof}

The next step is to obtain an upper bound for $\Big( \E \|\betaM - \beta\|_{2}^{r} \Big)^{\frac{2}{r}}$. This is done in the next proposition. 

\begin{proposition}\label{prop::MLE-bound}
    Assume model \eqref{model::gaussian-model} with $\sigma=1$. Suppose $k/p\rightarrow 0$ and $(k\log(p/k))/n \rightarrow 0$. Then, for any fixed $m\geq 2$, there exists a constant $C=C(m)>0$, such that
    \begin{equation*}
        \Big( \E \|\beta - \hat{\beta}^M\|_{2}^{m} \Big)^{\frac{2}{m}} \leq C k \log (p/k).
    \end{equation*}
\end{proposition}

The proof of this proposition is long. \textcolor{red}{We should write a couple of sentences explaining why it is long. } Hence, the proof is postponed to Section \ref{prop::MLE-bound:proof}. 

Combining Lemma \ref{lem::gaussian-matrix-satisfy-SRE} and Proposition \ref{prop::MLE-bound} establishes
$\E\|\betaM - \beta\|^{2}\mathbbm{1}_{\mathcal{A}^{c}} = o\Big(k\log (p/k)\Big)$. 



\item $\E \|\betaL - \beta\|^{2} \mathbbm{1}_{\mathcal{A}} = 2k\log (p/k) \Big(1+o(1)\Big)$: In establishing this bound, the main challenge is that we would like to obtain an upper bound with the sharp constant $2$. The standard bounds for the risk of LASSO are based on  mutual incoherence condition \cite{tropp2006just} and the restricted eigenvalue condition \cite{4839045} and do not offer sharp constants. Hence, inspired by \cite{su2016slope} we resort to the following oracle estimator: 
\begin{equation}\label{eq::oracle-estimator}
    \betaO := \eta_{\lambda}\big(\beta + X^{T}z\big),
\end{equation}
where $\eta_{\lambda}(y):= \argmin_{b\in \R^{p}} \frac{1}{2} \|y-b\|_{2}^{2} + \lambda \|b\|_{1}$ is known as the soft thresholding function. Note that this oracle estimator is using the same value of $\lambda$ as the one the original problem is using. 


The main idea is to show that $E (\|\tilde{\beta}^o- \hat{\beta}^L\|_2^2) = o(k \log (p/k))$, and hence the risk of this oracle estimator is the same as the risk of LASSO. Given $\varepsilon >0$, we set the regularization parameter of LASSO to
\begin{equation}
    \lambda = \lambda_{\varepsilon} := (1+\varepsilon)\sqrt{2\log(p/k)}. \label{eq::lambda-epsilon}
\end{equation} 

Let us start with the problem of obtaining an upper bound for the risk of oracle estimator. Conditional on $\|z\| = c\sqrt{n}$, $X^{T}z\sim \calN(0, c^{2}I_{p})$ and \textcolor{red}{Add a simple lemma}, we can conclude that \textcolor{red}{We need a better notation for these things}
\begin{equation*}
    \| \eta_{\lambda_{\varepsilon}}(\beta+X^{T}z) - \beta \| \overset{d}{=} c\| \eta_{\lambda_{\varepsilon'}}(\beta/c + \calN(0,I_{p})) - \beta/c \|,
\end{equation*}
where $\varepsilon' = (1+\varepsilon)/c - 1\geq 0$.
\textcolor{red}{The next step is to explain accurately how we have found an upper bound for the above term}. The next step would be to integrate the upper bound with respect to the distribution of $c$. However, to simplify the calculations, we use the following trick.
\begin{equation*}
    \mathcal{B}_{1} := \Big\{\|z\|_{2} \leq (1+\varepsilon)/\sqrt{n} \Big\}.
\end{equation*}
\textcolor{red}{Must be explained in a nicer way. } Note that we expect the probability of this event to go to $1$ as $n,p \rightarrow \infty$. Hence, based on Theorem 1 in \cite{guo2022signal}, for arbitrarily small $\defdelta\label{delta::1}>0$, we have
\begin{align}
    \E\bigg[ \|\betaO - \beta \|^{2} \mathbbm{1}_{\mathcal{B}_{1}} \bigg] &  \leq \E \bigg[ \frac{\|z\|^{2}}{n} \E \Big( \| \eta_{\lambda_{\varepsilon'}} \big( \beta/c + \calN(0,I_{p}) \big) - \beta/c \|^{2} ~\Big| \|z\|=c\sqrt{n} \Big) \mathbbm{1}_{\{\|z\|\leq(1+\varepsilon)\sqrt{n}\}} \bigg] \nonumber\\
    & \leq \E \bigg[ \frac{\|z\|^{2}}{n} 2(1+\varepsilon')^{2}k\log(p/k) \cdot (1+\deltanum{delta::1}) \mathbbm{1}_{\{\|z\|\leq(1+\varepsilon)\sqrt{n}\}} \bigg] \nonumber\\
    & \leq  (1+\varepsilon)^{2} (1+\deltanum{delta::1}) \cdot 2k\log(p/k), \label{eq::oracle-dominates}
\end{align}

where the last inequality is due to $(1+\varepsilon)^{2}/c^{2} = (1+\varepsilon')^{2}$. Thus, under $\mathcal{B}_{1}$, we have the MSE of the oracle estimator upper bounded by $2k\log(p/k)\cdot (1+o(1))$, as $\varepsilon,\deltanum{delta::1} \rightarrow 0$. In addition, 
\begin{equation}\label{eq:probB1}
P(\mathcal{B}_1)  \geq 1-\exp(-n\varepsilon^{2}/2). 
\end{equation}
 \textcolor{red}{Again we need proper lemma to cite to get this. }


As we discussed before, the final step of our proof is to show that the difference between $\E\|\tilde{\beta}^o - \hat{\beta}^L\|^2_2 = o(k \log (p/k))$. \textcolor{red}{Some intuition and roadmpa will be helpful. } The next lemma provides the first step:

\begin{lemma}\label{lem::close-to-beta-tilde}
    Let $S_{*}\subseteq \{1,\ldots, p\}$ be a subset of columns assumed to contain the supports of $\betaL, \betaO$ and $\beta$, i.e. $S_{*}\supseteq \supp(\betaL)\cup \supp(\betaO) \cup \supp(\beta)$. Suppose for some $\defdelta\label{delta::2}<1/2$, all the eigenvalues of $X_{S_{*}}^{T}X_{S_{*}}$ lie in $[1-\deltanum{delta::2}, 1+\deltanum{delta::2}]$. Then
    \begin{equation*}
        \|\betaO-\betaL\|_{2}^{2} \leq \frac{3\deltanum{delta::2}}{1-2\deltanum{delta::2}} \|\betaO-\beta\|_{2}^{2}.
    \end{equation*}
\end{lemma}
The proof of this lemma follows the same arguments that were used in the proof of Lemma 4.2 in \cite{su2016slope}. Hence we skip the argument.

\textcolor{red}{Think about it to see what is the best way to present the proof. }


Define the event $\mathcal{B}_{2}:= \mathcal{B}_{2}(\deltanum{delta::2})$, as tbe event that there exists a set $S_*$ such that $\supp(\betaL)\cup\supp(\betaO)\cup\supp(\beta) \subseteq S_{*}$ and that all the eigenvalues $X_{S_{*}}^{T}X_{S_{*}}$ lie withing $[1-\delta_2, 1+\delta_2]$. We will later prove that the probability of $\mathcal{B}_2$ is close to 1. 

Lemma \ref{lem::close-to-beta-tilde} implies that
\begin{equation}\label{eq::oracle-close-to-lasso}
    \E\|\betaL - \betaO \|^{2} \mathbbm{1}_{ \mathcal{B}_{1}\cap \mathcal{B}_{2}} \leq \frac{3\deltanum{delta::2}}{1-2\deltanum{delta::2}} \E \| \betaO -\beta \|^{2} \mathbbm{1}_{ \mathcal{B}_{1} } \leq \frac{3\deltanum{delta::2}}{1-2\deltanum{delta::2}}  (1+\deltanum{delta::1}) (1+\varepsilon)^{2} \cdot 2k\log(p/k).
\end{equation}
The right end is $2k\log(p/k) \cdot (1+o(1))$ as $\deltanum{delta::2}, \varepsilon\rightarrow 0$. To prove that the probability of the event $\mathcal{B}_2$ is close to one, we show how the set $S_*$ can be constructed. For this purpose we use the resolvent set used in \cite{su2016slope} for the SLOPE:

\begin{definition}[Resolvent set of Lasso]\label{def::resolvent-set-lasso}
    Fix $S=\supp(\beta)$ of cardinality at most $k$, and an integer $k^{*}$ obeying $k<k^{*}<p$. The set $S_{*}=S_{*}(S,k^{*})$ is said to be a resolvent set if it is the union of $S$ and the $k^{*}-k$ indicies with the largest values of $|X_{i}^{T}z|$ among all $i\in\{1,\ldots, p\}\setminus S$.  
\end{definition}

It turns out with a good choice of $k^*$, the resolvent set satisfies both conditions required in $\mathcal{B}_2$. The next proposition aims to prove this point. Define $S_{\diamond} := \supp(\beta)\cup\supp(\betaL)\cup\supp(\betaO)$. 

\begin{proposition}\label{prop::high-prob-lasso}
    Assume model \eqref{model::gaussian-model}. Consider the LASSO estimator $\betaL$ and the oracle estimator $\betaO$ \eqref{eq::oracle-estimator} with the regularization  $\lambda = \lambda_{\varepsilon} := (1+\varepsilon)\sqrt{2\log(p/k)}$. Let $S_{*} = S_{*}(S,k^{*})$ be the resolvent set. Suppose $k^{*}\geq 2k$, $k^{*}/p\rightarrow 0$ and $(k^{*}\log p)/n\rightarrow 0$. Then for any arbitrary small $\deltanum{delta::2} \in (0,1/2)$, $S_*$ satisfies the conditions required in $\mathcal{B}_2$ with probability greater than $1 - \exp\big[ -\defconstant\label{const::4}\varepsilon k\sqrt{2\log(p/k)} \big] - \constantnum{const::2}e^{-\constantnum{const::3} n\varepsilon^{2}}$, where
    $\constantnum{const::4}, \constantnum{const::1}, \constantnum{const::2}, \constantnum{const::3}>0$ are fixed numbers. Hence,
    \begin{equation}
 P( \mathcal{B}_2) \geq 1 - \exp\big[ -\defconstant\label{const::4}\varepsilon k\sqrt{2\log(p/k)} \big] - \constantnum{const::2}e^{-\constantnum{const::3} n\varepsilon^{2}}.
    \end{equation}
\end{proposition}
The proof of this theorem is presented in Section \ref{ssec:proof:prop4}. Note that if we define $\mathcal{B}:=\mathcal{B}_{1}\cap \mathcal{B}_{2}$ combining \eqref{eq:probB1} and Proposition \eqref{prop::high-prob-lasso} we have
\begin{equation}
    P(\mathcal{B}) \geq 1 - \exp(-n\varepsilon^{2}/2) -  \exp\big[ -\constantnum{const::4}\varepsilon k\sqrt{2\log(p/k)} \big] - \constantnum{const::2}e^{-\constantnum{const::3} n\varepsilon^{2}}. \label{eq::event-B-high-prob}
\end{equation}
Now we aim to use  \eqref{eq::oracle-dominates} and \eqref{eq::oracle-close-to-lasso} to finish the proof. 

\begin{align}
    \E \|\betaL - \beta\|^{2}\mathbbm{1}_{\mathcal{A}} =~& \E \|\betaO - \beta\|^{2}\mathbbm{1}_{\mathcal{A}\cap \mathcal{B}} + 2\E (\betaL - \betaO)^{T}(\betaO - \beta)\mathbbm{1}_{\mathcal{A}\cap \mathcal{B}} \\
    &+ \E \|\betaL - \betaO\|^{2}\mathbbm{1}_{\mathcal{A} \cap \mathcal{B} } + \E \| \betaL - \beta \|^{2}\mathbbm{1}_{ \mathcal{A} \cap \mathcal{B}^{c} } \nonumber\\
    \leq~& \E \| \betaO - \beta \|^{2} \mathbbm{1}_{ \mathcal{A}\cap\mathcal{B} } + 2\sqrt{\E\| \betaL - \betaO \|^{2} \mathbbm{1}_{ \mathcal{A} \cap \mathcal{B}}} \cdot \sqrt{ \E \| \betaO - \beta \|^{2} \mathbbm{1}_{ \mathcal{A} \cap \mathcal{B} } }  \nonumber\\
    &+ \E \| \betaL - \betaO \|^{2} \mathbbm{1}_{ \mathcal{A} \cap \mathcal{B}} + \Big( \E \| \betaL - \beta \|^{q} \mathbbm{1}_{\mathcal{A}} \Big)^{\frac{2}{q}} P(\mathcal{B}^{c}) \nonumber \\
    \leq~& \E \| \betaO - \beta \|^{2} \mathbbm{1}_{ \mathcal{B}_{1} } + 2\sqrt{\E\| \betaL - \betaO \|^{2} \mathbbm{1}_{ \mathcal{B}_{2} } } \cdot \sqrt{ \E \| \betaO - \beta \|^{2} \mathbbm{1}_{ \mathcal{B}_{1} } } \nonumber \\
    &+ \E \| \betaL - \betaO \|^{2} \mathbbm{1}_{ \mathcal{B}_{2} } + \Big( \E \| \betaL - \beta \|^{q} \mathbbm{1}_{\mathcal{A}} \Big)^{\frac{2}{q}} P(\mathcal{B}^{c}) \nonumber
    \\
    =~& 2k \log(p/k) \cdot \Big(1 + O\Big(\varepsilon +\deltanum{delta::1}+\sqrt{\deltanum{delta::2}}\Big) \Big)  + \Big( \E \| \betaL - \beta \|^{q} \mathbbm{1}_{\mathcal{A}} \Big)^{\frac{2}{q}} P(\mathcal{B}^{c}); \label{eq::lasso-risk-decomposition}
\end{align}
we have used H\"older's inequality with a power factor $q\geq2$. Therefore, as $\varepsilon,\deltanum{delta::1}, \deltanum{delta::2} \rightarrow 0$, the first term in the last line is the dominating term. 


It remains to derive an upper bound for $\E \| \betaL - \beta \|^{q} \mathbbm{1}_{\mathcal{A}} $. Note that \cite{bellec2018slope} has proved that the supremum risk of LASSO can be bounded by $C k \log(p/k)$, which is what we would like to prove as well. However, in order to prove this upper bound \cite{bellec2018slope} use $\lambda\geq C \sqrt{2\log(p/k)}$ for a constant $C>4+\sqrt{2}>(1+\varepsilon)$. This choice of $\lambda$ does not deliver the correct constant for the minimax risk. Hence, below we obtain a similar upper bound for the choice of $\lambda$ that offers the sharp constant for the minimax risk.  


Consider $\mathcal{A}$ \eqref{eq::event-A}, let the constant in $\mathcal{A}$ be $c_{0}=c_{0}(\deltanum{delta::3},\deltanum{delta::4},\delta_{0})$ defined by \eqref{eq::c_0}, we have

\begin{proposition}\label{prop::lasso-MSE-bound}
    Assume model \eqref{model::gaussian-model} and $\varepsilon>0$. Consider LASSO estimator $\betaL$ \eqref{eq::lasso-estimator0} with regularization $\lambda_{\varepsilon}$ as in \eqref{eq::lambda-epsilon}. Let $\mathcal{A}(c_{0},\delta_{0})$ be the event in \eqref{eq::event-A}. If $\defdelta\label{delta::3}$, $\defdelta\label{delta::4}>0$ such that $\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})(1+\deltanum{delta::3}) < 1+\varepsilon$. Then, for $q>2$ and some constant $C_{q}>0$, we have
    \begin{equation*}
        \E \Big[ \|\betaL-\beta\|_{2}^{q} ~ \mathbbm{1}_{\mathcal{A}}\Big] \leq \bigg( \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} + 1 \bigg)^{q} \Big(\frac{\lambda_{\varepsilon}\sqrt{k}}{\deltanum{delta::4}^{2}}\Big)^{q} \Big[\frac{1}{ (1-\delta_{0})^{q} } + \frac{C_{q}}{(\deltanum{delta::4}^{2}k\log(p/k))^{q}}\Big].
    \end{equation*}
\end{proposition}
The proof of this proposition is summarized in Section \ref{ssec:proof:prop5}. 




To demonstrate $\Big(\E \| \betaL - \beta \|^{q} \mathbbm{1}_{\mathcal{A}}\Big)^{\frac{2}{q}}P(\mathcal{B}^{c})\leq o(k\log (p/k))$, we have the following argument: First, fix $\varepsilon, \delta_{0}>0$. Second, select and fix $\deltanum{delta::3}$, $\deltanum{delta::4}>0$ such that $\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})(1+\deltanum{delta::3}) < 1+\varepsilon$. Then, from \eqref{eq::event-B-high-prob} and Proposition \ref{prop::lasso-MSE-bound}, if $n \geq \varepsilon^{-3}$ and $k\sqrt{2\log(p/k)}\geq \varepsilon^{-2}$, 
\begin{align}
    & \Big( \E \| \betaL - \beta \|^{q} \mathbbm{1}_{\mathcal{A}} \Big)^{\frac{2}{q}} P(\mathcal{B}^{c}) \nonumber \\
    \leq~  & \bigg( \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} + 1 \bigg)^{2} \Big(\frac{\lambda_{\varepsilon}\sqrt{k}}{\deltanum{delta::4}^{2}}\Big)^{2} \Big[\frac{1}{ (1-\delta_{0})^{2} } + \frac{C_{q}^{2/q}}{(\deltanum{delta::4}^{2}k\log(p/k))^{2}}\Big] \cdot P(\mathcal{B}^{c}) \nonumber \\
    \leq~ & C k\log(p/k) \cdot \varepsilon^{-4} \cdot \Big[\defconstant \exp\Big(-\defconstant n \varepsilon^{2} \Big) + \exp \Big(-\constantnum{const::4} \varepsilon k \sqrt{2\log(p/k)} \Big)\Big] \nonumber\\
    \leq~ & o\Big( k\log(p/k)\Big). \label{eq::lasso-mse-higher-order-bound}
\end{align}


\end{itemize}










%We refer to \cite{bellec2018slope} that it has been shown that under a condition similar to the restricted eigenvalue condition that LASSO can achieve the sparse minimax risk up to rate optimality. The condition introduced in \cite{bellec2018slope} is called the Strong Eigenvalue Condition defined below. This leads us to consider event $\mathcal{A}$. 
%\begin{definition}
%Let $c_{0}>0$ and $s\in\{1,\ldots,p\}$. We call a design matrix $X\in \R^{n\times p}$ satisfying the $SRE(s,c_{0})$ condition if $\|Xe_{j}\|_{2}\leq 1$ for all $j=1,\ldots, p$, and
%\begin{equation*}
%    \theta(s,c_{0}) := \min_{\Delta\in\mathcal{C}_{SRE}(s,c_{0}):\Delta\neq 0} \frac{\|X\Delta\|_{2}}{\|\Delta\|_{2}} >0,
%\end{equation*}
%where $\mathcal{C}_{SRE}(s,c_{0}):=\{\Delta\in\R^{p}: ~\|\Delta\|_{1}\leq(1+c_{0})\sqrt{s}\|\Delta\|_{2}\}$ is a cone in $\R^{p}$. 
%\end{definition}

%However, the result (Theorem 4.2 in \cite{bellec2018slope}) requires the regularization of LASSO satisfying $\lambda\geq C \sqrt{2\log(p/k)}$ for a constant $C>4+\sqrt{2}>(1+\varepsilon)$. Compared to our choice in \eqref{eq::lambda-epsilon}, larger $\lambda$ will cause the constant in the risk upper bound of the oracle estimator \eqref{eq::oracle-dominates} being larger than $2$. From \eqref{eq::lasso-risk-decomposition}, since the risk from the oracle estimator is the dominating term, it then results in an upper bound of the minimax risk with worse constant (larger than $2$). Therefore, in the following proposition, we intend to amend this result such that it can adapt to the choice of $\lambda$ in \eqref{eq::lambda-epsilon}.



Review \eqref{eq::lasso-MLE-decomposition}, \eqref{eq::MLE-higher-order-bound}, \eqref{eq::lasso-risk-decomposition} and \eqref{eq::lasso-mse-higher-order-bound}, we have completed the proof.


% \textcolor{red}{we should organize and summarize the rest of the proof here. }


\subsection{Proof of Proposition \ref{prop::MLE-bound}}\label{prop::MLE-bound:proof}
\begin{proof}[Proof of Proposition \ref{prop::MLE-bound}]


% \subsubsection{Roadmap of the proof of Proposition \ref{prop::MLE-bound}}
Recall the definition of the maximum likelihood estimator (MLE). For $k= |\supp(\beta)|$,
\begin{equation}\label{eq::MLE}
    \betaM = \argmin_{b\in \Theta(k)} \|y-Xb\|_{2}^{2}.
\end{equation}
It is straightforward to see from the definition of the MLE that since $\beta \in\Theta(k)$,
\[
\|y- X \beta\|_2^2 \geq \|y- X \betaM\|_2^2.  
\]
With $y=X\beta+z$, this implies
\begin{equation}\label{eq:fub:eq:MLE}
     \|X(\beta - \betaM)\|_{2}^{2} \leq 2 z^{T} X(\betaM-\beta).
\end{equation}
Fix $s\in\{1,\ldots,p\}$, let
\begin{equation}\label{eq::v-term-def}
    V_{s}:= \inf_{\Delta} \{\|X \Delta\|_{2}^{2}: ~ \|\Delta\|_{2}=1,~\|\Delta\|_{0}=s\}.
\end{equation}
Both $\beta$ and $\betaM$ are in $\Theta(k)$. Hence, $\|\beta-\betaM\|_0 \leq 2k$. Hence,
\begin{equation*}
    V_{2k}\cdot\|\beta - \betaM\|_{2}^{2} \leq \|X(\beta - \betaM)\|_{2}^{2} \leq 2 z^{T} X(\betaM-\beta) \leq 2 \|\betaM-\beta\|_{2} \cdot \sup_{\substack{\|u\|_{2}=1\\ \|u\|_{0}=2k}} z^{T}Xu.
\end{equation*}
Hence,
\begin{equation*}
    0\leq \|\beta - \betaM\|_{2} \leq \frac{2}{V_{2k}} \cdot\sup_{\substack{\|u\|_{2}=1\\ \|u\|_{0}=2k}} z^{T}Xu.
\end{equation*}
Then, using H\"older's inequality, we have
\begin{equation}\label{eq:upperbound2:MLE}
    \E \|\beta - \hat{\beta}\|_{2}^{m} \leq  2^{m} \bigg(\E \frac{1}{V_{2k}^{r}}\bigg)^{\frac{m}{r}} \bigg( \E \Big(\sup_{\substack{\|u\|_{2}=1\\ \|u\|_{0}=2k}} z^{T} Xu \Big)^{q}\bigg)^{\frac{m}{q}},
\end{equation}
where $r,q>0$, and $\frac{m}{r}+ \frac{m}{q} = 1$. Hence, we need to bound the two terms on the right hand side of \eqref{eq:upperbound2:MLE}. Since bounding these two terms requires delicate calculations we aim to do them in two separate lemmas, Lemma \ref{lem::inverse-min-eigenvalue} and Lemma \ref{lem::gaussian-complexity}.  

    \begin{lemma}\label{lem::inverse-min-eigenvalue}
    Suppose the Gaussian random design $X\in\R^{n\times p}$ in model \eqref{model::gaussian-model}. For $s\in \{1,\ldots,p\}$, let $V_{s}$ be defined as in \eqref{eq::v-term-def}. If $(s\log (p/s))/n\rightarrow 0$, then, for every fixed $r>0$, we have
    \begin{equation*}
        \E \frac{1}{V_{s}^{r}} = O(1).
    \end{equation*}
\end{lemma}
%In addition, we have the following upper bound for $\Big[\E \Big(\sup_{\substack{\|u\|_{2}=1\\ \|u\|_{0}=2k}} z^{T} Xu \Big)^{q}\Big]^{\frac{1}{q}}$.
    
% \textcolor{red}{We have to decide between $s$ and $k$ and make everything consistent. }

\begin{lemma}\label{lem::gaussian-complexity}
    Suppose the standard normal vector $z\in\R^{n}$ and the Gaussian design $X\in\R^{n\times p}$ in model \eqref{model::gaussian-model}. Denote $g\sim \calN(0, I_{p})$. For $s\in\{1,\ldots,p\}$, suppose $p/s\rightarrow \infty$ and $s\log(p/s) \rightarrow \infty$. Define $T(s)=\{u\in \R^{p}: \|u\|_{2}=1, \|u\|_{0}\leq s\}$. Then, for $\forall q\geq 1$,
    \begin{equation*}
        \Big[ \E \Big( \sup_{u\in T(s)} z^{T}Xu \Big)^{q} \Big]^{2/q} = \Big[ \E\left( \frac{\|z\|_{2}}{\sqrt{n}}\right)^{q} \Big]^{2/q} \cdot \bigg( \E \Big( \sup_{u\in T(s)} \langle g, u\rangle \Big)^{q} \bigg)^{2/q} \leq C s \log (p/s), \footnote{We can drop $|\cdot|$ in expectation since for symmetric $T(s)$, $\sup_{u\in T(s) }z^{T}Xu\geq0$ and $\sup_{u\in T(s)}\langle g,u\rangle\geq0$.}
    \end{equation*}
    for some constant $C>0$.
\end{lemma}

The proof of these two lemmas are presented after this proposition. Then, combining \eqref{eq:upperbound2:MLE} with the results of Lemmas \ref{lem::inverse-min-eigenvalue} and \ref{lem::gaussian-complexity} completes the proof.  

\end{proof}

\begin{proof}[Proof of Lemma \ref{lem::inverse-min-eigenvalue}]
    

% \subsubsection{Proof of Lemma \ref{lem::inverse-min-eigenvalue}}
Throughout the proof, we fix $s\in\{1,\ldots,p\}$ and let $V:=V_{s}$ for notational simplicity. Set $x= {\rm e}^{-8}$. The reasoning behind this particular choice of $x$ will become clear later in the proof. But as will be clear, this choice is not unique and many other choices will work as well.  We have
\begin{equation}\label{eq::inverse-min-eigenvalue-expectation}
    \E \frac{1}{V^{r}} = \E \left(\frac{1}{V^{r}} \mathbbm{1}_{(V\leq x)} \right) + \E
    \left(\frac{1}{V^{r}} \mathbbm{1}_{(V>x)}\right).
\end{equation}
Since $x$ is bounded, we have
\begin{equation}\label{eq:2ndterm:Vbound}
\E \left(\frac{1}{V^{r}} \mathbbm{1}_{(V>x)}\right)< \frac{1}{x^{r}}.
\end{equation}
Hence, in the rest of the proof, we aim to obtain an upper bound for $\E \left( \frac{1}{V^{r}} \mathbbm{1}_{(V\leq x)}\right)$. Towards this goal, we first obtain an upper bound for $P(V \leq 1-t)$. For $\forall t \in (0,1)$, using the union bound, we have
    \begin{equation*}
        P(V\leq 1-t) = P\Big(\min_{\substack{ S\subseteq [p] \\ |S|=s}} \inf_{\|\Delta\|_{2}=1} \|X_{S}\Delta\|_{2}^{2} \leq 1-t \Big) \leq \binom{p}{s} P \Big( \inf_{\|\Delta\|_{2}=1} \|X_{S}\Delta\|_{2}^{2} \leq 1-t \Big),
    \end{equation*}
    where to obtain the the last inequality we have used the union bound.
    The goal is to find an upper bound for $P \Big( \inf_{\|\Delta\|_{2}=1} \|X_{S}\Delta\|_{2}^{2} \leq 1-t \Big)$. The bound needs to be sharp for small values of $x$ to help us bound $\mathbb{E} (\frac{1}{V^r} \mathbbm{1} (V \leq x))$.\footnote{Note that standard concentration bounds for the singular values of Gaussian matrices are not sharp enough. } Towards this goal, define the set
    \[
    \mathscr{S}^{s-1} := \{ \Delta \in \mathbb{R}^{|S|} : \|\Delta=1\|_2=1 \}.
    \]
   We discretize the set $\mathscr{S}^{s-1}$ using an $\varepsilon$-net  and write the union bound over the net in the following way. Let $\mathcal{N}(\varepsilon)$ denote the $\varepsilon$-net of $\mathscr{S}^{s-1}}$. Then for $\forall \Delta \in \mathscr{S}^{s-1}$, there exists a $\Delta' \in \mathcal{N}(\varepsilon)$ such that $\|\Delta - \Delta'\|_{2} \leq \varepsilon$ and
    \begin{align}\label{eq::epsilon-net-ineq}
        \|X_{S}\Delta\|_{2}^{2} &= \|X_{S}\Delta'\|_{2}^{2} + \langle X_{S}(\Delta - \Delta'), X_{S}(\Delta+\Delta') \rangle \nonumber \\ &\geq \inf_{\Delta \in \mathcal{N}(\varepsilon)} \|X_{S}\Delta\|_{2}^{2} - \langle X_{S}(\Delta - \Delta'), X_{S}(\Delta+\Delta') \rangle \nonumber \\ 
        &\geq \inf_{\Delta \in \mathcal{N}(\varepsilon)} \|X_{S}\Delta\|_{2}^{2} - \|\Delta- \Delta'\|_2 \|\Delta+ \Delta'\|_2 \Big\langle X_{S} \frac{(\Delta - \Delta')}{\|\Delta-\Delta'\|_2}, X_{S}\frac{(\Delta+\Delta')}{\|\Delta + \Delta'\|_2}) \Big\rangle \nonumber \\
        &\overset{(a)}{\geq} \inf_{\Delta \in \mathcal{N}(\varepsilon)} \|X_{S}\Delta\|_{2}^{2} - 2 \epsilon  \Big\langle X_{S} \frac{(\Delta - \Delta')}{\|\Delta-\Delta'\|_2}, X_{S}\frac{(\Delta+\Delta')}{\|\Delta + \Delta'\|_2} \Big\rangle \nonumber \\    
             &\overset{(b)}{\geq} \inf_{\Delta \in \mathcal{N}(\varepsilon)} \|X_{S}\Delta\|_{2}^{2} - 2 \epsilon  \Big\| X_{S} \frac{(\Delta - \Delta')}{\|\Delta-\Delta'\|_2}\Big\|\Big\| X_{S}\frac{(\Delta+\Delta')}{\|\Delta + \Delta'\|_2}\Big\| \nonumber \\       
        &{\geq} \inf_{\Delta \in \mathcal{N}(\varepsilon)} \|X_{S}\Delta\|_{2}^{2} - 2\varepsilon\sup_{\Delta\in \mathscr{S}^{s-1}} \|X_{S}\Delta\|_{2}^{2},
    \end{align}
    where to obtain Inequality (a) we use the fact that $\|\Delta-\Delta'\| \leq \varepsilon$, and $\|\Delta+ \Delta'\|_2 \leq \|\Delta\|+ \Delta'\| \leq 2$. Also, to obtain Inequality (b) we have used the Cauchy-Schwartz inequality. Define 
    \[
    A:= \Big\{\sup_{\Delta \in \mathscr{S}^{s-1}} \|X_{S}\Delta\|_{2}^{2} \leq \frac{1}{1-t} \Big\}. 
    \]
    Let $2\varepsilon = (1-t)^{2}$. We have
    \begin{eqnarray}\label{eq:upper:for:lowest}
        \lefteqn{ P\Big( \inf_{\Delta \in \mathscr{S}^{s-1}} \|X_{S}\Delta\|_{2}^{2} \leq 1-t \Big)} \nonumber \\
        &\leq& P \Big( \inf_{\Delta \in \mathcal{N}(\varepsilon)} \|X_{S}\Delta\|_{2}^{2} \leq 2(1-t),~A \Big) + P(A^{c}) \nonumber \\
        &\leq& \frac{6^{s}}{(1-t)^{2s}} P\Big(\|X_{S}\Delta\|_{2}^{2} \leq 2(1-t) \Big) + P(A^{c}),
    \end{eqnarray}
    where the last inequality uses the union bound in addition to $|\mathcal{N}(\varepsilon)| \leq (3/\varepsilon)^{s}$ from Lemma \ref{lem::covering-number}. Note that the last expression holds for some fixed $S\subseteq [p]$, $|S|=s$, and a fixed $\Delta\in \mathscr{S}^{s-1}$. Our next goal is to bound the following two quantities from \eqref{eq:upper:for:lowest}: 

\begin{itemize}

\item $P\Big(\|X_{S}\Delta\|_{2}^{2} \leq 2(1-t) \Big)$: Note that $S$ is a fixed set and $\Delta$ is a fixed vector. Hence, $n\|X_{S}\Delta\|_{2}^{2} \sim \chi_{n}^{2}$. Applying Lemma \ref{lem::chi-square-concentration}, we have
\begin{equation}\label{p:xdelta:lower1}
P\Big(\|X_{S}\Delta\|_{2}^{2} \leq 2-2t\Big) \leq \exp\Big[ \frac{n}{2}\Big( 2t - 2 + \log(2(1-t)) \Big) \Big].
\end{equation}
An important feature of this bound that we need here is that as $t \rightarrow 1$, the probability $P\Big(\|X_{S}\Delta\|_{2}^{2} \leq 2-2t\Big)$ will be very small. We will get back to this point later. 

\item $P(A^{c})$: To obtain an upper bound for $P(A^{c})$ we again use the $\varepsilon$-net argument. Consider another $\varepsilon'$-net $\mathcal{N}(\varepsilon')$ for $\mathscr{S}^{s-1}$. Following a similar argument as the one in \eqref{eq::epsilon-net-ineq}, for certain $S\subseteq [p]$, $|S|=s$, we have 
\begin{equation*}
    \sup_{\Delta \in \mathscr{S}^{s-1}} \|X_{S}\Delta\|_{2}^{2} \leq \sup_{\Delta\in\mathcal{N}(\varepsilon')} \|X_{S}\Delta\|_{2}^{2} + 2\varepsilon'\Big( \sup_{\Delta \in \mathscr{S}^{s-1}} \|X_{S}\Delta\|_{2}^{2} \Big).
\end{equation*}
Thus,
\begin{equation}\label{eq:upperbound1}
    \sup_{\Delta \in \mathscr{S}^{s-1}} \|X_{S}\Delta\|_{2}^{2} \leq \frac{1}{1-2\varepsilon'} \sup_{\Delta\in\mathcal{N}(\varepsilon')} \|X_{S}\Delta\|_{2}^{2}.
\end{equation}
Let $1-2\varepsilon' = \sqrt{1-t}$. For $0<1-t\leq x$ we have 
\begin{eqnarray}\label{eq:sup:xsdelta:1}
    && P\Big( \sup_{\Delta \in \mathscr{S}^{s-1}} \|X_{S}\Delta\|_{2}^{2} > \frac{1}{1-t} \Big) \overset{(a)}{\leq} P \Big( \sup_{\Delta \in \mathcal{N}(\varepsilon')} \|X_{S}\Delta\|_{2}^{2}> \frac{1-2\varepsilon'}{1-t} \Big) \nonumber \\
    &\overset{(b)}{\leq} & |\mathcal{N}(\varepsilon')| \cdot P\Big( \|X_{S}\Delta\|_{2}^{2} > \frac{1}{\sqrt{1-t}} \Big) \overset{(c)}{\leq} \bigg(\frac{3}{\varepsilon'}\bigg)^{s} \cdot P\Big( \|X_{S}\Delta\|_{2}^{2} > \frac{1}{\sqrt{1-t}} \Big) \nonumber \\
    &\overset{(d)}{\leq} & \left(\frac{6}{1-\sqrt{x}}\right)^{s} \exp \Big\{ - \frac{n}{2}\Big( \frac{1}{\sqrt{1-t}} -1 - \log\frac{1}{\sqrt{1-t}} \Big) \Big\},
\end{eqnarray}
where to obtain Inequality (a), we have used \eqref{eq:upperbound1}. To obtain Inequality (b) we have used the union bound. Inequality (c) is the result of Lemmas \ref{lem::covering-number}, and finally Inequality (d) is concluded from Lemma \ref{lem::chi-square-concentration}.

\end{itemize}
    
In the rest of the proof, we use the bounds we provided above to obtain an upper bound for $\E \left(\frac{1}{V^{r}} \mathbbm{1}_{(V\leq x)} \right)$. Let $p_V(v)$ denote the probability density function of the random variable $V$. Also, define $F_V(u) = \int_0^u p_V(s)ds$. Then, we have
\begin{align}
\E \frac{1}{V^{r}} \mathbbm{1}_{(V\leq x)}  = \int_{0}^x \frac{1}{s^r} p_V(s)ds = \left. \frac{F_V(u)}{u^r}\right]_{0}^x + \int_{0}^x \frac{r F_V(s)}{s^{r+1}} ds = \frac{P(V \leq x)}{x^r} + \int_{0}^x \frac{r F_V(s)}{s^{r+1}} ds. 
\end{align}
To obtain the second equality above, we have used the integration by parts. To obtain the last Equality we have noted that from \eqref{p:xdelta:lower1} we have that $\lim_{u \rightarrow 0}  \frac{F_V(u)}{u^r} \rightarrow 0$ as $u \rightarrow 0$. Hence, by changing the varaible of integration from $s$ to $t= 1-s$, we will have

\begin{eqnarray}
     \lefteqn{\E \big( \frac{1}{V^{r}} \mathbbm{1}_{(V\leq x)} \Big) = \frac{P(V \leq x)}{x^r} + \int_{1-x}^1 P(V \leq 1-t) r(1-t)^{-r-1} dt}  \nonumber\\
    &\leq& \frac{P(V \leq x)}{x^r} + \int_{1-x}^1 \binom{p}{s} P\Big(\inf_{\Delta \in \mathscr{S}^{s-1}} \|X_{S}\Delta\|_{2}^{2} \leq 1-t \Big) r (1-t)^{-r-1} d t \nonumber\\
    &\overset{(a)}{\leq}& \frac{P(V \leq x)}{x^r} + \binom{p}{s} \int_{1-x}^1 \frac{6^{s}}{(1-t)^{2s}} P\Big( \|X_{S}\Delta \|_{2}^{2} \leq 2(1-t) \Big) r (1-t)^{-r-1} d t \nonumber\\
    &+& \binom{p}{s} \int_{1-x}^1 P \Big( \sup_{\Delta \in \mathscr{S}^{s-1}} \|X_{S}\Delta\|_{2}^{2} > \frac{1}{1-t} \Big) r(1-t)^{-r-1} d t \nonumber \\
    &\leq& \frac{P(V \leq x)}{x^r} + I_1 + I_2.
    \label{eq::left-tail-integration}
\end{eqnarray}
Note that to obtain Inequality (a), we have used \eqref{eq:upper:for:lowest}. 
In the next few lines we will show how $I_1$ and $I_2$ can be bounded. 
\begin{align}
    I_{1} &\overset{(a)}{\leq} \binom{p}{s} \int_{1-x}^1 \frac{6^{s}}{(1-t)^{2s}} r  (1-t)^{-r-1} \exp\Big[ \frac{n}{2}\Big( 2t -2 + \log(2(1-t)) \Big) \Big] dt \nonumber\\
    &= \binom{p}{s} \int_{1-x}^1 6^{s}r (1-t)^{\frac{n}{2}-r-2s-1}\exp \Big[ \frac{n}{2}\Big(2t - 1 +\log2\Big) \Big] dt \nonumber\\
    & \leq \binom{p}{s} 6^{s} r e^{\frac{n}{2}(\log2 + 1)} \int_{1-x}^{1} (1-t)^{\frac{n}{2}-r-2s-1} dt \nonumber\\
    & = \binom{p}{s} 6^{s} r e^{\frac{n}{2}(\log 2)} \frac{x^{\frac{n}{2}-r-2s}}{\frac{n}{2}-r-2s} \nonumber\\
    &\overset{(b)}{\leq} \binom{p}{s} 6^{s} r \frac{e^{\frac{n}{2}(-8+\log2)+r+4s}}{\frac{n}{2}-r-2s}\nonumber \\
    & \leq e^{C_{1}(s\log (p/s))-C_{2}n} = o(1), \label{eq::I_1-integration}
  \end{align}
where $C_{1},C_{2}>0$ are constants. Note that to obtain Inequality (a), we have used \eqref{p:xdelta:lower1}, and to obtain Inequality 
(b) we have set $x= \frac{1}{e^8}$. The last equality above is by the assumption $(s\log (p/s))/n \rightarrow 0$. 

In the next few lines we aim to find an upper bound for $I_2$. We have
\begin{align}
    I_{2} &\overset{(a)}{\leq} \binom{p}{s} \left( \frac{6}{1-\sqrt{x}} \right)^{s} \int_{1-x}^1 r (1-t)^{-r-1} \exp \Big\{ -\frac{n}{2} \Big( \frac{1}{\sqrt{1-t}} - 1 - \log \frac{1}{\sqrt{1-t}} \Big) \Big\} dt\nonumber \\
       &= \binom{p}{s} \left( \frac{6}{1-\sqrt{x}} \right)^{s} r \int_{1-x}^1  (1-t)^{-r-1} \exp \Big\{ -\frac{n}{2} \Big( \frac{1}{\sqrt{1-t}} - 1 - \log \frac{1}{\sqrt{1-t}} \Big) \Big\} dt\nonumber \\
    &\overset{(b)}{\leq} e^{C_1 s \log p/s}\int_{1-x}^1  (1-t)^{-r-1} \exp \Big\{ -\frac{n}{2} \Big( \frac{1}{\sqrt{1-t}} - 1 - \log \frac{1}{\sqrt{1-t}} \Big) \Big\} dt\nonumber \\
    & = e^{C_1 s \log p/s} \int_{1-x}^1 \exp \Big\{ -\frac{n}{2} \Big[ \frac{1}{\sqrt{1-t}} - 1 - \Big(1+\frac{4(r+1)}{n}\Big) \log \frac{1}{\sqrt{1-t}} \Big] \Big\} dt \nonumber\\
    & \overset{(c)}{=} e^{C_1 s \log p/s} \int_{1-x}^1 \exp \Big\{ -\frac{n}{2} \Big[ \frac{1}{\sqrt{1-t}} - 1 - 2 \log \frac{1}{\sqrt{1-t}} \Big] \Big\} dt \nonumber\\
     & \overset{(d)}{=} e^{C_1 s \log p/s} \int_{1-x}^1 \exp \Big\{ -\frac{n}{4} \Big[ \frac{1}{\sqrt{1-t}} \Big] \Big\} dt \nonumber\\
     & \overset{(e)}{=} e^{C_1 s \log p/s} \int_{1-x}^1 \exp \Big\{ -\frac{n}{4\sqrt{x}}  \Big\} dt \nonumber\\
    & \leq e^{C_1 s \log p/s} x \exp \Big\{ -\frac{n}{4\sqrt{x}}  \Big\} \nonumber\\
    & \leq e^{C_{1}(s\log (p/s)) - C_{2}n} \overset{(f)}{=} o(1),  \label{eq::I_2-integration}
\end{align}
where $C_{1},C_{2}>0$ are two constants. In the above equations,
\begin{itemize}
    \item To obtain Inequality (a), we have used \eqref{eq:sup:xsdelta:1}. 
    \item To obtain Inequality (b), we have used the Stirling approximation presented in Lemma \ref{lem:stirling}.  
    \item To obtain (c) we have used the fact that $r < \frac{n}{4}-1$ (for large enough $n$) and hence, $\frac{4(r+1)}{n}< 1$. 
    \item To obtain (d) we have used the fact that $x= {\rm e}^{-8}$ and hence for every $t \in [1-x, 1)$ we have $1+ 2 \log \frac{1}{\sqrt{1-t}} < \frac{1}{2 \sqrt{1-t}}$.
    \item To obtain (e), we have used the fact that, for every $t \in [1-x, 1)$, $\frac{1}{\sqrt{1-t}}> \frac{1}{\sqrt{x}}$.  
    \item To obtain (f), we have used the fact that $(s\log (p/s))/n \rightarrow 0$. 
\end{itemize}


By combing \eqref{eq::left-tail-integration} with \eqref{eq::I_1-integration} and \eqref{eq::I_2-integration}, we conclude that 
\begin{equation*}
    \E \Big(\frac{1}{V^{r}} \mathbbm{1}_{(V\leq x)} \Big)=O(1).
\end{equation*}
Therefore, Combining this result with \eqref{eq::inverse-min-eigenvalue-expectation} and \eqref{eq:2ndterm:Vbound}, we conclude that
\begin{equation*}
    \E \Big(\frac{1}{V^{r}} \Big)\leq O(1).
\end{equation*}

\end{proof}

\begin{proof}[Proof of Lemma \ref{lem::gaussian-complexity}]


    \textcolor{red}{Need to do the next part?}

% \subsubsection{Proof of Lemma \ref{lem::gaussian-complexity}}
We first construct an upper bound for $\Big[\E\Big( \sup_{u\in T(s)} \langle g, u\rangle \Big)^{q} \Big]^{2/q}$. Using Minkowski's inequality,
    \begin{equation}\label{eq::moments-of-gaussian-complexity}
        \bigg[ \E \Big( \sup_{u\in T(s)} ~ \langle g, u\rangle \Big)^{q} \bigg]^{2/q} \leq \bigg( \E \Big| \sup_{u\in T(s)} \langle g, u\rangle - \E \sup_{u\in T(s)} ~ \langle g, u \rangle \Big|^{q} \bigg)^{2/q} + \Big( \E \sup_{u\in T(s)}~ \langle g, u \rangle \Big)^{2}.
    \end{equation}
    Note that the second term above is the Gaussian complexity on $T(s)$. Following Exercise 5.7 in \cite{wainwright2019high}, for some constant $C>0$, we have
    \begin{equation}\label{eq::gaussian-complexity}
        \E \sup_{u\in T(s)} \langle g, u\rangle \leq \sqrt{C s \log (p/s)}.
    \end{equation}

    To bound the first term in \eqref{eq::moments-of-gaussian-complexity}, let $F(g):= \sup_{u\in T(s)}\langle g, u\rangle$. Then, for any $g, g' \in \R^{p}$,
    \begin{equation*}
        \langle g, u\rangle = \langle g-g', u\rangle + \langle g', u\rangle \leq \|g-g'\|_{2} \cdot \Big(\sup_{u\in T(s)} \|u\|_{2}\Big) + F(g').
    \end{equation*}
    Thus, $F$ is a $1$-Lipschitz function. Using the concentration of Lipshitz function of Gaussians (e.g., Theorem 2.2.6 in \cite{wainwright2019high}), we obtain
    \begin{eqnarray}
        && \E ~\Big| \sup_{u\in T(s)}  \langle g, u\rangle - \E \sup_{u\in T(s)}  \langle g, u \rangle \Big|^{q} = \int_{t>0} qt^{q-1}P\Big( |F(g)-\E F(g)| > t \Big) dt \nonumber \\
        &\leq& \int_{t>0} 2 qt^{q-1} e^{-\frac{t^{2}}{2}} d t  = 2^{\frac{q}{2}}q\Gamma(\frac{q}{2}) :=C_q. \label{eq::concentration-of-gaussian-complexity}
    \end{eqnarray}
    Here $\Gamma(\cdot)$ is the Gamma function. $C_q>0$ is a constant only depend on $q$. Then, based on \eqref{eq::moments-of-gaussian-complexity}, \eqref{eq::gaussian-complexity}, \eqref{eq::concentration-of-gaussian-complexity}, for some constant $C>0$, we have
    \begin{equation*}
        \bigg[\E \Big( \sup_{u\in T(s)} \langle g, u \rangle \Big)^{2q}\bigg]^{1/q} \leq (C_q)^{\frac{2}{q}} + C s \log(p/s) \leq C s \log (p/s),
    \end{equation*}
    as $s\log (p/s) \rightarrow \infty$.

    Finally, from the moments of the $\chi^{2}$ distribution, for $q<n$,
    \begin{equation*}
        \E \left( \frac{\|z\|_{2}}{\sqrt{n}} \right)^{q} = n^{-\frac{q}{2}} \cdot \frac{2^{\frac{q}{2}} \cdot\Gamma(\frac{n+q}{2})}{\Gamma(\frac{n}{2})} \leq 2^{\frac{q}{2}} =O(1).
    \end{equation*}
    Therefore, for some constant $C>0$,
    \begin{equation*}
        \bigg( \E \Big( \sup_{u\in T(s)} z^{T}Xu \Big)^{q} \bigg)^{2/q} \leq C s \log (p/s).
    \end{equation*}

\end{proof}

\subsection{Proof of Proposition \ref{prop::high-prob-lasso} }\label{ssec:proof:prop4}


Note that the event $\mathcal{B}_{2}:= \mathcal{B}_{2}(\deltanum{delta::2})$, has two parts:
\begin{itemize}
\item $\supp(\betaL)\cup\supp(\betaO)\cup\supp(\beta) \subseteq S_{*}$.
\item All the eigenvalues $X_{S_{*}}^{T}X_{S_{*}}$ lie withing $[1-\delta_2, 1+\delta_2]$
\end{itemize}
Let us start with the second condition and prove that it happens with high probability. In other words, we would like to prove that
   \begin{equation*}
     1-\delta_2 <  \sigma_{\min}(X_{S_*}^T X_{S_*})<  \sigma_{\max}(X_{S_*}^T X_{S_*}) < 1+\delta_2. 
    \end{equation*}
This result seems to be a simple conclusion of standard results on the minimum and maximum eigenvalues of Wishart matrices such as Lemma \ref{lem::eval-conc}. However, there is a subtle issue that needs to be address before such lemmas are useful: The choice of $S_*$ depends on $X$. Hence, the distribution of the elements of the matrix $X_{S_*}$ is not iid Gaussian. However, \cite{su2016slope} has proposed a clever trick to circumvent this issue. For the sake of brevity we do not mention their trick and only use the following lemma proved in \cite{su2016slope}. 

\begin{lemma}[Lemma A.11 in \cite{su2016slope}]\label{lem::X_S*-singular-values}
    Let $k<k^{*}<\min\{n,p\}$ be any (deterministic) integer. Denote by $\sigma_{\min}$ and $\sigma_{\max}$, respectively, the smallest and the largest singular value of $X_{S_{*}}$. Then for any $t>0$,
    \begin{equation*}
        \sigma_{\min} > \sqrt{1-1/n} - \sqrt{k^{*}/n} - t
    \end{equation*}
    holds with probability at least $1-e^{-nt^{2}/2}$. Furthermore,
    \begin{equation*}
        \sigma_{\max} < \sqrt{1-1/n} + \sqrt{k^{*}/n} + \sqrt{8k^{*}\log(p/k^{*})/n} + t
    \end{equation*}
    holds with probability at least $1-e^{-nt^{2}/2} - (\sqrt{2}ek^{*}/p)^{k^{*}}$.
\end{lemma}
By setting  $t=\sqrt{k^{*}\log(p/k^{*})/n}$ in Lemma \ref{lem::X_S*-singular-values}, we have
\begin{equation}\label{eq::singular-values-in-range}
    1-\deltanum{delta::2}\leq \sigma_{\min}(X_{S_{*}}^{T}X_{S_{*}}) \leq \sigma_{\max}(X_{S_{*}}^{T}X_{S_{*}}) \leq 1 +\deltanum{delta::2}.
\end{equation}
with probability larger than $1-(C ek^{*}/p)^{k^{*}}$ as $k^{*}/p\rightarrow 0$ and $k^{*}\log (p/k^{*}) / n \rightarrow 0$. 

We now discuss the second condition required in Event $\mathcal{B}_2$, i.e. $S_{\diamond} := \supp(\betaL)\cup\supp(\betaO)\cup\supp(\beta) \subseteq S_{*}$. The following lemma aims to prove this claim. 


\begin{lemma}\label{lem::resolvent-set-supp-recovery}
    Suppose $k^{*}\geq 2k$, $k^{*}/p\rightarrow 0$ and $(k^{*}\log p)/n \rightarrow 0$. Then 
    \begin{equation*}
        \inf_{\|\beta\|_{0}\leq k} P(S_{\diamond} \subseteq S_{*}) \geq 1 - \exp\big[ -\constantnum{const::1}\varepsilon k\sqrt{2\log(p/k)} \big] - \constantnum{const::2}e^{-\constantnum{const::3} n\varepsilon^{2}},
    \end{equation*}
    for some constants $\constantnum{const::1},\constantnum{const::2}, \constantnum{const::3}>0$.
\end{lemma}

\textcolor{red}{these lines should be pushed back!} Then, combining \eqref{eq::singular-values-in-range} with Lemma \ref{lem::resolvent-set-supp-recovery}, we conclude the statement in Proposition \ref{prop::high-prob-lasso}.
\end{proof}


\begin{proof}[Proof of Lemma \ref{lem::resolvent-set-supp-recovery}]
     By construction, $\supp(\beta)\subseteq S_{*}$. Hence we only need to show that the following two conditions hold with high probability:
     \begin{enumerate}
     \item $\supp(\betaL)\subseteq S_{*}$.
     \item $\supp(\betaO)\subseteq S_{*}$. 
    \end{enumerate}
     We first prove  $\supp(\betaL)\subseteq S_{*}$. Define $\bstar$ as the solution of the following `reduced' problem:
    \begin{equation}
        \arg\min_{b\in \R^{|S_{*}|}} \frac{1}{2}\|y-X_{S_{*}}b\|^{2} +\lambda_{\varepsilon}\|b\|_{1} \label{eq::lasso-reduced-prob}.
    \end{equation}
    In other words, if we assume that  $\supp(\betaL)\subseteq S_{*}$ holds, then the solution of LASSO has to be the same as $\bstar$ on $S_*$. Hence, as our next step we aim to show that $\betaL_{S_{*}} = \bstar$ and $\betaL_{S_{*}^{c}} = \mathbf{0}$. 
    
    From the KKT conditions of LASSO we conclude that if $\|X_{S_{*}^{c}}^{T}(y-X_{S_{*}}\bstar) \|_{\infty} \leq \lambda_{\varepsilon}$, then $\betaL_{S_{*}} = \bstar$ and $\betaL_{S_{*}^{c}} = \mathbf{0}$. Hence, to achieve out goal, it's sufficient to prove $\|X_{S_{*}^{c}}^{T}(y-X_{S_{*}}\bstar) \|_{\infty} \leq \lambda_{\varepsilon}$. To achive this goal we prove the following two conditions:
    \begin{equation}
        \| X_{S_{*}^{c}}^{T}X_{S_{*}}(\beta_{S_{*}} - \bstar) \|_{\infty} \leq \frac{\varepsilon}{2} \sqrt{2\log(p/k)}, \label{eq::lasso-kkt-1}
    \end{equation}
    and
    \begin{equation}
        \|X_{S_{*}^{c}}^{T}z\|_{\infty} \leq \Big(1+\frac{\varepsilon}{2}\Big) \sqrt{2\log(p/k)}. \label{eq::lasso-kkt-2}
    \end{equation}
    Before analyzing \eqref{eq::lasso-kkt-1} and \eqref{eq::lasso-kkt-2}, we first illustrate a property of the resolvent set using a clever trick from  \cite{su2016slope}. Let $Q\in \R^{n\times n}$ be an orthogonal matrix such that
\begin{equation*}
    Qz = \big( \|z\|, 0, \ldots, 0\big).
\end{equation*}
In the proofs, $Q$ can further be assumed to be measurable with respect to $z$. Let $\tilde{\omega}\in\R^{1\times p}$, $\tilde{W}\in\R^{(n-1)\times p}$ and
\begin{equation*}
    W=\begin{bmatrix}
\tilde{\omega}\\ 
\tilde{W}
\end{bmatrix} := QX.
\end{equation*}
$Q$ being independent of $X$ implies that $W$ is still a Gaussian random matrix, with i.i.d. $\calN(0,1/n)$ entries. Furthermore,
\begin{equation}\label{eq::Xz-omega-tilde}
    X_{i}^{T}z = (QX_{i})^{T}(Qz) = \|z\|(QX_{i})_{1} = \|z\|\tilde{\omega}_{i}.
\end{equation}
This indicates that $S_{*}$ is composed of the union of $S$ and $k^{*}-k$ indices in $\{1,\ldots, p\}\setminus S$ of the largest $|\tilde{\omega}_{i}|$. Since $\tilde{\omega}$ and $\Tilde{W}$ are independent, $\Tilde{W}$ and $S_{*}$ are also independent. Thus, $\tilde{W}_{S_{*}^{c}}$ and $\Tilde{W}_{S_{*}}$ are both Gaussian random matrices. Now we aim to use this trick to prove  \eqref{eq::lasso-kkt-1} and \eqref{eq::lasso-kkt-2}. 

\begin{itemize}
\item Proving $\| X_{S_{*}^{c}}^{T}X_{S_{*}}(\beta_{S_{*}} - \bstar) \|_{\infty} \leq \frac{\varepsilon}{2} \sqrt{2\log(p/k)}$: We have
    \begin{align}\label{eq:checkingKKT1}
        &X_{S_{*}^{c}}^{T}X_{S_{*}}(\beta_{S_{*}}-\hat{b}_{S_{*}}) = X_{S_{*}^{c}}^{T}X_{S_{*}}(X_{S_{*}}^{T}X_{S_{*}})^{-1}\big( X_{S_{*}}^{T}(y-X_{S_{*}}\hat{b}_{S_{*}}) - X_{S_{*}}^{T}z\big) \nonumber \\
        &= X_{S_{*}^{c}}^{T}Q^{T}\underbrace{QX_{S_{*}}(X_{S_{*}}^{T}X_{S_{*}})^{-1} \big (X_{S_{*}}^{T}(y-X_{S_{*}}\hat{b}_{S_{*}}) - X_{S_{*}}^{T}z\big)}_{:=\xi}.
    \end{align}
       We first derive the bound for $\|\xi\|$. We have
   \begin{align}
        \|\xi\| & \leq \|X_{S_{*}}(X_{S_{*}}^{T}X_{S_{*}})^{-1}\| \cdot \|X_{S_{*}}^{T}(y-X_{S_{*}}\hat{b}_{S_{*}}) - X_{S_{*}}^{T}z\|. 
 \end{align}
Hence, our next goal is to bound the three terms  $\|X_{S_{*}}(X_{S_{*}}^{T}X_{S_{*}})^{-1}\|$, $\|X_{S_{*}}^{T}(y-X_{S_{*}}\hat{b}_{S_{*}})$, and $X_{S_{*}}^{T}z$. Since $\hat{b}_{S_{*}}$ is the solution to the reduced Lasso problem \eqref{eq::lasso-reduced-prob}, its KKT condition implies that 
    \begin{equation}
        \|X_{S_{*}}(y-X_{S_{*}}\hat{b}_{S_{*}})\|_{\infty} \leq \lambda_{\varepsilon}. \label{eq::Sstar-KKT}
    \end{equation}
    Furthermore, if we set $t=1/2$ in Lemma \ref{lem::X_S*-singular-values} we obtain
    \begin{equation}
        \|X_{S_{*}}(X_{S_{*}}^{T}X_{S_{*}})^{-1}\| \leq \Big( \sqrt{1-1/n} - \sqrt{k^{*}/n} - 1/2 \Big)^{-1} < 2.01 \label{eq::X_Sstar-operator-norm}
    \end{equation}
    with probability at least $1-e^{-n/8}$ for sufficiently large $p$, where in the last step we have used $k^{*}/n\rightarrow 0$. Finally, we use the following Lemma to bound $\|X_{S_{*}}^{T}z\|$.
    
    
    \begin{lemma}[Lemma A.7 in \cite{su2016slope}]\label{lem::sup-X^T_S*z}
    Let $1\leq k^* <p$ be any (deterministic) integer, then
    \begin{equation*}
        \sup_{|T|=k^{*}} \|X_{T}^{T}z\| \leq \sqrt{32k^{*}\log(p/k^{*})}
    \end{equation*}
    with probability at least $1-e^{-n/2}-(\sqrt{2}ek^{*}/p)^{k^{*}}$. Above, the superemum is taken over all the subsets of $\{1,\ldots,p\}$ with cardinality $k^{*}$.
\end{lemma}
    Hence, from \eqref{eq::Sstar-KKT}, \eqref{eq::X_Sstar-operator-norm} and Lemma \ref{lem::sup-X^T_S*z}, we have
    \begin{align}
        \|\xi\| & \leq \|X_{S_{*}}(X_{S_{*}}^{T}X_{S_{*}})^{-1}\| \cdot \|X_{S_{*}}^{T}(y-X_{S_{*}}\hat{b}_{S_{*}}) - X_{S_{*}}^{T}z\| \nonumber\\
        & \leq 2.01 \Big( \sqrt{k^{*}}\lambda_{\varepsilon} + 4\sqrt{2k^{*}\log(p/k^{*})} \Big) \nonumber\\
        & \leq 2.01 \Big((1+\varepsilon)\sqrt{2} + 4\sqrt{2}\Big) \sqrt{k^{*}\log(p/k^{*})} \nonumber\\
        & \leq C \cdot \sqrt{k^{*}\log(p/k^{*})} \label{eq::xi-2norm-bound}
    \end{align}
    with probability at least $1-e^{-n/2} - (\sqrt{2} ek^{*}/p)^{k^{*}} - e^{-n/8}=: 1- P_{\xi}$; where in the third line we have used $k^{*}\geq k$.

As we discussed before \eqref{eq:checkingKKT1} in order to check the first KKT condtion we have to find an upper bound for 
    \begin{align}\label{eq:boundKKT1:1}
        X_{S_{*}^{c}}^{T}X_{S_{*}}(\beta_{S_{*}}-\hat{b}_{S_{*}}) &= X_{S_{*}^{c}}^{T}Q^{T}\underbrace{QX_{S_{*}}(X_{S_{*}}^{T}X_{S_{*}})^{-1} \big (X_{S_{*}}^{T}(y-X_{S_{*}}\hat{b}_{S_{*}}) - X_{S_{*}}^{T}z\big)}_{:=\xi} \nonumber \\
        &= \big(\tilde{\omega}_{S_{*}^{c}}^{T}, 0\big)\xi + \big( 0, \Tilde{W}_{S_{*}^{c}}^{T} \big)\xi.
    \end{align}



    For the first term, we have
    \begin{equation}
        \|(\tilde{\omega}_{S_{*}^{c}}^{T}, 0)\xi\|_{\infty} = |\xi_{1} |\cdot \|\tilde{\omega}_{S_{*}^{c}}^{T}\|_{\infty} \leq \|\xi\|_{2} \cdot \|\tilde{\omega}_{S_{*}^{c}}^{T}\|_{\infty}. \label{eq::small-omega-tilde-term}
    \end{equation}
    Based on \eqref{eq::Xz-omega-tilde}, we recognize $\tilde{\omega}_{S_{*}^{c}}$ is a Gaussian vector excludes the $k^{*}-k$ largest (in absolute value) coordinates from $p-k$ indices of $\{1,\ldots,p\}\setminus S$. Thus, suppose $\zeta_{1},\ldots, \zeta_{p-k}$ are i.i.d. $\calN(0,1)$ variables and $|\zeta|_{(1)}\geq\ldots\geq |\zeta|_{(p-k)}$. Hence, to bound the term $ \|(\tilde{\omega}_{S_{*}^{c}}^{T}, 0)\xi\|_{\infty}$ we need to find an upper bound for $|\zeta|_{(k^{*}-k+1)}|$. For this purpose we can use standard results such as Lemma \ref{lem::Gaussian-order-statistics}.   From Lemma \ref{lem::Gaussian-order-statistics} we obtain that 
    \begin{equation}
        \sqrt{n}\|\tilde{\omega}_{S_{*}^{c}}\|_{\infty} = |\zeta|_{(k^{*}-k+1)} \leq \Big(1+\frac{\varepsilon}{4}\Big) \cdot \sqrt{2 \log \frac{2(p-k)}{k^{*}-k+1}} \leq \Big(1+\frac{\varepsilon}{3}\Big) \sqrt{2\log \frac{p}{k}}, \label{eq::omega-tilde-bound}
    \end{equation}
  with probability at least 
    \begin{equation*}
        1- \exp \big[ - C \varepsilon k \sqrt{2\log(p/k)} \big] =: 1 - P_{1},
    \end{equation*}
    for some constant $C>0$; we used that $k\leq k^{*}-k+1$ and $Cp/k \leq (p-k)/k\leq p/k$. Thus, from \eqref{eq::small-omega-tilde-term} and \eqref{eq::omega-tilde-bound} and $k^{*}\geq k$, we obtain
    \begin{equation}\label{eq::small-omega-tilde-bound}
        \|(\tilde{\omega}_{S_{*}^{c}}^{T}, 0)\xi\|_{\infty} \leq C \cdot \sqrt{\frac{k^{*}}{n}\log\frac{p}{k^{*}}} \cdot \sqrt{2\log p} \leq C \cdot \sqrt{\frac{k^{*}\log p}{n}} \sqrt{2\log \frac{p}{k}}. 
    \end{equation}
    
    Our next goal is to bound the second term in \eqref{eq:boundKKT1:1}, i.e. $ \|(0, \Tilde{W}_{S_{*}^{c}}^{T})\xi \|_{\infty}$. \textcolor{red}{I think it is correct, but have to think about it more carefully later.} From the discussion about \eqref{eq::Xz-omega-tilde}, we note that $\xi$ is independent of $\Tilde{W}_{S_{*}^{c}}$, thus \textcolor{red}{Next equation requires a bit more explanation!}
    \begin{equation*}
        \|(0, \Tilde{W}_{S_{*}^{c}}^{T})\xi \|_{\infty} \overset{d}{=} \Big\|\sqrt{\frac{\xi_{2}^{2}+\cdots+\xi_{n}^{2}}{n}} (\zeta_{1}, \ldots, \zeta_{p-k^{*}}) \Big\|_{\infty} \leq \|\xi\|_{2} \frac{1}{\sqrt{n}} |\zeta|_{(1)},
    \end{equation*}
    with $\zeta_{1},\ldots, \zeta_{p-k^{*}}\simiid \calN(0,1)$ and $|\zeta|_{(1)}$ denote the largest one in absolute value. From Lemma \ref{lem::Gaussian-maxima}, we have $|\zeta|_{(1)} \leq C\cdot \sqrt{2\log(p-k^{*})}$, holds with probability at least $1- \exp[-C \sqrt{\log  p}] =: 1-P_{2}$, with some constant $C>0$; we used $k^{*}/p \rightarrow 0$. Thus, with \eqref{eq::xi-2norm-bound}, we have
    \begin{equation}\label{eq::big-w-tilde-bound}
        \|(0, \Tilde{W}_{S_{*}^{c}}^{T}) \xi\|_{\infty} \leq C\sqrt{\frac{k^{*}}{n}\log \frac{p}{k^{*}}} \sqrt{2\log (p-k^{*})} \leq C\sqrt{\frac{k^{*}\log p}{n}} \sqrt{2\log \frac{p}{k}}.
    \end{equation}

    \textcolor{red}{Requires revision still.}
    Combining \eqref{eq::small-omega-tilde-bound} and \eqref{eq::big-w-tilde-bound}, and \eqref{eq:boundKKT1:1} we have 
    \begin{equation}
        \|X_{S_{*}^{c}}^{T}X_{S_{*}}(\beta_{S_{*}} - \betaL_{S_{*}})\|_{\infty} \leq \|(\Tilde{\omega}_{S_{*}^{c}}^{T}, 0)\xi\|_{\infty} + \|(0, \Tilde{W}_{S_{*}^{c}}^{T})\xi\|_{\infty} \leq C\sqrt{\frac{k^{*}\log p}{n}} \sqrt{2\log (p/k)}, \label{eq::XTX(betahat-beta)-inf-bound}
    \end{equation}
    with probability at least $1-P_{\xi} - P_{1}- P_{2}$ for \eqref{eq::xi-2norm-bound}, \eqref{eq::small-omega-tilde-term}, \eqref{eq::big-w-tilde-bound} to hold.


`



\item Proving $ \|X_{S_{*}^{c}}^{T}z\|_{\infty} \leq \Big(1+\frac{\varepsilon}{2}\Big) \sqrt{2\log(p/k)}$: 
 Following the discussion about \eqref{eq::Xz-omega-tilde}, under event \eqref{eq::small-omega-tilde-term} and that $\|z\|_{2}/\sqrt{n} \leq (1+\varepsilon/3)$, we have
    \begin{align}
        \|X_{S_{*}^{c}}^{T}z\|_{\infty} = \|z\|_{2} \cdot \|\tilde{\omega}_{S_{*}^{c}}\|_{\infty} \leq \Big(1+\frac{\varepsilon}{3}\Big)^{2} \sqrt{2\log \frac{2(p-k)}{k^{*}-k+1}} \leq \Big(1+\frac{\varepsilon}{2}\Big) \sqrt{2\log \frac{p}{k}} \label{eq::Xz-inf-bound}
    \end{align}
    holds with probability at least $1 - P_{z} - P_{\xi}$ where
    \begin{equation*}
        P\Big(\|z\|_{2}/\sqrt{n} \geq 1 + \varepsilon/3\Big) \leq e^{-n\varepsilon^{2}/18} := P_{z}.
    \end{equation*} 
    
    As a result, we have (1):
    \begin{equation*}
        \supp(\betaL) \subseteq S_{*}
    \end{equation*}
    holds with high probability $1-P_{1}-P_{2}-P_{\xi}-P_{z}$ under events \eqref{eq::xi-2norm-bound}, \eqref{eq::small-omega-tilde-term}, \eqref{eq::big-w-tilde-bound} and \eqref{eq::Xz-inf-bound}.


\end{itemize}

    
 
    
    
    

    
    
    
    
    \textcolor{red}{Up to the next proposition I have revised the above proof once. }


    \textbf{Back to show (2)}. In order to show $\supp(\betaO) \subseteq S_{*}$,  it is sufficient to see that
    \begin{equation}
        \|X_{S_{*}^{c}}^{T}z\|_{\infty} \leq \lambda_{\varepsilon}. \label{eq::supp-beta-tilde}
    \end{equation}
    We mark this event holding under \eqref{eq::Xz-inf-bound} with corresponding high probability $1-P_{z}-P_{\xi}$.

    As a conclusion of \eqref{eq::XTX(betahat-beta)-inf-bound}, \eqref{eq::Xz-inf-bound} and \eqref{eq::supp-beta-tilde}, we have that for some constants $\defconstant\label{const::1}$, $\defconstant\label{const::2}$, $\defconstant\label{const::3}>0$, $\supp(\betaL) \subseteq S_{*}$ holds with probability at least
    \begin{equation*}
        1- P_{\xi} - P_{1} - P_{2} - P_{z} = 1 - \exp\big[ -\constantnum{const::1}\varepsilon k\sqrt{2\log(p/k)} \big] - \constantnum{const::2}e^{-\constantnum{const::3}n\varepsilon^{2}}.
    \end{equation*}







\subsection{Proof of Proposition \ref{prop::lasso-MSE-bound}}\label{ssec:proof:prop5}

The basic proof idea of this section comes from \cite{bellec2018slope}. Throughout the proof, we will use the following notation: Let $\Big(|u|_{(1)}, \ldots, |u|_{(p)}\Big)$ denote the non-increasing rearrangement of $(|u_{1}|, \ldots, |u_{p}|)$. For given $\deltanum{delta::3}$, $\deltanum{delta::4}$, $\defdelta\label{delta::5}\in(0,1)$ and any $u=(u_{1},\ldots,u_{p})\in\R^{p}$, define
    \begin{subequations} \label{eq::H-G-function}
    \begin{align}
       & H(u):= (1+\deltanum{delta::4}) \Big(\sum_{j=1}^{k} |u|_{(j)} 4\sqrt{\log(2p/j)} + (1+\deltanum{delta::3}) \sum_{j=k+1}^{p} |u|_{(j)}\sqrt{2\log(p/k)}\Big), \\
       & G(u):=(1+\deltanum{delta::4}) \deltanum{delta::5}^{-1} \sqrt{\log(1/\deltanum{delta::5})} \|Xu\|_{2}. 
    \end{align}
    \end{subequations}
In addition, let
\begin{equation}
    \delta(\lambda):= e^{- \frac{\lambda^{2}}{2}}, ~\Leftrightarrow ~ \sqrt{2\log (1/\delta(\lambda))} = \lambda. \label{eq::delta(lambda)}
\end{equation}
We will use the following inequality: by using Stirling's formula, for any $s\in[p]$, $s\log (s/e)\leq \log(s!) \leq s\log(s)$. Hence, 
\begin{equation}
    s\log(2p/s) \leq \sum_{j=1}^{s}\log(2p/j) = s\log(2p) - \log(s!) \leq s\log(2ep/s). \label{eq::stirling}
\end{equation}

\begin{proof}[Proof of Proposition \ref{prop::lasso-MSE-bound}]

Following \cite{bellec2018slope}, we first show a bound for the realization of the random matrix $X$, i.e. fix $X\in \R^{n\times p}$. We have the following lemma:
\begin{lemma}\label{lem::lasso-l2-bound}
    Assume model \eqref{model::gaussian-model} and let $\|\beta\|_{0}\leq k$. Given $\varepsilon,\delta_{0}\in (0,1)$, let $\deltanum{delta::3}, \deltanum{delta::4}$ be any positive numbers such that $\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})(1+\deltanum{delta::3})<1+\varepsilon$. Assume the $SRE(k,c_{0})$ condition holds with 
    \begin{equation}\label{eq::c_0}
        c_{0} := \bigg( \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} + 1 \bigg) / \bigg( 1 - \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})(1+\deltanum{delta::3})}{1+\varepsilon} \bigg).
    \end{equation}
    Consider the LASSO estimator with tuning parameter $\lambda_{\varepsilon}$ satisfying \eqref{eq::lambda-epsilon}.
    Then, on the event \eqref{eq::stochastic-error-event}, we have
    \begin{equation}
    \|\betaL-\beta\|_{2} \leq C(k,\lambda_{\varepsilon},\deltanum{delta::5})\lambda_{\varepsilon} \sqrt{k}, \label{eq::lasso-l2bound}
    \end{equation}
    where $\deltanum{delta::5}\in(0,1)$ is a parameter in $G(u)$ in event \eqref{eq::stochastic-error-event} and
    \begin{equation} \label{eq::constant_in_lasso_2norm_bound}
         C(k,\lambda_{\varepsilon},\deltanum{delta::5}) := \bigg( \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} + 1 \bigg) \cdot \bigg( \frac{1}{\deltanum{delta::4}^{2}}\frac{\log(1/\deltanum{delta::5})}{k\log(1/\delta(\lambda_{\varepsilon}))} \vee \frac{1}{\theta^{2}(k,c_{0})} \bigg).
    \end{equation}
\end{lemma}
The proof of this lemma is presented later in the section.

The above lemma relies on the event \eqref{eq::stochastic-error-event} which sets a limit for the randomness from $z$, though it still assumes $X$ is fixed. Then we refer to Lemma \ref{lem::bound-on-stochastic-error}, which analyzes the probability for the condition of the above lemma to hold, for every $\deltanum{delta::5} \in(0,1)$. By integrating the tail bound, we obtain the following lemma:

\begin{lemma}\label{lem::lasso-MSE-bound}
    Assume model \eqref{model::gaussian-model} with $\|\beta\|_{0}\leq k$. Let $c_{0}>0$ be as in \eqref{eq::c_0}. Consider the LASSO estimator $\betaL$ \eqref{eq::lasso-estimator0} with tuning parameter $\lambda_{\varepsilon}$ in \eqref{eq::lambda-epsilon}. Suppose the $SRE(k,c_{0})$ holds. Then, for any $q>2$,
    \begin{equation*}
         \E \|\betaL-\beta\|_{2}^{q} \leq \bigg( \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} + 1 \bigg)^{q} \Big(\frac{\lambda_{\varepsilon}\sqrt{k}}{\deltanum{delta::4}^{2}}\Big)^{q} \Big[\frac{1}{\theta^{2q}(k,c_{0})} + \frac{C_{q}}{(\deltanum{delta::4}^{2}k\log(p/k))^{q}}\Big],
    \end{equation*}
    where $C_{q} = q/2\cdot \Gamma(q)$ with Gamma function $\Gamma(\cdot)$.
\end{lemma}
The proof of this lemma is presented later in the section.

Lemma \ref{lem::lasso-MSE-bound} can be viewed as an uniform upper bound for the conditional expectation $\E \Big(\|\hat{\beta}-\beta\|_{2}^{q} ~|X\Big)$ for all $X\in \mathcal{A}$. Then, applying the tower property, we obtain
\begin{align*}
    & \E \Big[ \|\hat{\beta}-\beta\|_{2}^{q} ~ \mathbbm{1}_{\mathcal{A}}\Big] =   \E \bigg[ \E \Big(\|\hat{\beta}-\beta\|_{2}^{q} ~|X\Big)\mathbbm{1}_{\mathcal{A}} \bigg] \\
    \leq~& \bigg( \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} + 1 \bigg)^{q} \Big(\frac{\lambda_{\varepsilon}\sqrt{k}}{\deltanum{delta::4}^{2}}\Big)^{q} \Big[\frac{1}{ (1-\delta_{0})^{q} } + \frac{C_{q}}{(\deltanum{delta::4}^{2}k\log(p/k))^{q}}\Big].
\end{align*}
\end{proof}


The next lemma referring to Lemma A.2 in \cite{bellec2018slope} describes an inequality useful for simplification of LASSO problem.
\begin{lemma}\label{eq::convex-minimization-ineq}
    Let $h: \R^{p} \rightarrow \R$ be a convex function. Let $z \in \R^{n}$, $X$ be any $n\times p$ matrix, and $y=X\beta+z$. If $\betaL$ is a solution of the minimization problem $\min_{\beta \in \R^{p}} \Big ( \frac{1}{2}\|X\beta - y\|_{2}^{2} +h(\beta) \Big)$, then $\betaL$ satisfies for all $\beta \in \R^{p}$
    \begin{equation*}
        \|X(\betaL - \beta)\|_{2}^{2} \leq z^{T}X(\betaL-\beta) + h(\beta) - h(\betaL). 
    \end{equation*}
\end{lemma}


\begin{proof}[Proof of Lemma \ref{lem::lasso-l2-bound}]
    From Lemma \ref{eq::convex-minimization-ineq}, letting $h(\cdot) = \lambda_{\varepsilon} \|\cdot\|_{1}$ in the condition of Lemma \ref{eq::convex-minimization-ineq}, we have that for all $\beta \in \R^{p}$, the following holds almost surely:
    \begin{equation}
        \|X(\betaL - \beta)\|_{2}^{2} \leq \bigtriangleup^{*}, \label{eq::triangle-star}
    \end{equation}
    where
    \begin{equation*}
        \bigtriangleup^{*} := z^{T}X(\betaL-\beta) + \lambda_{\varepsilon} \|\beta\|_{1} - \lambda_{\varepsilon} \|\betaL\|_{1}.
    \end{equation*}
    In the remaining proof, let $u=\betaL-\beta$ and define
    \begin{equation*}
        \Tilde{H}(u) := \sqrt{1+\delta_{0}}(1+\deltanum{delta::4}) \bigg(4 \|u\|_{2} \Big(\sum_{j=1}^{k} \log (2p/j)\Big)^{1/2} + (1+\deltanum{delta::3}) \sqrt{2\log(p/k)}\sum_{j=k+1}^{p} |u|_{(j)} \bigg).
    \end{equation*}
    Using the Cauchy-Schwarz inequality and \eqref{eq::stirling},
    \begin{align}
        & \sqrt{1+\delta_{0}}H(u) \leq \Tilde{H}(u) \leq \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon}\frac{4+\sqrt{2}}{\sqrt{2}} \lambda_{\varepsilon} \sqrt{k} \|u\|_{2} \nonumber\\
        & + \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})(1+\deltanum{delta::3})}{1+\varepsilon}\lambda_{\varepsilon} \sum_{j=k+1}^{p} |u|_{(j)} := F(u), \label{eq::F(u)}
    \end{align}
    where $H(\cdot)$ is defined in \eqref{eq::H-G-function}, and the last inequality follows from \eqref{eq::lambda-epsilon}, \eqref{eq::stirling} and $4\sqrt{2\log(2ep/k)}\leq (4+\sqrt{2})/\sqrt{2}\cdot \sqrt{2\log(p/k)}$. Let $S:= \supp(\beta)$,
    \begin{equation}
        \|\beta\|_{1} - \|\betaL\|_{1} = \|\beta\|_{1} - \|\beta+u\|_{1} = \|\beta\|_{1} - \|\beta_{S} + u_{S}\|_{1} - \|u_{S^{c}}\|_{1} \leq \|u_{S}\|_{1} - \|u_{S^{c}}\|_{1}. \label{eq::l1-difference}
    \end{equation}
    Then, on the event \eqref{eq::stochastic-error-event}, using \eqref{eq::F(u)} and \eqref{eq::l1-difference} we have
    \begin{equation}\label{eq::bound-delta-star-1}
        \bigtriangleup^{*} \leq \lambda_{\varepsilon} \Big( \sqrt{k}\|u\|_{2} - \sum_{j=k+1}^{p} |u|_{(j)} \Big) + \max\big(F(u), \Tilde{G}(u)\big),
    \end{equation}
    where $G(u)$ is defined in \eqref{eq::H-G-function} and $\Tilde{G}(u): = \sqrt{1+\delta_{0}} G(u)$. Transforming $\tilde{G}(u)$ using \eqref{eq::delta(lambda)}, we have
    \begin{equation*}
        \Tilde{G}(u) = \sqrt{1+\delta_{0}}\lambda_{\varepsilon} \sqrt{k} \sqrt{\frac{\log(1/\deltanum{delta::5})}{k\log(1/\delta(\lambda_{\varepsilon}))}} \frac{1+\deltanum{delta::4}}{\deltanum{delta::4}} \|Xu\|_{2}.
    \end{equation*}
    From \eqref{eq::bound-delta-star-1}, we have the following discussion:
    \begin{itemize}
        \item If $\Tilde{G}(u)>F(u)$, this implies
        \begin{equation}
            \|u\|_{2} \leq \frac{\sqrt{2}}{4+\sqrt{2}} (1+\varepsilon) \frac{1}{\deltanum{delta::4}} \sqrt{\frac{\log(1/\deltanum{delta::5})}{k\log(1/\delta(\lambda_{\varepsilon}))}} \|Xu\|_{2}. \label{eq::u2-bounded-by-xu2}
        \end{equation}
        Therefore,
        \begin{align*}
            \bigtriangleup^{*} & \leq \lambda_{\varepsilon} \sqrt{k} \|u\|_{2} + \Tilde{G}(u) \\
            & \leq \lambda_{\varepsilon} \sqrt{k} \frac{\sqrt{2}}{4+\sqrt{2}} (1+\varepsilon) \frac{1}{\deltanum{delta::4}} \sqrt{\frac{\log(1/\deltanum{delta::5})}{k\log(1/\delta(\lambda_{\varepsilon}))}} \|Xu\|_{2} \\
            & + \lambda_{\varepsilon}\sqrt{k} \sqrt{1+\delta_{0}}(1+\deltanum{delta::4}) \frac{1}{\deltanum{delta::4}} \sqrt{\frac{\log(1/\deltanum{delta::5})}{k\log(1/\delta(\lambda_{\varepsilon}))}} \|Xu\|_{2} \\
            & = \bigg[ \sqrt{1+\delta_{0}}(1+\deltanum{delta::4}) + \frac{\sqrt{2}}{4+\sqrt{2}}(1+\varepsilon) \bigg] \frac{1}{\deltanum{delta::4}} \lambda_{\varepsilon} \sqrt{k} \sqrt{\frac{\log(1/\deltanum{delta::5})}{k\log(1/\delta(\lambda_{\varepsilon}))}} \|Xu\|_{2}.
        \end{align*}
        Combining the above with \eqref{eq::triangle-star},
        \begin{equation*}
            \|Xu\|_{2} \leq \bigg[ \sqrt{1+\delta_{0}}(1+\deltanum{delta::4}) + \frac{\sqrt{2}}{4+\sqrt{2}}(1+\varepsilon) \bigg] \frac{1}{\deltanum{delta::4}} \lambda_{\varepsilon} \sqrt{k} \sqrt{\frac{\log(1/\deltanum{delta::5})}{k\log(1/\delta(\lambda_{\varepsilon}))}}.
        \end{equation*}
        Then, connecting the above with \eqref{eq::u2-bounded-by-xu2}, we have
        \begin{align}
            \|\betaL - \beta\|_{2} & \leq \frac{\sqrt{2}}{4+\sqrt{2}} (1+\varepsilon) \frac{1}{\deltanum{delta::4}} \sqrt{\frac{\log(1/\deltanum{delta::5})}{k\log(1/\delta(\lambda_{\varepsilon}))}} \nonumber \\
            & \cdot \bigg[ \sqrt{1+\delta_{0}} (1+\deltanum{delta::4}) + \frac{\sqrt{2}}{4+\sqrt{2}}(1+\varepsilon) \bigg] \frac{1}{\deltanum{delta::4}} \lambda_{\varepsilon} \sqrt{k} \sqrt{\frac{\log(1/\deltanum{delta::5})}{k\log(1/\delta(\lambda_{\varepsilon}))}} \nonumber \\
            & = \frac{\sqrt{2}}{4+\sqrt{2}} (1+\varepsilon) \bigg[ \sqrt{1+\delta_{0}}(1+\deltanum{delta::4}) + \frac{\sqrt{2}}{4+\sqrt{2}}(1+\varepsilon) \bigg] \frac{1}{\deltanum{delta::4}^{2}} \frac{\log(1/\deltanum{delta::5})}{k\log(1/\delta(\lambda_{\varepsilon}))} \lambda_{\varepsilon} \sqrt{k}. \label{eq::casei-l2bound}
        \end{align}

        \item If $\Tilde{G}(u)\leq F(u)$, replacing the maximum with $F(u)$, we obtain
        \begin{align*}
            \bigtriangleup^{*} & \leq \lambda_{\varepsilon}  \Big( \sqrt{k}\|u\|_{2} - \sum_{j=k+1}^{p} |u|_{(j)} \Big) \\
            & + \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} \lambda_{\varepsilon} \sqrt{k} \|u\|_{2} + \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})(1+\deltanum{delta::3})}{1+\varepsilon}\lambda_{\varepsilon} \sum_{j=k+1}^{p} |u|_{(j)}\\
            & = \bigg(1+ \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} \bigg) \lambda_{\varepsilon}\sqrt{k}\|u\|_{2} - \bigg( 1 -\frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})(1+\deltanum{delta::3})}{1+\varepsilon} \bigg) \lambda_{\varepsilon} \sum_{j=k+1}^{p}|u|_{(j)} \\
            & =: \bigtriangleup.
        \end{align*}
        From \eqref{eq::triangle-star}, we know $\bigtriangleup \geq \bigtriangleup^{*} \geq 0$ almost surely. As a result, from the above equations, $u=\betaL - \beta \in \mathcal{C}_{SRE}(k, c_{0})$, where
        \begin{equation*}
            c_{0} := \bigg( 1+\frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}}\bigg) / \bigg( 1 - \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})(1+\deltanum{delta::3})}{1+\varepsilon} \bigg).
        \end{equation*}
        Note that by the assumption of this lemma, we have selected $\deltanum{delta::3}$, $\deltanum{delta::4}$ such that the above $c_{0}>0$.Thus, we can apply $SRE(k,c_{0})$ and have
        \begin{equation}
            \|\betaL-\beta\|_{2} \leq \frac{\|Xu\|_{2}}{\theta(k,c_{0})} \leq \bigg( \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} + 1 \bigg) \lambda_{\varepsilon}\sqrt{k} \frac{\|Xu\|_{2}}{\theta^{2}(k,c_{0})}, \label{eq::caseii-l2bound}
        \end{equation}
        where the second inequality is due to
        \begin{align*}
            \|Xu\|_{2}^{2} \leq \bigtriangleup^{*} \leq \bigg( \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} + 1 \bigg) \lambda_{\varepsilon} \sqrt{k} \frac{\|Xu\|_{2}}{\theta(k,c_{0})}.  
        \end{align*}
        Combining \eqref{eq::casei-l2bound} and \eqref{eq::caseii-l2bound}, we have
        \begin{equation}
            \|\betaL-\beta\|_{2} \leq C(k,\lambda_{\varepsilon}, \deltanum{delta::5}) \lambda_{\varepsilon} \sqrt{k},
        \end{equation}
        with
        \begin{equation*}
            C(k,\lambda_{\varepsilon},\deltanum{delta::5}) := \bigg( \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} + 1 \bigg) \cdot \bigg( \frac{1}{\deltanum{delta::4}^{2}}\frac{\log(1/\deltanum{delta::5})}{k\log(1/\delta(\lambda_{\varepsilon}))} \vee \frac{1}{\theta^{2}(k,c_{0})} \bigg).
        \end{equation*}
    \end{itemize}

\end{proof}



\begin{lemma}[Bound on the stochastic error]\label{lem::bound-on-stochastic-error}
    Let $\deltanum{delta::5}\in(0,1)$ and $z\sim \calN(0,I_{n})$ and $X\in \R^{n\times p}$ be a fixed matrix such that $\max_{j\in [p]} \|Xe_{j}\|_{2} \leq \sqrt{1+\delta_{0}}$, then
\begin{equation}
    \Big \{ z^{T}Xu \leq \sqrt{1+\delta_{0}}\cdot \max\big ( H(u), G(u) \big), ~ \forall u \in \R^{p} \Big\} \label{eq::stochastic-error-event}
\end{equation}
holds with probability at least $1-\deltanum{delta::5}/2$.
\end{lemma}

\begin{proof}
Because of the scalability, we prove it for $\max_{j\in [p]} \|Xe_{j}\|_{2} \leq 1$. For $\deltanum{delta::3} \in (0,1)$, let 
    \begin{equation*}
        N(u):= \sum_{j=1}^{k}|u|_{(j)} 4\sqrt{\log (2p/j)} +  (1+\deltanum{delta::3}) \sum_{j=k+1}^{p} |u|_{(j)} \sqrt{2\log (p/k)}.     
    \end{equation*}
    Let $g_{j} = z^{T}Xe_{j}$, $j=1\ldots, p$. We have
    \begin{align*}
        \sup_{N(u)\leq 1} z^{T}Xu & \leq \sup_{N(u)\leq 1} \bigg[ \sum_{j=1}^{k} 4 \sqrt{\log(2p/j)} ~|u|_{(j)} ~ \frac{|g|_{j}}{4\sqrt{\log(2p/j)}} \\
        & + \sum_{j=k+1}^{p} (1+\deltanum{delta::3}) \sqrt{2\log(p/k)} ~|u|_{(j)} ~ \frac{|g|_{(j)}}{(1+\deltanum{delta::3})\sqrt{2\log(p/k)}} \bigg]\\
        & \leq \Big( \max_{1\leq j\leq k} \frac{|g|_{(j)}}{4\sqrt{\log(2p/j)}} \Big) \vee \Big( \max_{k+1\leq j\leq p} \frac{|g|_{(j)}}{(1+\deltanum{delta::3})\sqrt{2\log(p/k)}} \Big) \\
        & = \Big( \max_{1\leq j\leq k} \frac{|g|_{(j)}}{4\sqrt{\log(2p/j)}} \Big) \vee \frac{|g|_{(k+1)}}{(1+\deltanum{delta::3})\sqrt{2\log(p/k)}}.
    \end{align*}

    For $L>0$ to be determined, let $T:=\{u\in \R^{p}: \max\Big(N(u), \frac{1}{L}\|Xu\|_{2}\Big) \leq 1\}$. Note that $f(v):= \sup_{u\in T}v^{T}Xu$ is a Lipschitz function with Lipschitz constant $L$. By the concentration of the Lipschitz function of Gaussian distribution around the median (for example, Inequality (1.4) in \cite{ledoux1991probability}), we have with probability at least $1-\deltanum{delta::5}/2$,
    \begin{align*}
        \sup_{u\in T} z^{T}Xu & \leq \Med\bigg[ \sup_{u\in T} z^{T}Xu \bigg] + L \sqrt{2 \log (1/\deltanum{delta::5})} \\
        & \leq \Med \bigg[ \sup_{N(u)\leq 1} z^{T}Xu \bigg] + L\sqrt{2\log(1/\deltanum{delta::5})} \\
        & \leq 1 + \deltanum{delta::4},
    \end{align*}
    where in the last inequality we have let $L=\deltanum{delta::4}/\sqrt{2\log(1/\deltanum{delta::5})}$ and used Lemma \ref{lem::median-inequality}. 
\end{proof}




\begin{proof}[{Proof of Lemma \ref{lem::lasso-MSE-bound}}]
From \eqref{eq::constant_in_lasso_2norm_bound},
\begin{equation}
    C(k,\lambda_{\varepsilon},\deltanum{delta::5}) \geq \bigg( \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} + 1 \bigg) \frac{1}{\theta^{2}(k,c_{0})}. \label{eq::lower-bound-C_gamma}
\end{equation}
    Then $\deltanum{delta::5}^{*}:= \exp\Big( \frac{k\deltanum{delta::4}^{2}}{\theta^{2}(k,c_{0})} \log (1/\delta(\lambda_{\varepsilon}))  \Big)$ is the smallest $\deltanum{delta::5}>0$ such that the equality in \eqref{eq::lower-bound-C_gamma} holds. From \eqref{eq::lasso-l2bound}, for $t\geq \log(1/\deltanum{delta::5}^{*}):=T$,
    \begin{equation*}
        Z := \bigg( \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} + 1 \bigg)^{-1} \frac{\deltanum{delta::4}^{2}k\log(1/\delta(\lambda_{\varepsilon}))}{\lambda_{\varepsilon}\sqrt{k}} \|\betaL-\beta\|_{2} \leq t,
    \end{equation*}
    with probability at least $1-(e^{-t})/2$. Thus, for any $q>2$,
    \begin{align*}
        \E Z^{q} = \int_{0}^{\infty} q t^{q-1} P(Z>t) d t \leq \int_{0}^{T} qt^{q-1} d t + \int_{T}^{\infty} qt^{q-1}\frac{e^{-t}}{2} dt \leq T^{q} + \frac{q}{2}\Gamma(q) = T^{q} +C_{q},
    \end{align*}
    where $\Gamma(\cdot)$ is the Gamma function. Thus, under the $SRE(k,c_{0})$ condition, we obtain
    \begin{equation*}
        \E \|\hat{\beta}-\beta\|_{2}^{q} \leq \bigg( \frac{\sqrt{1+\delta_{0}}(1+\deltanum{delta::4})}{1+\varepsilon} \frac{4+\sqrt{2}}{\sqrt{2}} + 1 \bigg)^{q} \Big(\frac{\lambda_{\varepsilon}\sqrt{k}}{\deltanum{delta::4}^{2}}\Big)^{q} \Big[\frac{1}{\theta^{2q}(k,c_{0})} + \frac{C_{q}}{(\deltanum{delta::4}^{2}k\log(p/k))^{q}}\Big].
    \end{equation*}
\end{proof}


The following lemmas are auxiliary to prove Lemmas \ref{lem::lasso-l2-bound} and \ref{lem::lasso-MSE-bound} and Proposition \ref{prop::lasso-MSE-bound}. Some of them are based on \cite{bellec2018slope}. We skip those proofs to prevent duplicate work.



\begin{lemma}[Proposition E.1 in \cite{bellec2018slope}]\label{lem::prop-E.1}
    Let $g_{1}, \ldots, g_{p}$ be standard Gaussian random variables. Denote by $\Big(|g|_{(1)}, \ldots, |g|_{(p)}\Big)$ the non-increasing rearrangement of $\Big(|g_{1}|, \ldots, |g_{p}|\Big)$. Then for any $s\in \{1\ldots,p\}$ and all $t>0$, we have
    \begin{equation*}
        P\bigg( \frac{1}{s} \sum_{j=1}^{s} |g|_{(j)}^{2} > t \log (2p/s) \bigg) \leq (2p/s)^{1-3t/8}.
    \end{equation*}
\end{lemma}

The proof of the next lemma follows that of Proposition E.2 in \cite{bellec2018slope}. 
\begin{lemma}\label{lem::median-inequality}
    Under the assumptions of Lemma \ref{lem::prop-E.1}, assume $k/p \rightarrow 0$, then
    \begin{align*}
        & P \bigg( \Big( \max_{1\leq j\leq k} \frac{|g|_{(j)}}{4\sqrt{\log(2p/j)}} \Big) \vee \frac{|g|_{(k+1)}}{(1+\deltanum{delta::3})\sqrt{2\log(p/k)}} \leq 1 \bigg) \\
        & \geq 1 - \frac{k}{2p} - \exp\big[ - C\cdot \deltanum{delta::3}k\sqrt{2\log(p/k)} \big] \geq \frac{1}{2},
    \end{align*}
    for any $\deltanum{delta::3} \geq C/(k\sqrt{2\log(p/k)})$ with some $C>0$.
\end{lemma}

\begin{proof}
    Lemma \ref{lem::prop-E.1} with $t=16/3$ and the inequality $|g|_{(j)}^{2} \leq \frac{1}{j}\sum_{l=1}^{j}|g|_{(l)}^{2}$ imply 
    \begin{equation}
        P \bigg( |g|_{(j)}^{2} \leq \frac{16}{3} \log (2p/j) \bigg) \geq 1 -\frac{j}{2p}, \quad j=1,\ldots, p. \label{eq::gaussian-order-stat-16/3-concent}
    \end{equation}
    Let $q\geq 0$ be an integer such that $2^{q} \leq k < 2^{q+1}$. Applying \eqref{eq::gaussian-order-stat-16/3-concent} to $j=2^{l}$ for $l=0, \ldots, q-1$ and using the union bound, we obtain that the event
    \begin{equation*}
        \Omega_{0} := \bigg\{ \max_{l=0,\ldots, q-1} \frac{|g|_{(2^{l})}\sqrt{3}}{4\sqrt{\log(2p/2^{l})}} \leq 1 \bigg\}
    \end{equation*}
    satisfies $P(\Omega_{0}) \geq 1 - \sum_{l=0}^{q-1} \frac{2^{l}}{2p} = 1 - \frac{2^{q-1}}{2p} \geq 1 - \frac{k}{2p}$. For any $j< 2^{q}$, there exists $l\in\{0, \ldots, q-1\}$ such that $2^{l}\leq j < 2^{l+1}$. On the event $\Omega_{0}$,
    \begin{equation*}
        |g|_{(j)} \leq |g|_{(2^{l})} \leq \frac{4}{\sqrt{3}} \sqrt{\log \frac{2p}{2^{l}}} \leq \frac{4}{\sqrt{3}} \sqrt{\log \frac{4p}{j}} \leq 4 \sqrt{\log \frac{2p}{j}}, \quad \forall j <2^{q}.
    \end{equation*}
    And for $2^{q}\leq j \leq k$,
    \begin{equation*}
        |g|_{(j)} \leq |g|_{2^{q-1}} \leq \frac{4}{\sqrt{3}} \sqrt{\log \frac{2p}{2^{q-1}}} < \frac{4}{\sqrt{3}} \sqrt{\log \frac{8p}{j}} \leq 4 \sqrt{\log \frac{2p}{j}}.
    \end{equation*}
    Thus, on the event $\Omega_{0}$ we have $|g|_{(j)} \leq 4 \sqrt{\log (2p/j)}$ for all $j=1,\ldots, k$. 

    In addition, using Lemma \ref{lem::Gaussian-order-statistics}, we have
    \begin{equation*}
        P\bigg( \frac{|g|_{(k+1)}}{(1+\deltanum{delta::3})\sqrt{2\log \frac{p}{k}}} \geq 1 \bigg) \leq \exp \Big[ -kC\deltanum{delta::3}\sqrt{2\log (p/k)} \Big].
    \end{equation*}
\end{proof}


















==> unified_1st_order_lower_bound.tex <==
\section{A unified first order lower bound proposition}\label{sec::unified-1st-order-lower}

% The following proposition provides a unified lower bound for the minimax risk in different SNR regimes.

\textcolor{teal}{Yilin: The following proposition can then be adapted in all three regimes with the following selections of spike $\mu$. Here, $\mu$ is used as a single parameter for the prior spike. (When I wrote this proposition, I haven't used $\mu$ for the SNR symbol.) For Regime (I) \& (II), the spike $\mu$ is selected to be the boundary SNR described in $\Theta(k,\tau)$. For Regime (III), the spike $\mu$ can an arbitrary choice satisfying $\sqrt{2\log(p/k)}-\mu \rightarrow +\infty$ and $\mu = \sqrt{2\log(p/k)} \cdot (1+o(1))$.}

\begin{proposition}\label{prop::unified-first-order-lower-bound}
    Assume model \eqref{model::gaussian-model}, $n, p/k \rightarrow \infty$ and $(\log (p/k))/n \rightarrow 0$. Let $\lambda>0$ and $\pi:= \pi^{\lambda, p,k}$ be the independent block prior of $\beta$ with the spike $\lambda$ satisfying $\sqrt{2\log (p/k)} - \lambda \rightarrow +\infty$. Let $\hat{\beta}_{\pi}$ denote the Bayesisan estimator of $\beta$ under $\pi$. Then,
    \begin{equation*}
        \E_{\pi}\|\hat{\beta}_{\pi} - \beta\|^{2} \geq (1+o(1)) \cdot \sigma^{2} k \lambda^{2}.
    \end{equation*}
\end{proposition}
\begin{proof}
    Using the scalability of the model and the squared loss, it is equivalent to prove for the unit variance noise model. Let $\sigma = 1$ in model \eqref{model::gaussian-model}. Let $m:= \lceil p/k \rceil$. Let $\pi_{S}^{\lambda, m}$ be the single spike prior of $\beta\in \R^{m}$, $\pi_{S}^{\lambda, m}(\beta^{(j)} = \lambda e_{i}) = \frac{1}{m}$. Write $\beta = (\beta^{(1)}, \beta^{-1})$ where $\beta^{(1)} \in \R^{m}$ and $\beta^{(-1)} \in \R^{p-m}$. Accordingly, $X= \big(X^{(1)}, X^{(-1)}\big)^{T}$ with $X^{(1)} \in \R^{n\times m}$ and $X^{(-1)}\in \R^{n\times (p-m)}$. Let $\Tilde{y}= y-X^{(-1)}\beta^{(-1)}$. Then
\begin{equation*}
    B(\pi_{IB}^{\lambda, p, k}) = \E_{\pi} \|\hat{\beta}_{\pi} - \beta\|^{2} \geq k \cdot \E_{\pi} \|\E_{\pi} \big( \beta^{(1)} \big | \Tilde{y}, X^{(1)} \big) - \beta^{(1)}\|^{2} = k\cdot B(\pi_{S}^{\lambda, m}).
\end{equation*}
As $p/k \rightarrow \infty$ and $(\log (p/k))/n \rightarrow 0$, we can apply Lemma \ref{lem::spike-prior-lower-bound} on the Bayesian risk of $\beta^{(1)}$. We have
\begin{equation*}
    B(\pi_{IB}^{\lambda, p, k}) \geq k\cdot B(\pi_{S}^{\lambda, m}) \geq k \lambda^{2} (1+o(1)).
\end{equation*}
\end{proof}

\begin{lemma}\label{lem::spike-prior-lower-bound}
    Consider model \eqref{model::gaussian-model} with $\sigma=1$ and $\beta\in \R^{m}$. Suppose $n, m \rightarrow \infty$ and $(\log m)/ n \rightarrow 0$. Let $\pi=\pi_{S}(\lambda;m)$ be the single spike prior of $\beta$. Denote $\hat{\beta}_{\pi}$ as the Bayesian estimator under $\pi$. For $\lambda>0$ satisfying $\sqrt{2\log m} - \lambda \rightarrow \infty$, we have
\begin{equation*}
    \E_{\pi}\|\hat{\beta}_{\pi} - \beta\|^{2} \geq \lambda^{2} (1+o(1)).
\end{equation*}
\end{lemma}
\begin{proof}
    Under the single spike prior, let $I\in [m]$ denote the selected spike index, the posterior probability that the first coordinate is selected is
\begin{equation*}
    p_{1}:= P(I=1~|~ y, X) = \frac{\exp(\lambda x_{1}^{T}y - \lambda^{2}\|x_{1}\|^{2}/2)}{\exp(\lambda x_{1}^{T}y - \lambda^{2}\|x_{1}\|^{2}/2) + \sum_{i=2}^{m} \exp (\lambda x_{i}^{T}y - \lambda^{2}\|x_{i}\|^{2}/2)}.
\end{equation*}
Then,
\begin{eqnarray*}
    \E_{\pi}\|\hat{\beta}_{\pi} - \beta\|^{2} &=& \lambda^{2} \E_{\lambda e_{1}} \big( 1-p_{1} \big)^{2} + \lambda^{2}(m-1)\E_{\lambda e_{2}} p_{1}^{2} \\
    &\geq& \lambda^{2}\E_{\lambda e_{1}}\big( 1-p_{1} \big)^{2}.
\end{eqnarray*}
From Lemma \ref{lem::first-posterior-probability-goes-to-zero}, 
\begin{equation*}
    p_{1}(y,X) \rightarrow 0 \quad \text{in } P_{\lambda e_{1}}\text{-probability}.
\end{equation*}
Therefore, since $0\leq p_{1}\leq 1$, by continuous mapping and bounded convergence theorems, we have
\begin{equation*}
    \E_{\pi}\|\hat{\beta}_{\pi} - \beta\|^{2} \geq \lambda^{2} (1+o(1)).
\end{equation*}
\end{proof}

\begin{lemma}\label{lem::first-posterior-probability-goes-to-zero}
    Assume model \eqref{model::gaussian-model} with $\sigma=1$, $n, m \rightarrow \infty$ and $(\log m)/ n \rightarrow 0$. Suppose $\lambda>0$ and $\sqrt{2\log m} - \lambda \rightarrow +\infty$. Let $\beta = \lambda e_{1}$. Then
\begin{equation*}
    p_{1}(y,X) := \frac{\exp(\lambda x_{1}^{T}y - \lambda^{2}\|x_{1}\|^{2}/2)}{\exp(\lambda x_{1}^{T}y - \lambda^{2}\|x_{1}\|^{2}/2) + \sum_{i=2}^{m} \exp (\lambda x_{i}^{T}y - \lambda^{2}\|x_{i}\|^{2}/2)} \rightarrow 0 \quad \text{in } P_{\lambda e_{1}}\text{-probability}.
\end{equation*}
\end{lemma}
\begin{proof}
    Under $P_{\lambda e_{1}}$, using the independence of $\{x_{i}: ~i=2,\ldots ,m\}$ and $\lambda x_{1} + z$,
\begin{eqnarray*}
    p_{1}^{(\lambda e_{1})} &=& \Bigg[ 1 + \frac{\sum_{i=2}^{m} \exp\Big( \lambda x_{i}^{T} (\lambda x_{1}+ z) - \lambda^{2}\|x_{i}\|^{2}/2 \Big)}{\exp\Big( \lambda^{2} \|x_{1}\|^{2}/2 + \lambda x_{1}^{T}z \Big)} \Bigg]^{-1} \\
    &\overset{d}{=}& \Bigg[ 1 + \frac{\sum_{i=2}^{m}\exp\Big( \|\lambda x_{1}+ z\|\lambda x_{i,1} - \lambda^{2} x_{i,1}^{2}/2 - \lambda^{2}\|x_{i,-1}\|^{2}/2\Big)}{\exp\Big( \lambda^{2}\|x_{1}\|^{2}/2 + \lambda x_{1}^{T}z\Big)} \Bigg]^{-1} \\
    &=& \big[1+\mathcal{A}_{n,m}\mathcal{B}_{n,m}\big]^{-1}.
\end{eqnarray*}
where
\begin{align*}
    & \mathcal{A}_{n,m} = \frac{\sum_{i=2}^{m} \exp\left( \|\lambda x_{1} + z\| \lambda x_{i,1} - \frac{\lambda^{2}}{2} x_{i,1}^{2} - \frac{\lambda^{2}}{2} \|x_{i,-1}\|^{2} \right)}{(m-1) (1+\frac{\lambda^{2}}{n})^{-\frac{n}{2}} \exp\left( \frac{1}{2} \frac{1}{1+n/\lambda^{2}} \|z+\lambda x_{1}\|^{2} \right) },  \\
    & \mathcal{B}_{n,m} = \frac{(m-1) (1+\frac{\lambda^{2}}{n})^{-\frac{n}{2}} \exp\left( \frac{1}{2} \frac{1}{1+n/\lambda^{2}} \|z+\lambda x_{1}\|^{2} \right)}{\exp\left( \frac{\lambda^{2}}{2}\|x_{1}\|^{2} + \lambda x_{1}^{T}z \right)}. 
\end{align*}
From Lemmas \ref{lem::A-term-convergest-to-one} and \ref{lem::B-term-converges-to-infty},
\begin{equation*}
    \mathcal{A}_{n,m} \overset{p}{\rightarrow} 1, \text{ and } \mathcal{B}_{n,m} \overset{p}{\rightarrow} +\infty. 
\end{equation*}
Thus, it follows that
\begin{equation*}
    p_{1}(y,X) \rightarrow 0 \quad \text{in } P_{\lambda e_{1}}\text{-probability}.
\end{equation*}
\end{proof}





\begin{lemma} \label{lem::A-term-convergest-to-one}
    Assume $x_{1}, \ldots, x_{m} \simiid \calN(0, \frac{1}{n}I_{n})$, $z\sim \calN(0, I_{n})$ and $\{x_{i}: i=1,\ldots,m\}$ being independent with $z$. Suppose $n, m\rightarrow \infty$, $(\log m)/n \rightarrow 0$ and $0<\lambda = O(\sqrt{\log m})$. Let $\mathcal{A}_{n,m}$ be defined in \eqref{term::A-first-order-spike}. We have 
    \begin{equation*}
        \mathcal{A}_{n,m} := \frac{\sum_{i=2}^{m} \exp\left( \|\lambda x_{1} + z\| \lambda x_{i,1} - \frac{\lambda^{2}}{2} x_{i,1}^{2} - \frac{\lambda^{2}}{2} \|x_{i,-1}\|^{2} \right)}{(m-1) (1+\frac{\lambda^{2}}{n})^{-\frac{n}{2}} \exp\left( \frac{1}{2} \frac{1}{1+n/\lambda^{2}} \|z+\lambda x_{1}\|^{2} \right) } \overset{p}{\rightarrow}1.
    \end{equation*}
\end{lemma}

\begin{proof}
Define
\begin{equation*}
    S_{n,m} := \sum_{i=2}^{m} \exp\Big[ \|\lambda x_{1} + z\|\lambda x_{i,1} - \frac{\lambda^{2}}{2}x_{i,1}^{2} - \frac{\lambda^{2}}{2}\|x_{i,-1}\|^{2} \Big].
\end{equation*}
Let
\begin{equation*}
    Y_{m,i} := \exp\Big[ \|\lambda x_{1} + z\|\lambda x_{i,1} - \frac{\lambda^{2}}{2}x_{i,1}^{2} - \frac{\lambda^{2}}{2}\|x_{i,-1}\|^{2} \Big].
\end{equation*}
We will utilize the weak law of triangular arrays in Lemma \ref{lem::WLLN-triangular}. Note that $\{Y_{m,i}: i=2,\ldots, n\}$ are independent only if conditioning on $\|\lambda x_{1}+z\|$. Hence, instead, we will prove, for certain $b_{n,m}$ to be determined,
\begin{enumerate}[label=(\roman*)]
    \item $\sum_{i=2}^{m}P\Big(Y_{m,i}>b ~\Big|\|\lambda x_{1}+z\| \Big) \rightarrow 0 $ a.s..
    \item $b^{-2} \sum_{i=2}^{m} \E \Big [ Y_{m,i}^{2} \mathbbm{1}_{(Y_{m,i}\leq b)} ~\Big| \|\lambda x_{1} + z\| \Big] \rightarrow 0$ a.s..
\end{enumerate}
For simplicity, without ambiguity, we write $b=b_{n,m}$ in the following proof.

To prove condition (i), using Lemma \ref{lem::wlln-conditions-lemma} (i) and applying the non-central $\chi^{2}$ inequality in Lemma \ref{lem::concentration-non-central-chisquare},
\begin{eqnarray}
    && \sum_{i=2}^{m} P\Big(Y_{m,i}>b ~\Big|\|\lambda x_{1}+z\| \Big) \nonumber\\
    &=& (m-1) P \bigg[ \Big( \sqrt{n}x_{i,1} - \frac{\sqrt{n}}{\lambda} \|\lambda x_{1}+ z\| \Big)^{2} + \Big(\sqrt{n} \|x_{i,-1}\|\Big)^{2} < \frac{n}{\lambda^{2}} \Big( \|\lambda x_{1}+z\|^{2} -2\log b \Big) ~\Big | \|\lambda x_{1}+z\| \bigg] \nonumber\\
    &=& (m-1) P \bigg( \chi_{n}^{2}(\gamma_{1}) < \frac{n}{\lambda^{2}} \big( \|\lambda x_{1} + z\|^{2} -2\log b \big) ~\Big| \|\lambda x_{1}+z\| \bigg) \nonumber\\
    & \leq & (m-1) \exp \bigg[ - \frac{n c_{1}^{2}}{4(n+2\gamma_{1})^{2}} \bigg] \nonumber\\
    &=& \exp \bigg[ - \frac{n}{4(n+2\gamma_{1})^{2}}\Big( c_{1} - \frac{2(n+2\gamma_{1})}{\sqrt{n}}\sqrt{\log(m-1)} \Big)\Big( c_{1} + \frac{2(n+2\gamma_{1})}{\sqrt{n}}\sqrt{\log(m-1)} \Big) \bigg]. \label{eq::upp-bound-cond-i}
\end{eqnarray}
where $c_{1}= n+ n/\lambda^{2} \cdot 2\log b$ and $\gamma_{1} = n/\lambda^{2} \cdot \|\lambda x_{1} + z\|^{2}$. Since $\lambda^{2} = o(n)$, by strong law of large numbers,
\begin{equation*}
    \frac{1}{n} \| \lambda x_{1} + z \|^{2} \rightarrow 1 \text{ a.s..}
\end{equation*}
Thus, $n+2\gamma_{1} = n \cdot \frac{n}{\lambda^{2}} \big( 1+o_{p}(1) \big)$. A sufficient condition for the upper bound in \eqref{eq::upp-bound-cond-i} goes to zero a.s. is 
\begin{equation*}
    \bigg[ \frac{n}{4(n+2\gamma_{1})^{2}} \frac{2(n+\gamma_{1})}{\sqrt{n}} \sqrt{\log (m-1)} \bigg]^{-1} = o_{p} \bigg( c_{1} - \frac{2(n+2\gamma_{1})}{\sqrt{n}}\sqrt{\log (m-1)} \bigg),
\end{equation*}
or
\begin{equation}
    4\sqrt{\frac{n}{\log (m-1)}} = o_{p} \bigg( 2\log b - \frac{2(\lambda^{2}+2\|\lambda x_{1} + z\|^{2} )}{\sqrt{n}}\sqrt{\log (m-1)} \bigg). \label{eq::b-selection}
\end{equation}
There exists such choice of $b$ since 
\begin{equation}
    \frac{2(\lambda^{2}+2\gamma_{1})}{\sqrt{n}} \sqrt{\log (m-1)} \frac{\lambda^{2}}{n} = \frac{2(\lambda^{2} +2\|\lambda x_{1} + z\|^{2})}{\sqrt{n}} \sqrt{\log (m-1)} = 4 \sqrt{n \log (m-1)} \big(1+o_{p}(1)) \label{eq::b-selection-cond-ii}
\end{equation}
as $\lambda^{2} = o(n)$ and $\log (m-1) \rightarrow \infty$. Therefore, condition (i) is satisfied.

To prove condition (ii), using Lemma \ref{lem::wlln-conditions-lemma} (ii) and applying Lemma \ref{lem::concentration-non-central-chisquare}, we have
\begin{eqnarray*}
    && b^{-2}\sum_{i=2}^{m} \E \Big[ Y_{m,i}^{2} \mathbbm{1}_{(Y_{m,i}\leq b)} ~ \Big | \|\lambda x_{1} + z\| \Big] \\
    &=& b^{-2} (m-1) \Big(1+\frac{2\lambda^{2}}{n}\Big)^{-n/2} \exp \bigg( \frac{2\|\lambda x_{1}+ z\|^{2}}{2+n/\lambda^{2}} \bigg) \\
    && \cdot P\bigg[ \Big(Z - \frac{n/\lambda^{2}}{\sqrt{2+n/\lambda^{2}}} \|z+\lambda x_{1}\| \Big)^{2} + \chi_{n-1}^{2} \geq \Big(2 +n/\lambda^{2}\Big)\Big(\|\lambda x_{1} + z\|^{2} - 2\log b \Big) ~\Big | \|\lambda x_{1}+z\| \bigg] \\
    &\leq& b^{-2} (m-1)  \Big(1+\frac{2\lambda^{2}}{n}\Big)^{-n/2} \exp \bigg( \frac{2\|\lambda x_{1}+ z\|^{2}}{2+n/\lambda^{2}} \bigg) \\
    &=& \exp \bigg[ -2\log b + \log (m-1) -\lambda^{2} + \frac{2\|\lambda x_{1}+ z\|^{2}}{2+n/\lambda^{2}} \bigg].
\end{eqnarray*}
Since $\lambda = O(\sqrt{\log m})$ and $\log m = o(n)$,  we have $\frac{\|\lambda x_{1} + z\|^{2}}{2+n/\lambda^{2}}=\lambda^{2}\big( 1+o_{p}(1) \big)$, $\lambda^{2} = o(\sqrt{n\cdot \log m})$ and $\log (m-1) = o(\sqrt{n \log m})$. For $b$ satisfying \eqref{eq::b-selection}, \eqref{eq::b-selection-cond-ii}, $\sqrt{n\cdot \log m}= O_{p} (2\log b)$. Therefore, 
\begin{equation*}
    \exp \bigg[ -2\log b + \log (m-1) -\lambda^{2} + \frac{2\|\lambda x_{1}+ z\|^{2}}{2+n/\lambda^{2}} \bigg] \rightarrow 0 \text{ a.s..}
\end{equation*}
Thus, condition (ii) is satisfied. 

Finally, we calibrate 
\begin{equation*}
    a_{n,m}:= \sum_{i=2}^{m} \E \Big[ Y_{m,i} \mathbbm{1}_{(Y_{m,i}\leq b)} ~\Big| \|\lambda x_{1}+z\|\Big].
\end{equation*}
From Lemma \ref{lem::wlln-conditions-lemma} (iii), we have
\begin{equation*}
    a_{n,m} = (m-1) \Big(1 +\lambda^{2}/n \Big)^{-n/2} \exp\bigg( \frac{\|\lambda x_{1} + z\|^{2}}{2(1+n/\lambda^{2})} \bigg) \bigg( 1- P\Big[ \chi_{n}^{2} (\gamma_{2}) \leq n+\gamma_{2}-c_{2} ~\Big | \|\lambda x_{1} + z \| \Big] \bigg), \label{eq::a_n_p_definition}
\end{equation*}
where $c_{2}= (1+n/\lambda^{2})\cdot2\log b + n - \frac{1+2n/\lambda^{2}}{1+n/\lambda^{2}} \|\lambda x_{1} + z\|^{2}$ and $\gamma_{2} = \frac{(n/\lambda^{2})^{2}}{1+n/\lambda^{2}}\|\lambda x_{1} + z\|^{2}$.
We will show that
\begin{equation*}
    P\Big[ \chi_{n}^{2} (\gamma_{2}) \leq n+\gamma_{2}-c_{2} ~\Big | \|\lambda x_{1} + z \| \Big] \rightarrow 0 \text{ a.s..}
\end{equation*}
Using Lemma \ref{lem::concentration-non-central-chisquare}, we have
\begin{equation*}
    P\Big[ \chi_{n}^{2} (\gamma_{2}) \leq n+\gamma_{2}-c_{2} ~\Big | \|\lambda x_{1} + z \| \Big] \leq \exp \bigg[ - \bigg( \frac{\sqrt{n}c_{2}}{2(n+\gamma_{2})} \bigg)^{2} \bigg].
\end{equation*}
As $\frac{1}{n}\|\lambda x_{1} + z\|^{2} \rightarrow 1$ a.s., $\gamma_{2} = \frac{n}{\lambda^{2}} \big(1+o_{p} (1)\big)$. Using the selection of $b$ in \eqref{eq::b-selection} and \eqref{eq::b-selection-cond-ii}, $\frac{n}{\lambda^{2}}\sqrt{n\log m}=O_{p}(c_{2})$. Thus, $\sqrt{\log m} = O_{p} \Big( \frac{\sqrt{n}c_{2}}{2(n+\gamma_{2})} \Big)$. As $m\rightarrow \infty$, we have 
\begin{equation*}
    \exp \bigg[ - \bigg( \frac{\sqrt{n}c_{2}}{2(n+\gamma_{2})} \bigg)^{2} \bigg] \rightarrow 0 \text{ a.s..}
\end{equation*}
Thus,
\begin{equation*}
    a_{n,m} = (m-1) \bigg(1+\frac{\lambda^{2}}{n}\bigg)^{-\frac{n}{2}}  \exp\bigg( \frac{\|\lambda x_{1} + z\|^{2}}{2(1+n/\lambda^{2})} \bigg) \cdot \big(1+o_{p}(1)\big).
\end{equation*}
Now, we use Lemma \ref{lem::WLLN-triangular} with the bounded convergence theorem to obtain, $\forall \epsilon > 0$,
\begin{equation*}
    P\bigg( \bigg| \frac{S_{n,m}-a_{n,m}}{b_{n,m}}\bigg| > \epsilon \bigg) = \E P\bigg( \bigg| \frac{S_{n,m}-a_{n,m}}{b_{n,m}}\bigg| > \epsilon \bigg | \|\lambda x_{1} + z\| \bigg) \rightarrow 0.
\end{equation*}
Therefore, we conclude
\begin{equation*}
    \mathcal{A}_{n,m} \overset{p}{\rightarrow} 1.
\end{equation*}
\end{proof}

\begin{lemma}\label{lem::B-term-converges-to-infty}
    Assume $x_{1}, \ldots, x_{m} \simiid \calN(0, \frac{1}{n}I_{n})$, $z\sim \calN(0, I_{n})$ and $\{x_{i}: i=1,\ldots,m\}$ being independent with $z$. Suppose $n, m\rightarrow \infty$, $(\log m)/n \rightarrow 0$. Let $\lambda >0$ and $\sqrt{2\log m} - \lambda \rightarrow \infty$. Let $\mathcal{B}_{n,m}$ be defined in \eqref{term::B-first-order-spike}. Then 
    \begin{equation*}
        \mathcal{B}_{n,m} = \frac{(m-1) (1+\frac{\lambda^{2}}{n})^{-\frac{n}{2}} \exp\left( \frac{1}{2} \frac{1}{1+n/\lambda^{2}} \|z+\lambda x_{1}\|^{2} \right)}{\exp\left( \frac{\lambda^{2}}{2}\|x_{1}\|^{2} + \lambda x_{1}^{T}z \right)} \overset{p}{\rightarrow} +\infty.
    \end{equation*}
\end{lemma}

\begin{proof}
    \begin{equation*}
    \mathcal{B}_{n,m} = (m-1) \left(1+\frac{\lambda^{2}}{n}\right)^{-\frac{n}{2}} \exp \left[ \frac{1}{2(1+n/\lambda^{2})} \|z\|^{2} - \left(1-\frac{1}{1+n/\lambda^{2}}\right)\left(\lambda x_{1}^{T}z + \frac{\lambda^{2}}{2} \|x_{1}\|^{2}\right) \right].
\end{equation*}
Using that 
\begin{itemize}
    \item $\|z\|^{2} = n + O_{p}(\sqrt{n})$,
    \item $\frac{\lambda^{2}}{2} \|x_{1}\|^{2} + \lambda x_{1}^{T} z = \frac{\lambda^{2}}{2} \Big( 1+O_{p}(\frac{1}{\sqrt{n}}) \Big) + \lambda \cdot O_{p} (1)$,
\end{itemize}
we have
\begin{eqnarray*}
    \mathcal{B}_{n,m} &=& \big(1+o_{p}(1)\big) \exp \bigg[ \log (m-1) - \frac{\lambda^{2}}{2} + \frac{1}{2(1+n/\lambda^{2})} \Big(n + O_{p}(\sqrt{n})\Big) \\
    && - \frac{n/\lambda^{2}}{1+n/\lambda^{2}} \Big( \frac{\lambda^{2}}{2} + O_{p} \Big(\sqrt{\log m} + \frac{\log m}{\sqrt{n}} \Big) \Big) \bigg] \\
    &=& \big(1+o_{p}(1)\big) \exp\bigg[ \log (m-1) - \frac{\lambda^{2}}{2} + O_{p}\Big( \sqrt{\log m} + \frac{\log m}{\sqrt{n}} \Big) \bigg].
\end{eqnarray*}
Note that $\log (m-1) - \frac{\lambda^{2}}{2} = \Big( \sqrt{\log (m-1)} - \frac{\lambda}{\sqrt{2}} \Big) \Big( \sqrt{\log (m-1)} + \frac{\lambda}{\sqrt{2}} \Big)$. For $\sqrt{2\log m} - \lambda \rightarrow +\infty$, $\log (m-1) - \frac{\lambda^{2}}{2} = \omega(\sqrt{\log (m-1)})$. Since $(\log m)/n \rightarrow 0 $, $(\log m)/\sqrt{n} = o(\sqrt{\log m})$. Thus, $\log (m-1) - \frac{\lambda^{2}}{2} = \omega (\sqrt{\log (m-1)} + \frac{\log m}{\sqrt{n}})$ and $\log (m-1) - \frac{\lambda^{2}}{2} \rightarrow + \infty$. Therefore,
\begin{equation*}
    \mathcal{B}_{n,m} \overset{p}{\rightarrow} + \infty.
\end{equation*}
\end{proof}

\begin{lemma}\label{lem::wlln-conditions-lemma}
Assume $x_{1}, \ldots, x_{m} \simiid \calN(0, \frac{1}{n}I_{n})$, $z\sim \calN(0, I_{n})$ and $\{x_{i}: i=1,\ldots,m\}$ being independent with $z$. Let
\begin{equation*}
    Y_{m,i} := \exp\Big[ \|\lambda x_{1} + z\|\lambda x_{i,1} - \frac{\lambda^{2}}{2}x_{i,1}^{2} - \frac{\lambda^{2}}{2}\|x_{i,-1}\|^{2} \Big], \quad i=2,\ldots, n.
\end{equation*}
Let $Z\sim \mathcal{N}(0,1)$, $\chi_{n-1}^{2}$ denote the chi-squared variable with degrees of freedom $n-1$. $(Z, \chi_{n-1}^{2})$ are independent with $(x_{1}, z)$. Then for $\forall \lambda >0$ and $\forall b>0$,
\begin{enumerate}[label=(\roman*)]
    \item \begin{eqnarray*}
        && \sum_{i=2}^{m} P(Y_{m,i}> b |\|\lambda x_{1} + z\|) = (m-1)\\
        && \cdot P\bigg(\bigg(\sqrt{n} x_{2,1} - \frac{\sqrt{n}}{\lambda}\|\lambda x_{1} + z\|\bigg)^{2} + (\sqrt{n}\|x_{2,-1}\|)^{2} < \frac{n}{\lambda^{2}} (\|\lambda x_{1} + z\|^{2} - 2\log b) \bigg\vert \|\lambda x_{1} + z\| \bigg). \nonumber
    \end{eqnarray*}
    \item
    \begin{eqnarray*}
        && \sum_{i=2}^{m} \E\left[Y_{m,i}^{2}\mathbbm{1}_{(Y_{m,i}\leq b)}|\|\lambda x_{1} + z\|\right] \\
        &=& (m-1) \left(1+\frac{2\lambda^{2}}{n}\right)^{-\frac{n}{2}} \exp \left( \frac{2\| \lambda x_{1} + z\|^{2}}{2+n/\lambda^{2}} \right) \cdot \nonumber\\
        && P\left[\left. \left(Z - \frac{n/\lambda^{2}}{\sqrt{2+n/\lambda^{2}}} \|z+\lambda x_{1}\| \right)^{2} + \chi_{n-1}^{2} \geq (2+\frac{n}{\lambda^{2}})(\|\lambda x_{1} + z\|^{2} - 2\log b)  \right\vert \|\lambda x_{1} + z\|\right]. \nonumber
    \end{eqnarray*}
    \item 
    \begin{eqnarray*}
        && \sum_{i=2}^{m} \E \left[ \left. Y_{m,i} \mathbbm{1}_{(Y_{m,i}\leq b)} \right\vert \|z+\lambda x_{1}\| \right] \nonumber\\
        &=& (m-1) \left(1+\lambda^{2}/n\right)^{-\frac{n}{2}} \exp \left( \frac{\|z+\lambda x_{1}\|^{2}}{2(1+n/\lambda^{2})} \right) \cdot \nonumber\\
        && P\left[  \left(Z-\frac{n/\lambda^{2}\|z+\lambda x_{1}\|}{\sqrt{1+n/\lambda^{2}}}\right)^{2} + \chi_{n-1}^{2} \geq \left(1+\frac{n}{\lambda^{2}}\right) \left( \|z+\lambda x_{1}\|^{2} - 2\log b \right) \right]. \nonumber
    \end{eqnarray*}
\end{enumerate}
\end{lemma}
\begin{proof}
    $Y_{m,i} \leq b$ is equivalent to 
    \begin{eqnarray*}
        && \exp\left[ -\frac{1}{2} (\lambda x_{i,1} - \|\lambda x_{1} + z\|)^{2} - \frac{1}{2} \lambda^{2} \|x_{i,-1}\|^{2} + \frac{1}{2}\|\lambda x_{1} + z\|^{2} \right] \leq b \\
        &\Leftrightarrow& (\lambda x_{i,1} - \|\lambda x_{1} + z\|)^{2} + (\lambda \|x_{i,-1}\|)^{2} \geq \|\lambda x_{1} + z\|^{2} - 2\log b.
    \end{eqnarray*}
    Thus, equality (i) follows. 

    To show equality (ii), we first take extra condition on $x_{i,-1}$ and integrate with $x_{i,1}$. By combining the exponential function with the normal density function of $x_{i,1}$, we obtain
    \begin{eqnarray}
        && \E\left[ \left.Y_{m,i}^{2} \mathbbm{1}_{Y_{m,i}\leq b} \right\vert x_{i,-1}, \|z+\lambda x_{1}\|\right] \nonumber\\
        &=& \E \left[\exp\left( 2\lambda \|\lambda x_{1} + z\| x_{i,1} - \lambda^{2} x_{i,1}^{2} - \lambda^{2} \|x_{i,-1}\|^{2} \right) \right.\nonumber\\
        &&\left.\left. \cdot \mathbbm{1}_{\big\{(\lambda x_{i,1} - \|\lambda x_{1} + z\|)^{2} + (\lambda \|x_{i,-1}\|)^{2} \geq \|\lambda x_{1} + z\|^{2} - 2\log b\big\}} \right\vert x_{i,-1}, \|z+\lambda x_{1}\|\right] \nonumber\\
        &=& \frac{1}{\sqrt{1+2\lambda^{2}/n}} \exp\left( \frac{2\|z+\lambda x_{1}\|^{2}}{2+n/\lambda^{2}}\right) \cdot \exp\left(-\lambda^{2}\|x_{i,-1}\|^{2}\right) \nonumber\\
        &&  \cdot \mathbbm{1}_{\big\{\left(Z-\frac{n/\lambda^{2}}{\sqrt{2+n/\lambda^{2}}}\|z+\lambda x_{1}\|\right)^{2} \geq \left(2+\frac{n}{\lambda^{2}}\right)\left(\|\lambda x_{1}+z\|^{2} - 2\log b - \lambda^{2} \|x_{i,-1}\|^{2}\right)\big\}}, \label{eq::equality-ii-1}
    \end{eqnarray}
    where $Z\sim \mathcal{N}(0,1)$ and $\chi_{n-1}^{2}$ denote the Chi-squared random variable with degrees of freedom $n-1$. $(Z, \chi_{n-1}^{2}$ are independent with $(x_{1}, x_{i,-1}, z)$ for each $i=1,\ldots n$. Then, taking the expectation of $x_{i,-1}$ and using $n\|x_{i,-1}\|^{2}\sim \chi^{2}_{n-1}$, 
    \begin{eqnarray}
        && \E\left[e^{-\lambda^{2}\|x_{i,-1}\|^{2}} \cdot \mathbbm{1}_{\big\{\left(Z-\frac{n/\lambda^{2}}{\sqrt{2+n/\lambda^{2}}}\|z+\lambda x_{1}\|\right)^{2} \geq \left(2+\frac{n}{\lambda^{2}}\right)\left(\|\lambda x_{1}+z\|^{2} - 2\log b - \lambda^{2} \|x_{i,-1}\|^{2}\right)\big\}}\bigg| \|\lambda x_{1} + z\|\right] \nonumber\\
        &=& \E\left[ e^{-\frac{\lambda^{2}}{n} \cdot n \|x_{i,-1}\|^{2}} \cdot \mathbbm{1}_{\Big\{ n\|x_{i,-1}\|^{2} \geq \frac{n}{\lambda^{2}} \left( \|\lambda x_{1} + z\|^{2} - 2\log b \right) - \frac{n/\lambda^{2}}{2+n/\lambda^{2}} \left( Z - \frac{n/\lambda^{2}}{\sqrt{2+n/\lambda^{2}}} \|\lambda x_{1} + z\| \right)^{2}  \Big\}} \bigg| \|\lambda x_{1} + z\| \right] \nonumber\\
        &=& P\bigg\{ \chi_{n-1}^{2} \geq \bigg(1+\frac{2\lambda^{2}}{n}\bigg) \bigg[ \frac{n}{\lambda^{2}} \Big( \|\lambda x_{1} + z\|^{2} - 2\log b \Big) \nonumber\\
        && - \frac{n/\lambda^{2}}{2+n/\lambda^{2}} \Big(Z - \frac{n/\lambda^{2}}{\sqrt{2+n/\lambda^{2}}}\|z+\lambda x_{1}\|\Big)^{2} \bigg] \bigg| \|\lambda x_{1} + z\| \bigg\} \nonumber\\
        &=& P\bigg\{ \Big(Z - \frac{n/\lambda^{2}}{\sqrt{2+n/\lambda^{2}}}\|z+\lambda x_{1}\|\Big)^{2} + \chi_{n-1}^{2} \geq \Big(2 + \frac{n}{\lambda^{2}}\Big) \Big( \|\lambda x_{1} + z\|^{2} - 2\log b \Big) \bigg| \|\lambda x_{1} + z\| \bigg\}. \label{eq::equality-ii-2}
    \end{eqnarray}
    Equality (ii) follows by taking expectation with $x_{i,-1}$ of equation \eqref{eq::equality-ii-1} and using \eqref{eq::equality-ii-2}. 

    The argument of equality (iii) follows similarly from equality (ii).
\end{proof}
